Follow the Sun and Go with the Wind: Carbon Footprint Optimized Timely E-Truck Transportation

We study the carbon footprint optimization (CFO) of a heavy-duty e-truck traveling from an origin to a destination across a national highway network subject to a hard deadline, by optimizing path planning, speed planning, and intermediary charging planning. Such a CFO problem is essential for carbon-friendly e-truck operations. However, it is notoriously challenging to solve due to (i) the hard deadline constraint, (ii) positive battery state-of-charge constraints, (iii) non-convex carbon footprint objective, and (iv) enormous geographical and temporal charging options with diverse carbon intensity. Indeed, we show that the CFO problem is NP-hard. As a key contribution, we show that under practical settings it is equivalent to finding a generalized restricted shortest path on a stage-expanded graph, which extends the original transportation graph to model charging options. Compared to alternative approaches, our formulation incurs low model complexity and reveals a problem structure useful for algorithm design. We exploit the insights to develop an efficient dual-subgradient algorithm that always converges. As another major contribution, we prove that (i) each iteration only incurs polynomial-time complexity, albeit it requires solving an integer charging planning problem optimally, and (ii) the algorithm generates optimal results if a condition is met and solutions with bounded optimality loss otherwise. Extensive simulations based on real-world traces show that our scheme reduces up to 28% carbon footprint compared to baseline alternatives. The results also demonstrate that e-truck reduces 56% carbon footprint than internal combustion engine trucks.

==> algs/approx-high-soc.tex <==

\begin{algorithm}[!tb]

    % \newcommand{\multiline}[1]{%
    %     \begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
    %       #1
    %     \end{tabularx}
    % }

    \caption{test$(s, d, \beta_0, T, \Omega, \epsilon_\beta, \epsilon_F)$}\label{alg:appro-high-soc-test}
    \begin{algorithmic}[1]
        % \SetInd{0.25em}{0.1em}
        \State $\delta_\beta \gets \frac{\epsilon_\beta B}{|V|+1}$, 
        $\underline{M}_{\beta} \gets - (|V|+1)$, 
        $\overline{M}_{\beta} \gets \lceil \frac{|V|+1}{\epsilon_\beta} \rceil$
        \State $\delta_F \gets \frac{\epsilon_F \Omega}{|V|+1}$, $M_F \gets \lceil \frac{|V|+1}{\epsilon_F}\rceil + |V| + 1 $
        \State $\psi \gets $ NULL
        \For{$i \gets \overline{M}_{\beta} \text{ to } \underline{M}_{\beta}, v \in V \cup \{s,d\}$ }
            \State $\psi' \gets \text{getMinT}(v,B,i\delta_\beta, \epsilon_\beta)$ 
            \State $\psi \gets \text{merge}(\psi', \psi)$
        \EndFor
        \State $\sigma(s,s,\cdot, \cdot, \cdot) \gets 0$
        \State $\sigma(s,v,\cdot, \cdot, \cdot) \gets \infty, \forall v \in V \backslash \{s\}$

        \For{$i_c \gets \overline{M}_{\beta} \text{ to } \underline{M}_{\beta}$,
        $i_v \gets \overline{M}_{\beta} \text{ to } \underline{M}_{\beta}$,
        $i_{ini} \gets \overline{M}_{\beta} \text{ to } \underline{M}_{\beta}$,}
        \For{$i_\rho \gets 1 \text{ to } M_F$,\, $i_F \gets 1 \text{ to } M_F$}
        \For{$u\in \cup \{s,d\},\, v \in V_c \cup \{s,d\}$}
            \State $\beta_c \gets i_c \delta_\beta$,
            $\beta_v \gets i_v \delta_\beta$,
            $\beta_{ini} \gets i_{ini} \delta_\beta$
            \State $\rho \gets i_\rho \delta_F$, 
            $\hat{F} \gets i_F \delta_F$, 
            % \State $t_c \gets \phi^{-1}(\beta_{ini}, \beta_c)$
            \State $t_c \gets \Phi_u^{-1}( \min\{ B, \beta_{ini} + \beta_c) \} - \Phi_u^{-1}(\beta_{ini})$
            \State $\tau \gets \psi(s, u, \beta_0, \beta_v)$
            \State $t_w \gets g_v(\beta_{ini}, t_c, \tau, \hat{F})$
            \State $t_r \gets \psi(u,v, \min \left\{ \beta_{ini} + \beta_c, B \right\}, \beta_v)$
            \State $\sigma_u \gets \sigma(s, u, \rho, \beta_0, \beta_{ini}) $
            \State $\tilde{\sigma} \gets \sigma_u + t_r + t_w + t_c $
            \State $\sigma_v \gets \sigma(s, v, \rho, \beta_0, \beta_v) $
            \If{ $\tilde{\sigma} \leq \sigma_v$ }
                \State $\sigma(s, v, \rho, \beta_0, \beta_v) \gets \tilde{\sigma}$
            \EndIf
        \EndFor
        \EndFor
        \EndFor
        % $\text{sol} \gets \text{NULL}$, 
        

        \State Let $i^*_\rho \in \left\{ 1,\cdots, M \right\}$ be the minimal $i_\rho$ such that $\sigma(s, d, i_\rho \delta_F, \beta_0, \lfloor \frac{\beta_{lb} -\epsilon B}{\delta_\beta}  \rfloor \delta_\beta ) \leq T $
        \If{$\rho^*$ exists}
            \State sol $\gets$ the solution corresponding to $\rho^*$
        \Else
            \State sol $\gets$ NULL
        \EndIf
        \State \Return sol
        
    \end{algorithmic}
\end{algorithm}

==> algs/approx-high.tex <==

\begin{algorithm}[!tb]

    % \newcommand{\multiline}[1]{%
    %     \begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
    %       #1
    %     \end{tabularx}
    % }

    \caption{solveCFO$(s,d,T,\beta_0, \epsilon)$ \textcolor{blue}{Not ready yet. This form of algorithm might be wrong...}}\label{alg:appro-high}
    \begin{algorithmic}[1]
        % \SetInd{0.25em}{0.1em}
        \State 
        % $\text{sol} \gets \text{NULL}$, 
        $\delta\gets\frac{\epsilon T}{|V|+1}$, $M\gets\lceil \frac{|V|+1}{\epsilon} \rceil + |V| + 1$
        \State $\rho(s,s, i\delta, \beta_0) \gets 0, \forall i \in \left\{ 1,...,M \right\}$
        \State $\rho(s,v, i\delta, \beta_0) \gets \infty, \forall i \in \left\{ 1,...,M \right\}, \forall v \in V \backslash \{s\}$
        \State $\beta_s \gets \beta_0$
        \State $\beta_v \gets -\infty, \forall v \in V \backslash \{s\}$
        \For{$i_c \gets 1$ to $M$, $i_w \gets 1$ to $M$, $i_{r} \gets 1$ to $M$, $i_{\tau} \gets 1$ to $M$}
            \State $t_c \gets i_c\delta,\, t_w \gets i_w\delta $
            \State $t_r \gets i_c\delta,\, \tau \gets i_{\tau}\delta $
            \If{$t_c \in [0, t_c^{ub}+\delta]$ and $t_w \in [t_w^{lb}, t_w^{ub}+\delta]$}
            \State $t_c \gets \min \left\{ t_c, t_c^{ub} \right\}$, $t_w \gets \min \left\{ t_w, t_w^{ub} \right\}$
            \For{$u \in \{s,d\} \cup V_c,\, v \in \{s,d\} \cup V_c $}
                \State $\tilde{\rho} \gets \rho(s, u, \tau, \beta_0) + F_u(\beta_u, t_c, \tau+t_w)$
                \State $\rho_{prev} \gets \rho(s, v, \tau + t_c + t_w + t_r)$
                \State { \Longunderstack[l]{$\tilde{\beta}\gets\beta(u,v,t_r,\beta_u+\phi(t_c,\beta_u))$ \\\; computed by calling Algorithm~\ref{alg:appro-low} \\\; with the same parameters and tolerance $\epsilon$}}.
                \If{$\tilde{\rho} < \rho_{prev} $ and $\tilde{\beta}\geq 0$}
                    \State $\rho(s,v,\tau+t_c+t_w,t_r) \gets \tilde{\rho}$
                    \State $\beta_v \gets \tilde{\beta}$
                \EndIf
                % \If{$t_e \in [t_e^{lb}, t_e^{ub}]$ }
                %     \State $\tilde{\beta} \gets \min\left\{ B, \beta(s,u, \tau, \beta_0) - c_e(t_e) \right\}$
                %     \If{$\tilde{\beta} \geq 0$}
                %         \State \Longunderstack[l]{$\beta(s,v,\tau+t_e,\beta_0)=$
                %         $\qquad\max\left\{\tilde{\beta},\beta(s,v,\tau+t_e,\beta_0)\right\}$%$\max\{\tilde{\beta},\beta(s,v,\tau+t_e, \beta_0)\}$
                %         % $  $
                %         }
                %     \EndIf
                % \EndIf
            \EndFor
            \EndIf
        \EndFor

        \If{\textcolor{blue}{TODO:}}
            \State sol $\gets$ the solution for ... % $\beta\left(s,d,(1+\epsilon)T_0,\beta_0\right)$
        \Else
            \State sol $\gets$ NULL
        \EndIf
        \State \Return sol
        
    \end{algorithmic}
\end{algorithm}

==> algs/approx-low-soc.tex <==

\begin{algorithm}[!tb]

    % \newcommand{\multiline}[1]{%
    %     \begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
    %       #1
    %     \end{tabularx}
    % }

    \caption{getMinT$(s,B_0,\beta_0, \epsilon)$}\label{alg:appro-low-soc}
    \begin{algorithmic}[1]
        % \SetInd{0.25em}{0.1em}
        % \State \textbf{Initialization Phase:} 
        % $\text{sol} \gets \text{NULL}$, 
        \State $\delta\gets\frac{\epsilon B_0}{|V|+1}$, 
        $\underline{M}\gets  -(|V| + 1) $, 
        $\overline{M}\gets \lceil \frac{|V|+1}{\epsilon} \rceil$
        \State  $\psi(s,s, \beta_0, i\delta) \gets 0, \forall i \in \left\{ \underline{M},...,\overline{M} \right\}$
        \State  $\psi(s,v, \beta_0, i\delta) \gets \infty, \forall i \in \left\{ \underline{M},...,\overline{M} \right\}, \forall v \in V \backslash \{s\}$
        \For{$i \gets \overline{M}$ to $\underline{M}$, }
            \For{$e = (u,v) \in E$}
            \For{$j \gets \lfloor \frac{c^{lb}_e}{\delta} \rfloor \text{ to } \lceil \frac{c^{ub}_e}{\delta} \rceil $}
                \State $\beta_u \gets i\delta, \hat{c} \gets j\delta$
                \State \begin{equation*}
                    % \setlength{\mathindent}{0pt}
                    % \hspace{-5mm}
                    t_e \gets \left\{  
                        \begin{aligned}
                            & t_e^{lb},& \text{if } j = \lceil \frac{c_e^{ub}}{\delta} \rceil, \\
                            & c_e^{-1}(\hat{c}), & \text{if } \hat{c} \in [c_e^{lb}, c_e^{ub}),  \\
                            & \infty, & \text{otherwise}.
                        \end{aligned}
                    \right.
                \end{equation*}
                \State $\beta_v \gets \min \{B, \beta_u - \hat{c}\}$
                \If{$ \beta_v \in [-\epsilon B, B]$}
                    \State $\tilde{\psi} \gets \psi(s, u, \beta_0, \beta_u) + t_e$
                    \State $\psi_{prev} \gets \psi(s, v, \beta_0, \beta_v) $
                    \State $\psi(s,v, \beta_0, \beta_f-\hat{c}) \gets \min \left\{ \tilde{\psi}, \psi_{prev}  \right\}$
                \EndIf
                % \If{$t_e \in [t_e^{lb}, t_e^{ub} + \delta]$ }
                %     \State $t_e \gets \min \left\{ t_e, t_e^{ub} \right\}$
                %     \State $\tilde{\psi} \gets \min\left\{ B, \psi(s,u, \tau, \beta_0) - c_e(t_e) \right\}$
                %     \If{$\tilde{\psi} \geq 0$}
                %         \State \Longunderstack[l]{$\psi(s,v,\tau+t_e,\beta_0)\gets$
                %         \\ $\qquad\max\left\{\tilde{\psi},\psi(s,v,\tau+i\delta,\beta_0)\right\}$%$\max\{\tilde{\beta},\beta(s,v,\tau+t_e, \beta_0)\}$
                %         % $  $
                %         }
                %     \EndIf
                % \EndIf
            \EndFor
            \EndFor
        \EndFor

        \State \Return $\psi$
        
    \end{algorithmic}
\end{algorithm}

==> algs/approx-low.tex <==

\begin{algorithm}[!tb]

    % \newcommand{\multiline}[1]{%
    %     \begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
    %       #1
    %     \end{tabularx}
    % }

    \caption{getMaxSoC$(s,T_0,\beta_0, \epsilon)$}\label{alg:appro-low}
    \begin{algorithmic}[1]
        % \SetInd{0.25em}{0.1em}
        % \State \textbf{Initialization Phase:} 
        % $\text{sol} \gets \text{NULL}$, 
        \State $\delta\gets\frac{\epsilon T_0}{|V|+1}$, $M\gets \left(   \lceil \frac{|V|+1}{\epsilon} \rceil + |V| + 1 \right)$
        \State  $\Omega(s,s, i\delta, \beta_0) \gets \beta_0, \forall i \in \left\{ 1,...,M \right\}$
        \State  $\Omega(s,v, i\delta, \beta_0) \gets - \infty, \forall i \in \left\{ 1,...,M \right\}, \forall v \in V \backslash \{s\}$
        \For{$i \gets 1$ to $M$, $j \gets 1$ to $M$}
            \For{$e = (u,v) \in E$}
                \State $t_e \gets i\delta, \tau \gets j\delta$
                \If{$t_e \in [t_e^{lb}, t_e^{ub} + \delta]$ }
                    \State $t_e \gets \min \left\{ t_e, t_e^{ub} \right\}$
                    \State $\tilde{\Omega} \gets \min\left\{ B, \Omega(s,u, \tau, \beta_0) - c_e(t_e) \right\}$
                    \If{$\tilde{\Omega} \geq 0$}
                        \State \Longunderstack[l]{$\Omega(s,v,\tau+t_e,\beta_0)\gets$
                        \\ $\qquad\max\left\{\tilde{\Omega},\Omega(s,v,\tau+i\delta,\beta_0)\right\}$%$\max\{\tilde{\beta},\beta(s,v,\tau+t_e, \beta_0)\}$
                        % $  $
                        }
                    \EndIf
                \EndIf
            \EndFor
        \EndFor

        % \If{$\beta\left(s,d,(1+\epsilon)T_0,\beta_0\right) \geq 0$}
        %     \State sol $\gets$ the solution for $\beta\left(s,d,(1+\epsilon)T_0,\beta_0\right)$
        % \Else
        %     \State sol $\gets$ NULL
        % \EndIf

        % \For{$k \gets 1$ to $K$}
        %     % \State Compute $\text{sol}^+$ with $\vec{\lambda}[k]$ by solving problem~\eqref{prob:dual} \label{alg:dualsub:primal}
        %     \If{$\delta_i^\beta[k] = 0$ and $\delta_i^\tau[k] = 0, \forall i\in \left\{ 1,...,N+1 \right\}$}
        %         \State \Return sol $\gets \text{sol}^+$  \label{alg:dualsub:optimal}
        %     \EndIf
        %     \If{$\delta_i^\beta[k] \leq 0$ and $\delta_i^\tau[k] \leq 0, \forall i\in \left\{ 1,...,N+1 \right\}$ \textbf{and} $\text{sol}^+$ has less objective }
        %         \State sol $\gets \text{sol}^+$ 
        %     \EndIf
        %     % \State $\hat{p} \gets \text{DFS}(\emptyset, p^\star, n)$
        %     % \If{$g(\hat{p}) < g(p^\star) $}
        %     %     \State $p^\star \gets \hat{p}$
        %     % \State Compute $\vec{\lambda}[k+1]$ according to~\eqref{eq:dualupdate}.
        % \EndFor
        \State \Return $\Omega$
        
    \end{algorithmic}
\end{algorithm}

==> algs/dfs.tex <==

\begin{algorithm}[htb]
    \caption{Iterative Deepening Approach}\label{alg:ida}
    \begin{algorithmic}[1]
        \State \textbf{Initialization:} $p^\star = \emptyset, N=|\csgpre{V}|$ \label{alg:ida:1}
        \For{$n \gets 2$ to $N$}
            \State $\hat{p} \gets \text{DFS}(\emptyset, p^\star, n)$
            \If{$g(\hat{p}) < g(p^\star) $}
                \State $p^\star \gets \hat{p}$
            \EndIf
        \EndFor
        \State \Return $p^\star$ \label{alg:ida:end}
        \State
        \Procedure{DFS}{$p$, $p^\star$, $n$} \label{alg:ida:dfs1}
            \If{$(|p| == n)$ and $(p_n == d)$ }
                \If{$g(p) < g(p^\star) $}
                    \State $p^\star \gets p$
                \EndIf
                \State \Return $p^\star$
            \EndIf
            \State $u \gets \text{tail}(p)$
            \For{ $\forall (u, v) \in \csgpre{E}$  }
                \State $p' \gets p \circ v$ 
                \If{TEST($p'$)}  \Comment{See Algorithm~\ref{alg:test}}
                    \State $p^\star \gets \text{DFS}(p', p^\star, n) $ 
                \EndIf
            \EndFor
            \State \Return $p^\star$
        \EndProcedure \label{alg:ida:dfsend}
    \end{algorithmic}
\end{algorithm}



==> algs/test.tex <==

\begin{algorithm}[htb]
    \caption{Candidate Test}\label{alg:test}
    \begin{algorithmic}[1]
        \Procedure{Test}{$p=[p_1,...,p_k]$, $p^\star$} 
        \If{ $\tilde{t}^{lb}(p) > T$} \label{alg:test:ddl}
            \State \Return false
        \EndIf
        \If{distance($p_k,d$) > distance($p_{k-1},d$)} \label{alg:test:distance}
            \State \Return false
        \EndIf
        \If{$\underline{g}(p) > g(p^\star)$} \label{alg:test:lb} \Comment{See~\eqref{prob:csso-lp}}
            \State \Return false
        \EndIf

        \State \Return true
           
        \EndProcedure 
    \end{algorithmic}
\end{algorithm}

==> arxiv/4.1.csg.tex <==

% A prefix for charging station graph (csg)
\newcommand{\csgpre}[1]{\tilde{\mathcal{#1}}}
\newcommand{\exgpre}[1]{\hat{\mathcal{#1}}}

% \item We can add a virtual charging station at the destination $d$ for notation convenience, since there is no benefit to charge and wait at the end.

% In this section, we will ...
\subsection{Charging Station Graph}
\textcolor{blue}{TODO: Might need to rewrite to be compatible with the method described below}.
One of the core challenges in \textsf{CFO} is to ensure the SoC feasibility between two charging stations. 
% It is unclear an electric truck 
To address this, we consider a new graph $\csgpre{G} = (\csgpre{V}, \csgpre{E})$ on charging stations.
Here $\csgpre{V} = \mathcal{V}_c \cup \{s,d\} $ is the set of charging stations along with two points origin $s$ and destination $d$. 
The construction of the edge set $\csgpre{E}$ requires more efforts. 
We want to eliminate charging station pairs $(i,j)$ that $j$ is not reachable from $i$ without intermediate recharging.
In particular, for each $i\in \csgpre{V} $ and $j \in \csgpre{V}$, we define $C_{ij}(\tau)$ as the minimum energy consumption traveling from $i$ to $j$ in the original graph~$\mathcal{G}$ without charging stops, subject to deadline $\tau$.
In particular, $C_{ij}(\tau)$ is the optimal value of the \textsf{PASO} problem with deadline $\tau$.
\begin{equation}
\begin{aligned}
   C_{ij}(\tau) = \min_{\vec{t} \in \mathcal{T}, \vec{x} \in \mathcal{X}_{ij}^r }\;& \sum_{(u,v) \in \mathcal{E}_r}^{} x_{uv} c_{uv}(t_{uv})   \\
    \text{s.t. }\;& \sum_{(u,v)\in \mathcal{E}_r} x_{uv} t_{uv} \leq \tau
\end{aligned} \label{prob:paso}
\end{equation}
Note that computing the optimal value of the problem~\eqref{prob:paso} is also NP-hard. However, we can obtain an upper bound of problem~\eqref{prob:paso} with small optimality loss by efficient heuristics (e.g.,~\cite{dengEnergyefficient2017}). Our method in the following is still applicable if we replace the value of $C_{ij}(\tau)$ with its upper bound.

% Another issue, however, requires more efforts to tackle
% $C_{ij}(T)$ can be shown to be non-increasing.
% We need to ignore regenerative system here to ensure the SoC feasibility.

For each $i\in \csgpre{V}$ and $j \in \csgpre{V}$, define the $t_{ij}^{fast}$ and $t_{ij}^{slow}$ as the minimum traveling time and maximum traveling time respectively between origin $i$ and destination $j$ without intermediate recharging stops. 
Then we can denote the set of $\csgpre{E}$ as 
\begin{align}
    \csgpre{E} = \left\{ (i,j) \in \csgpre{V} \times \csgpre{V} : C_{ij}(t^{slow}_{ij}) \leq \alpha B \right\} \label{set:csedge}
\end{align}
That is, there is an edge between $i$ and $j$ only when $j$ is reachable from $i$ without intermediate recharging stops. Here $0 \leq \alpha \leq 1$ is a constant to address the negative value of $c_{uv}(\cdot)$ in~\eqref{prob:paso} due to the regenerative system. In particular, because $c_{uv}(\cdot)$ can have negative value, the difference between maximum SoC and minimum SoC can be larger than the summation of $c_{uv}(\cdot)$ as illustrated in Fig.~\ref{fig:soc-alpha}. So we use $\alpha B$ as a soft penalty to ensure the SoC constraint between $i$ and $j$. 
Note that the worst case rarely happens in practice and the regenerative system of an electric truck has little impact during the whole path~\cite{su2021Energy}. Therefore, it is sufficient to choose a fairly large $\alpha$ (e.g., $0.95$) in practice which only introduce little optimality loss.

\begin{figure}[!tb]
    \includegraphics[width=.9\linewidth]{figs/socAlpha.pdf}
    \vspace{-4mm}
    \caption{SoC profile along a path. 
    We use $\alpha$ to give a soft penalty to ensure the SoC constraint.
    }\label{fig:soc-alpha}
    \vspace{-5mm}
\end{figure}

For each edge $(i,j) \in \csgpre{E}$, we define three decision variables related to time planning $t_{ij}^r$, $t_{ij}^w$, $t_{ij}^c$, denoting the amount of time for driving on the real road segment, waiting at the charging station, and charing at the charging station, respectively.
We define the objective function $\tilde{F}_{ij}$ the same as the objective function for the charging station $j$. 
For each $(i,j)\in \csgpre{E}$, we assign a time lower bound and time upper bound for the time driving on road $t_{ij}^r$:
% We can then define the time limit for real road part of edge $(i,j) \in \csgpre{E}$.
\begin{align}
    \tilde{t}_{ij}^{ub} = t_{ij}^{slow}, \qquad
    \tilde{t}_{ij}^{lb} =
    \left\{  
    \begin{aligned}
        & t_{ij}^{fast} &\, \text{if }  C_{ij}(t_{ij}^{fast}) \leq \alpha B, \\
        & C_{ij}^{-1}(\alpha B) &\, \text{otherwise.}
    \end{aligned}
    \right.
\end{align} 
Here, $C_{ij}^{-1}(\cdot)$ is the inverse function of $C_{ij}(\cdot)$. Note that $C_{ij}(\tau)$ is a non-decreasing function with respect to $\tau$ since increase $\tau$ will enlarge the constraint set for the problem~\eqref{prob:paso}. 
Therefore, we can always found the (upper bound) value of $C_{ij}^{-1}(\cdot)$ by a simple bisection.
Therefore, given any path on $\csgpre{G}$, there is always a time schedule that satisfies the SoC constraint, since one can always fully charge the battery before going to the next charging station.

==> arxiv/4.1.expanded-graph.tex <==

\subsection{Time-Expanded and Battery-Expanded Graph}
The CFO problem remains challenging on the charging station graph due to the coupling of decisions on each edge. That is, the decisions of driving time, waiting time and charging time at the current edge affects carbon-intensities of the following charging stations. To address this, we construct a new time-expanded and battery-expanded graph $\exgpre{G}=(\exgpre{V}, \exgpre{E})$ from the charging station graph $\csgpre{G}=(\csgpre{V},\csgpre{E})$. 
In particular, for each node $i \in \csgpre{V}$, we add $(N_{\tau}+1)(N_{\beta}+1)$ copies to the new node set $(i, i_\beta, i_\tau) \in \exgpre{V}$ for all $i_\beta = 0,...,N_\beta$ and $i_\tau = 0,...,N_\tau$. Here $N_\beta$ and $N_\tau$ are the number of discretized states for $\beta$ and $\tau$ respectively.
For each edge $(i,j) \in \csgpre{E}$, we add the edge $((i,i_\beta, i_\tau), (j, j_\beta, j_\tau))$ to the new edge set $\exgpre{E}$. 
An edge $((i,i_\beta, i_\tau), (j, j_\beta, j_\tau))$ means we require the e-truck to travel from node $i$ to $j$ with initial SoC $i_\beta B / N_\beta$, initial arrival time $i_\tau T / N_\tau$ at node $i$ and 
final SoC $j_\beta B / N_\beta$, final arrival time $j_\tau T / N_\tau$ at node $j$.
The cost for the edge $((i,i_\beta, i_\tau), (j, j_\beta, j_\tau))$ is given by
\begin{subequations}
    \begin{align}
        \min_{t^w, t^r, t^c}\;&  F_{ij}(\beta_i, t^c, \tau_i + t^w) \\
        \text{s.t. }\;& \tau_j = \tau_i + t^w + t^r + t^c \label{cons:exg:tau} \\
        & \beta_j = \beta_i + \phi(t^c, \beta_i) - C_{ij}(t^r_{ij}) \label{cons:exg:soc} \\
        & \beta_i = i_\beta B / N_\beta,  \,
        \beta_j = j_\beta B / N_\beta,  \\
        & \tau_i = i_\tau T / N_\tau, \,
        \tau_j = j_\tau T / N_\tau, \\
        & t^w \geq t^w_0, \tilde{t}^{lb}_{ij} \leq t^r \leq \tilde{t}^{ub}_{ij}, t^c \geq 0.
    \end{align} \label{prob:exg}
\end{subequations}

We discard the edge if problem~\eqref{prob:exg} is infeasible.
Despite the complexity of problem~\eqref{prob:exg} at the first glance, we can actually convert it to a single-variable optimization problem over an interval. Given on-road travel time $t^r$, we can uniquely determine $t^c$ by constraint~\eqref{cons:exg:soc} and then determine $t^w$ by constraint~\eqref{cons:exg:tau}. Then problem~\eqref{prob:exg} can be efficiently solved via classic algorithms (e.g. golden-section search~\cite{avriel1966optimally} or Powell's method~\cite{powell1964efficient}).
\textcolor{blue}{TODO: Maybe add explicit formulation?}

% The infeasible problem?

By constructing the expanded graph $\exgpre{G}$, we achieve to distribute the coupling decisions to different nodes and edges on the new graph. 
This allows us to simply apply a shortest path algorithm (e.g. Dijkstra) on the expanded graph $\exgpre{G}$ from node $(s, \lceil \beta_0/N_\beta \rceil, 0)$ to a virtual destination node $\hat{d}$. Here, we additionally add the node $\hat{d}$ and zero-weight edges $((d, i_\beta, i_\tau) , \hat{d})$ for all $i_\beta = 0,...,N_\beta$ and $i_\tau = 0,...,N_\tau$ for auxiliary purpose. Once obtain the path, we can retrieve the speed planning and charing scheduling decisions by solving problem~\eqref{prob:exg} along the given path.

We remark that by discretize the SoC and traveling time, we discard some of the feasible solutions because problem~\eqref{prob:exg} is not always feasible. 
% However, ()
\textcolor{blue}{TODO: Maybe we can provide a optimality bound in the following subsection}


\subsection{Performance Analysis}
\begin{itemize}
    \item Time complexity
    \begin{itemize}
        \item For constructing the graph.
        \item For solving one instance of CFO problem.
    \end{itemize}
    \item Optimality gap.
\end{itemize}

\subsection{Implementation Details}
\begin{itemize}
    \item Reducing the number of edges.
\end{itemize}

% \noindent\textbf{Time Complexity.}
% \\Complexity for constructing the graph: 
% \\Complexity for solving an instance of CFO.
% 
% \textbf{Performance guarantee:}


==> arxiv/4.1.ida.tex <==

\subsection{An Iterative Deepening Approach}
% In practice, a human driver may want to reduce the number of recharging stops. 
% The idea behind is that in practice, we can 
In practice, the number of recharging stops of a trip should not be too large if we take the human drivers' experience into account. Besides, large number of recharging stops may have little marginal benefit while significantly increases the time complexity. 
Based on those observations, we propose an iterative deepening approach by iteratively allowing more recharging stops in a path.
% At each iteration, we fix the number of 

\noindent\textbf{Time Scheduling and Speed Optimization.}
Let us first consider the case where a path $p = [p_1, ..., p_n]$ on $\csgpre{G}$ is given. Then the problem remains to solve the following \emph{charge scheduling and speed optimization} (CSSO) problem on the charging station graph.

\newcommand{\pip}{ {p_{i} p_{i+1}} }
\begin{subequations}
\begin{align}
   g(p) = \min_{\vec{t}, \vec{\beta}, \vec{\tau}}\;&  \sum_{i=1}^{n-1} 
   F_{p_i p_{i+1}}\left(\hat{\beta}_{p_i} , t_{p_i p_{i+1}}^c, \tau_{p_{i}} + t^w_{p_i p_{i+1}} + t^c_{p_i p_{i+1}} \right) \label{obj:spd} \\
    \text{s.t. }\;& \hat{\beta}_{p_i} = \beta_{p_i} - C_{p_i p_{i+1}}(t_{p_i p_{i+1}}^r) \geq 0, \forall i \in [1,n-1] \label{cons:spd:bhat} \\
    & \beta_{p_{i+1}} = \hat{\beta}_{p_{i}} + \phi(t^c_{p_i p_{i+1}}, \hat{\beta}_{p_i}), \forall i \in [1,n-1] \label{cons:spd:b} \\
    & \tau_{p_{i+1}} = \tau_{p_i} + t^r_{p_{i} p_{i+1}} + t^w_{\pip} + t^c_{\pip} , \forall i \in [1,n-1] \label{cons:spd:tau} \\
    & \sum_{i=1}^{n-1} \left(   t^r_{p_{i} p_{i+1}} + t^w_{\pip} + t^c_{\pip} \right) \leq T \label{cons:spd:ddl} \\
    & t^c_{\pip}  \geq 0, \; t^w_{\pip} \geq w_0, , \forall i \in [1,n-1] \label{cons:spd:box1} \\
    & \tilde{t}^{lb}_{\pip} \leq  t^r_{\pip} \leq \tilde{t}^{lb}_{\pip} , \forall i \in [1,n-1] \label{cons:spd:box2} \\
    & \beta_{p_1} = \beta_0, \, \tau_{p_1} = 0 \label{cons:spd:init}
\end{align} \label{prob:csso}
\end{subequations}
We additionally set $g(p)=\infty$ if the above problem is infeasible or $p=\emptyset$.
Here, the objective~\eqref{obj:spd} is the same as before. We introduce an auxiliary variable $\hat{\beta}$ in~\eqref{cons:spd:bhat} for notational convenience. 
Constraint~\eqref{cons:spd:bhat} is to ensure the SoC constraint. Constraints~\eqref{cons:spd:b} and \eqref{cons:spd:tau} are state variable constraints similar as before. Constraint~\eqref{cons:spd:ddl} is to satisfy the deadline constraint. 
Constraints~\eqref{cons:spd:box1} and \eqref{cons:spd:box2} are the box constraints on the time decision variables.
Constraint~\eqref{cons:spd:init} defines the initial conditions for $\beta$ and $\tau$. 
Note that the CSSO problem~\eqref{prob:csso} is defined on the charging graph~$\csgpre{G}$ and thus has much smaller size as compared to the CFO problem~\eqref{prob:cfo}. A typical size of~\eqref{prob:csso} is $n=10$ on the US national highway network.

Even though we reduce the problem to a specific path on the charging garph~$\csgpre{G}$, the CSSO problem ~\eqref{prob:csso} is still non-convex due to the non-convex objective~\eqref{obj:spd} and non-convex constraints~\eqref{cons:spd:bhat} and~\eqref{cons:spd:b}. 
Therefore, it is still difficult to obtain the global minimum. 
If our approach, however, an upper bound of $g(p)$ can also be used without further modification. Thus, we can use local minimization algorithm and solvers (e.g., NLopt~\cite{johnson2014nlopt}) to solve problem~\eqref{prob:csso}. 

\noindent\textbf{An Iterative Deepening Approach.} 
After defining the CSSO problem and $g(p)$, we are ready to reformulate the \textsf{CFO} problem in a iterative deepening manner on $\csgpre{G}$:
\begin{align}
    % \textsf{CFO-ID}: \quad 
    \min_{n\in \left\{ 2,...,|\csgpre{V}| \right\}}\; \min_{p \in \mathcal{P}_n} g(p)  \label{prob:cfo-id}
\end{align}
Here $|\csgpre{V}|$ is the number of nodes on $\csgpre{G}$. We denote $\mathcal{P}_n$ is the set of all paths from $s$ to $d$ with $n$ nodes:
\begin{equation}
\begin{aligned}
    \mathcal{P}_n = \Big\{ p = [p_1, &...,p_n] : p_1 = s,\, p_n = d, \text{ and } 
    \\ & (p_i, p_{i+1}) \in \csgpre{E},\, \forall i \in \left\{ 1,...,n-1 \right\} \Big\}
\end{aligned}
\end{equation}
We set $\mathcal{P}_n = \emptyset$ if no such path exists.
Problem~\eqref{prob:cfo-id} gives us a new perspective of solving \textsf{CFO} problem. 
We can first fix the number of nodes $n$ in a path, find the best path within $\mathcal{P}_n$, and increase the number of node in the next iteration. The overall procedure is outlined in Algorithm~\ref{alg:ida}.  Lines~\ref{alg:ida:1}-\ref{alg:ida:end} correspond to the outer minimization in problem~\eqref{prob:cfo-id} and the inner minimization problem is solved by a depth first search (DFS) procedure (lines~\ref{alg:ida:dfs1}-\ref{alg:ida:dfsend}). 
Note that in practice, it is sufficient to set the total number of outer iterations $N$ to a relatively small number to let Algorithm~\ref{alg:ida} produce high-quality solutions.

\input{algs/dfs.tex}
\input{algs/test.tex}

In the DFS procedure, for a path $p=[p_1,...,p_k]$, we use $\text{tail}(p) = p_k$ to denote the last node of $p$ and $|p|=k$ to denote the number nodes in $p$. We also use $p'=p\circ v = [p_1,...,p_k,v]$ to denote the concatenation of a path $p$ and a node $v$. The DFS procedure is defined in a recursive manner, if the searched path $p$ has exactly $n$ nodes, then we update the current best path $p^\star$ if necessary. 
Otherwise, we construct a new path $p'$ by the concatenation of $p$ and a out neighbor of tail($p$), recursively call DFS on $p'$.

\noindent\textbf{Candidate Test.}
Note that even through $n$ is relatively small in practice, the number of candidates $|\mathcal{P}_n| = O(|\csgpre{V}|^n)$ can still be very large, which leads to high computational cost. To reduce the computational cost, a candidate test procedure is therefore necessary to prune unnecessary branches in the DFS search tree.
A good candidate test procedure can significantly prune the DFS search space and speedup our algorithm. 

We provide several criteria to test a promising candidate path $p$ as outlined in Algorithm~\ref{alg:test}. 
% The first two conditions are straightforward. 
We first check if the minimum travel time already exceeds the deadline $T$ in line~\ref{alg:test:ddl} where we use $\tilde{t}^{lb}(p)$ to denote the minimum travel time of $p$. 
The second condition in line~\ref{alg:test:distance} is to check if path $p$ is heading towards the destination, where distance($u,v$) denotes the straight line distance between two nodes $u$ and $v$.
This condition is a heuristic to avoid path with back road.
The third condition in line~\ref{alg:test:lb} check the objective lower bound $\underline{g}(p)$ with the current best objective value $g(p^\star)$ and prune the sub-optimal branches.
% The problem remains on how to obtain a tight lower bound $\underline{g}(p)$. In 
There are many ways to obtain a lower bound of $g(p)$. In the following, we provide simple yet effective way by relaxing problem~\eqref{prob:csso} to a simple linear programming (LP). 
For each node $i\in \mathcal{V}_c$, we denote the lower bound of carbon intensity by
\begin{equation}
\underline{\pi}_i = \min_{ 0 \leq \tau \leq T} \pi_i(\tau)
\end{equation}
Given a path $p = [p_1, ..., p_k]$, we compute the lower bound $\underline{g}(p)$ by solving the following \textsf{csso-LP} problem.
\begin{subequations}
\begin{align}
    \underline{g}(p) = \min_{\Delta \beta}\;& \sum_{i=1}^{k-1} \underline{\pi}_{p_i} \Delta \beta_{p_i} \label{obj:lp} \\
    \text{s.t. }\;&  0 \leq \Delta \beta_{p_i} \leq B, \forall i \in \left\{ 1,...,k-1 \right\} \\
    & \beta_0 + \sum_{i=1}^{k-1} \Delta \beta_{p_i} \geq \sum_{i=1}^{k-1} C_{p_i p_{i+1}}\left(t^{ub}_{p_i p_{i+1}} \right) \label{cons:lp:soc}
\end{align} \label{prob:csso-lp}
\end{subequations}
Here, we replace the objective~\eqref{obj:spd} by its lower bound~\eqref{obj:lp} and reduce the complicated constraints in~\eqref{prob:csso} to a simple constraint~\eqref{cons:lp:soc}, which only require the overall energy charged to the battery is greater than or equal to the minimum energy consumption along the path $p$.
Note that the right hand side of~\eqref{cons:lp:soc} can be pre-computed and thus is a constant. Therefore, problem~\eqref{prob:csso-lp} can be easily solved by greedily allocate charged energy $\Delta \beta$ with minimum carbon intensity.
Meanwhile, we can show that $\underline{g}(p)$ is indeed a lower bound of $g(p)$ by the following Lemma.
\begin{lemma}
 $\forall p=[p_1,...,p_k]$ on graph $\csgpre{G}$, we have $\underline{g}(p) \leq g(p)$. 
\end{lemma}
\begin{proof}[Proof]
    Given a path $p=[p_1,...,p_k]$, for every feasible solution $\vec{t}, \vec{\beta}, \vec{\tau}$ of problem~\eqref{prob:csso}, we can compute a feasible solution in problem~\eqref{prob:csso-lp} :
    \begin{equation}
        \Delta \beta_{p_{i+1}} = \phi(t^c_{p_i p_{i+1}}, \hat{\beta}_{p_i}), \forall i \in \left\{ 1,...,k-1 \right\}
    \end{equation}
    which leads to a lower objective
    \begin{equation}
        \begin{aligned}
       \underline{g}(p) 
       & \leq \sum_{i=1}^{k-1} \underline{\pi}_{p_i} \Delta \beta_{p_i} \\
       & \leq  \sum_{i=1}^{k-1} F_{p_i p_{i+1}}\left(\hat{\beta}_{p_i} , t_{p_i p_{i+1}}^c, \tau_{p_{i}} + t^w_{p_i p_{i+1}} + t^c_{p_i p_{i+1}} \right)
        \end{aligned}
    \end{equation}
    This inequality holds for any feasible solution of problem~\eqref{prob:csso}. Therefore, we have $\underline{g}(p) \leq g(p)$.
    % This is true because every feasible solution of csso can be transformed to a feasible solution of csso-LP with lower objective value.
\end{proof}

% Overall, we provide a te
% Therefore, we can

% \noindent\textbf{Implementation Details.} 
% \begin{itemize}
%     \item The edge order of dfs.
% \end{itemize}

==> arxiv/4.admm.tex <==
\section{An ADMM Based Method}

One of the challenges of \textsf{CFO} lies in the coupling constraints~\eqref{cons:cfo:soc} and~\eqref{cons:cfo:tau} along the selected path. 
In this section, we use the splitting technique and leverage the idea from the alternating direction method of multipliers~(ADMM)~\cite{boyd2011distributed} to decouple the constraints. 
After decomposition, the update steps of ADMM can be easily tackled by solving a number of small-size subproblems and a shortest path problem.
In particular, we reformulate the \textsf{CFO} problem by introducing auxiliary variables $\vec{\beta'}$ and $\vec{\tau'}$.
\begin{align}
    \min_{
        \substack{
        \vec{\beta'} \in \mathcal{B} , \vec{\tau'} \in \mathcal{S},  \\
        \vec{\beta} \in \mathcal{B} , \vec{\tau} \in \mathcal{S},  \\
        \vec{t} \in \mathcal{T}, \vec{x} \in \mathcal{X} 
        }}
        \;& \sum_{(i,j)\in \mathcal{E}} x_{ij} F_{ij}(\beta_i, t_{ij}, \tau_i) \label{obj:cfop}  \\
    \text{s.t. }\;
    & x_{ij} \cdot \left( \beta_j' - \min \left\{ B,  \beta_i - c_{ij}(t_{ij}, \beta_i) \right\} \right)  = 0, \, \forall (i,j) \in \mathcal{E} \label{cons:cfop:soc} \\
    & x_{ij} \cdot \left(   \tau_j' - \tau_i - t_{ij} \right) = 0, \, \forall (i,j) \in \mathcal{E} \label{cons:cfop:tau} \\
    & x_{ij} (\beta_j - \beta_j') = 0, \forall (i,j) \in \mathcal{E} \label{cons:cfop:beq} \\
    & x_{ij} (\tau_j - \tau_j') = 0, \forall (i,j) \in \mathcal{E} \label{cons:cfop:taueq}
\end{align}
Here, we replace $\beta_j$ with $\beta_j'$ in the SoC constraint~\eqref{cons:cfop:soc} and replace $\tau_j$ with $\tau_j'$ in the traveling time constraint~\eqref{cons:cfop:tau}. We introduce additional constraints~\eqref{cons:cfop:beq} and~\eqref{cons:cfop:taueq} to make sure the auxiliary variables equal to the original variables along the selected path. 
The augmented Lagrangian is given by:
\newcommand{\gij}{g_{ij}(t_{ij}, \beta_i, \beta_j, \tau_i, \beta_j', \tau_j', \lambda_{ij}^\beta, \lambda^\tau_{ij}, \mu_{ij}^\beta, \mu_{ij}^\tau)}
\newcommand{\dualvec}{\vec{\lambda}^\beta, \vec{\lambda}^\tau, \vec{\mu}^\beta, \vec{\mu}^\tau}
\newcommand{\dualveck}{\vec{\lambda}^{\beta k}, \vec{\lambda}^{\tau k}, \vec{\mu}^{\beta k}, \vec{\mu}^{\tau k}}
\begin{align}
    &\mathcal{L}_{\rho}(\vec{t}, \vec{x}, \vec{\beta}, \vec{\tau}, \vec{\beta}', \vec{\tau}', \dualvec) = \nonumber \\
    &\sum_{(i,j)\in \mathcal{E}} x_{ij} \gij
\end{align}
where $\dualvec$ are the dual variables for the constraints \eqref{cons:cfop:soc}-\eqref{cons:cfop:taueq} respectively. The function $g_{ij}$ is given by
\begin{align}
     & \gij  = \\
     &F_{ij}(\beta_i, t_{ij}, \tau_i)  \label{gij:obj} \\
     &+ L_{\rho}(\lambda^\beta_{ij}, \beta_j' - \min \left\{ B,  \beta_i - c_{ij}(t_{ij}, \beta_i) \right\} ) \label{gij:lamb} \\
     &+  L_{\rho}(\mu^{\beta}_{ij}, \beta_j - \beta_j' ) \label{gij:mub}  \\
     & + L_{\rho}(\lambda^\tau_{ij}, \tau_{j}' - \tau_i - t_{ij} )
     + L_{\rho}(\mu^{\tau}_{ij}, \tau_j - \tau_j') \label{gij:tau}
      % + \mu^\tau_{ij} \left( \tau_i - \tau_i' \right)  + \frac{\rho}{2} \left( \tau_i - \tau_i' \right)^2
\end{align}
where auxiliary function $L\rho(\lambda, z)$ is given by
\begin{equation*}
    L_{\rho}(\lambda, z) = \lambda z + \frac{\rho}{2} z^2
\end{equation*}
where $\rho > 0$ is a penalty term for the equality constraints. An iteration of ADMM for solving problem~\eqref{obj:cfop} consists of the following steps:

1) path-update step 
\begin{align}
    &(\vec{x}^{k+1},\vec{\beta}'^{k+1},\vec{\tau}'^{k+1}) = \nonumber  \\
    & \qquad  \arg\min_{
        \substack{
        \vec{x} \in \mathcal{X}, \vec{\beta}' \in \mathcal{B}, \\ \vec{\tau}' \in \mathcal{S} 
        }}
        \mathcal{L}_{\rho}(\vec{t}^{k}, \vec{x}, \vec{\beta}^k, \vec{\tau}^k, \vec{\beta}', \vec{\tau}', \dualveck) \label{admm:pathupdate}
\end{align}

2) t-update step
\begin{align}
    &(\vec{t}^{k+1}, \vec{\beta}^{k+1},\vec{\tau}^{k+1}) = \nonumber  \\
    & \qquad  \arg\min_{
        \substack{
        \vec{t} \in \mathcal{T} , \vec{\beta} \in \mathcal{B}, \\
        \vec{\tau} \in \mathcal{S}
        }} 
    \mathcal{L}_{\rho}(\vec{t}, \vec{x}^{k+1}, \vec{\beta}, \vec{\tau}, \vec{\beta}'^{k+1}, \vec{\tau}'^{k+1}, \dualveck) \label{admm:tupdate}
\end{align}

3) dual-update step, for each $(i,j) \in \mathcal{E}$ such that $x^{k+1}_{ij}=1$
\begin{align}
    \begin{split}
    \lambda_{ij}^{\beta (k+1)} &= 
          \lambda_{ij}^{\beta k} + \rho \left(\beta_j'^{k+1} - \min \left\{ B, \beta_i^{k+1} - c_{ij}(t_{ij}^{k+1}, \beta_i^{k+1}   \right\}\right) \\
    \lambda_{ij}^{\tau (k+1)} 
        &= \lambda_{ij}^{\tau k} + \rho \left( \tau_j'^{k+1}  - \tau_i^{k+1} - t_{ij}^{k+1} \right) \\
    \mu_{ij}^{\beta (k+1)} &= \mu_{ij}^{\beta k} + \rho \left( \beta_j^k - \beta_j'^k \right) \\
    \mu_{ij}^{\tau (k+1)} &= \mu_{ij}^{\tau k} + \rho \left( \tau_j^k - \tau_j'^k \right) 
    \end{split}\label{admm:dualupdate}
\end{align}

% As compare to the method of multipliers, which 
% The path-update step and the t-update step can be treated as a single \emph{Gauss-Seidel} pass~\cite{boyd2011distributed} over the two sets of variables, which is a approximately
% Given the dual variables, instead of jointly optimize $L_{\rho}$ given 
The path-update step~\eqref{admm:pathupdate} and the t-update step~\eqref{admm:tupdate} can be treated as an inexact minimization step for the primal minimization of all the primal variables with given dual variables. Then the dual variables are updated in~\eqref{admm:dualupdate} by a simple dual ascent step with step size $\rho$.
The first two steps are still complicated at the first glance. 
However, as we will discuss later, both the path-update step and the t-update step can be efficiently solved by decomposing them into small subproblems. 
% Therefore, by splitting the coupled variables $\vec{\beta}$, $\vec{\tau}$ with auxiliary variables $\vec{\beta}'$, $\vec{\tau}'$, we develop an ADMM based algorithm whose iteration can be efficiently solved by solving decoupled subproblems. 
% Next, we will discuss details on how to solve the path-update step and t-update step.
% We first remark some overall observations here and then discuss how to solve the first two steps later.
% Finally, the dual-update step~\eqref{admm:dualupdate} is simply a dual ascent step with step size $\rho$.
% Therefore, both path-

\noindent
\textbf{Solution for path-update step.}
In the path-update step~\eqref{admm:pathupdate}, we optimize over the path $\vec{x}$ and the auxiliary variables $\vec{\beta}'$ and $\vec{\tau}'$. 
For each edge $(i,j)\in \mathcal{E}$, the value of $g_{ij}$ only depends on $\beta_j'$ and $\tau_j'$. Therefore, we can separately optimize the function $g_{ij}$ for each $(i,j)$ and then obtain the solution of the path-update step by solving a shortest path problem with the optimal value of $g_{ij}$ as the weight for each edge. 
In particular, for each edge $(i,j)\in \mathcal{E}$, we observe the relevant terms in $g_{ij}$. The objective term~\eqref{gij:obj} is constant with respect to $\beta_j'$ and $\tau_j'$. The following terms~\eqref{gij:lamb}-\eqref{gij:tau} is a quadratic function with respect to both $\beta_j'$ and $\tau_j'$. Therefore, we can obtain the optimal values of $g_{ij}$ by finding the minimal value of a quadratic function within a interval. Therefore, for each $(i,j) \in \mathcal{E}$, the solutions are given by
\begin{align}
    \begin{split}
    \tilde{\tau}_j'^{k+1} &= \frac{1}{2} \tau_j^{k} + \frac{1}{2} (\tau_i^{k} + t_{ij}^{k} ) + \frac{1}{2\rho} ( \mu_{ij}^{\tau k} - \lambda_{ij}^{\tau k} ) \\
    \tau_j'^{k+1} &=  \Pi(\tilde{\tau}_j'^{k+1},\, 0,\,T) \\
    \tilde{\beta}_j'^{k+1} &= \frac{1}{2} \beta_j^{k} + \frac{1}{2}  \min \left\{ B, \beta_i^k - c_{ij}^{k}(t_{ij}^{k}, \beta_i^{k}) \right\}  + \frac{1}{2\rho} ( \mu_{ij}^{\beta k} - \lambda_{ij}^{\beta k} ) \\
    \beta_j'^{k+1} &=  \Pi(\tilde{\beta}_j'^{k+1},\, 0,\,B) \\
    \end{split}
\end{align}
Here, the projection function $\Pi(x, l, u)$ projects the value of $x$ to the interval $[l,u]$, i.e.,
\begin{align}
    \Pi(x, l, u) = \left\{  
    \begin{aligned}
        &l,\, &\text{if}\; x &< l \\
        &x,\, &\text{if}\; l &\leq x \leq u \\
        &u,\, &\text{if}\; x &> u
    \end{aligned}
    \right.
\end{align}
By substituting the updated $\tau_j'^{k+1}$, $\beta_j'^{k+1}$ back to $g_{ij}$ we obtain the new weight for edge $(i,j)$. We can then use those computed weights to solve a shortest path problem and obtain the updated path selection variable $\vec{x}$. 

\noindent
\textbf{Solution for t-update step.}
In the t-update step~\eqref{admm:tupdate}, we optimize over the variables $\vec{t}$, $\vec{\beta}$, and $\vec{\tau}$. By exploring the structure of $\mathcal{L}_{\rho}$, we can solve this step by decomposing it into a number of small subproblems with three variables $t_{ij}$, $\beta_i$ and $\tau_i$. 
In particular, for each selected edge pair $(l,i)$,$(i,j)$ such that $x_{li}=1$ and $x_{ij}=1$, we solve the following subproblem:\footnote{To deal with the case where $i=s$ is the origin, we additionally $x_{0s}=1$ and $\mu_{0s} = 0$. Then the subproblem also needs to be solved for $l=0$ and $i=s$. with additionally constraint $\beta_s = \beta_0$ and $\tau_s = 0$.}

\begin{align}
    \min_{\beta_i, t_{ij}, \tau_i} \; &F_{ij}(\beta_i, t_{ij}, \tau_i)   \label{admm:tupdate:obj}
     \\ & + L_{\rho}(\lambda^\beta_{ij}, \beta_j'^{k+1} - \min \left\{ B,  \beta_i - c_{ij}(t_{ij}, \beta_i) \right\} )  \label{admm:tupdate:lamb}
     \\ & + L_{\rho}(\lambda^\tau_{ij}, \tau_{j}'^{k+1} - \tau_i - t_{ij} )
     \\ & +  L_{\rho}(\mu^{\beta}_{li}, \beta_i - \beta_i'^{k+1} )  
     + L_{\rho}(\mu^{\tau}_{li}, \tau_i - \tau_i'^{k+1}) \label{admm:tupdate:mu}  \\
     \text{s.t.} \;& 0 \leq \beta_i \leq B, \quad t_{ij}^{lb} \leq t_{ij} \leq t_{ij}^{ub}, \quad 0 \leq \tau_i \leq T
      % + \mu^\tau_{ij} \left( \tau_i - \tau_i' \right)  + \frac{\rho}{2} \left( \tau_i - \tau_i' \right)^2
\end{align}
Note that the objective function of the above is slightly different from function $g_{ij}$. We use the index $i$ instead of $j$ in the additive term~\eqref{admm:tupdate:mu} and change the corresponding dual variables. We make this adjustment to make sure the above subproblem only depends on the three variables $t_{ij}$, $\beta_i$ and $\tau_i$. 

The objective of the above subproblem~\eqref{admm:tupdate:obj}-\eqref{admm:tupdate:mu} may have different forms for different types of edges. For example, $F_{ij} \equiv 0$ for the non-charging edge $(i,j) \in \mathcal{E}_w \cup \mathcal{E}_r$ and $c_{ij} \equiv 0$ for the waiting edge $(i,j) \in \mathcal{E}_w$. Therefore, the subproblem can be largely simplified for non-charging edges. For the charging edges, however, we encounter a non-convex term $F_{ij}$ in the objective, making the subproblem more difficult to solve. 
Fortunately, the subproblem has only three variables within a finite box (if we additionally add a constraint $t_{ij} \leq T$). 
One straightforward method is the exhaustive grid search to find the global minimum of the above subproblem with complexity 
$O\left( \left( \frac{\max\{B,T\}}{\epsilon} \right)^3 \right)$ 
where $\epsilon$ is the accuracy tolerance. In practice, we can use better ways to divide the search domain via e.g., Branch and Bound (BnB) or the DIviding Rectangles (DIRECT) method~\cite{jones1993lipschitzian,gablonsky2001locally}. 

% \noindent
% \textbf{Termination Condition.}
% Unfortunately, the convergence of ADMM is not guaranteed for non-convex problem. 

\noindent
\textbf{Time Complexity.}
% We summarize our approach in Algorithm~xxx. 
Let $n=|\mathcal{V}|$ be the number of nodes and $m=|\mathcal{E}|$ the number of edges in the graph. The path-update step involves updating the weights for edge each edge with complexity $O(m)$ and solving a shortest path problem with negative weights. If we use Bellman-Ford algorithm~\cite{bellman1958routing}, the complexity is $O(mn)$. The complexity of the t-update step is
$O\left( m \left( \max\{B,T\}/\epsilon \right)^3 \right)$.
The complexity is $O(m)$ for the dual-update step. 
Therefore, the overall time complexity of one iteration is $O\left(mn+ m \left( \max\{B,T\}/\epsilon \right)^3\right)$.

\noindent
\textbf{Discussions.}

% Note that the augmented Lagrangian $\mathcal{L}_\rho$ is the sum of the product of the path selection variable $x_{ij}$ and corresponding weight $g_{ij}$. 





==> arxivSource/0.preamble.tex <==
\usepackage[utf8]{inputenc}
\usepackage{graphics} % Required for the inclusion of images
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{amsmath,amsfonts}
\usepackage{bbm, bm}
% \usepackage{subfigure}
\usepackage{subcaption}
\usepackage{listings}
\usepackage{hyperref}
\usepackage{pifont}
\usepackage{tabularx}
%\usepackage[ruled,linesnumbered]{algorithm2e}
\usepackage{algorithmicx}
\usepackage[noend]{algpseudocode}
\usepackage{algorithm}
\usepackage{tablefootnote}
\usepackage{float}
\usepackage{nicematrix}
\usepackage{tikz}
\usepackage{booktabs}
\usetikzlibrary{arrows}
\usetikzlibrary{positioning,matrix,calc}

\newcommand{\coo}{\ensuremath{\mathrm{CO_2}}} % https://tex.stackexchange.com/questions/480391/typing-co-2-easily
\newcommand{\trianglebullet}{$\mbox{\ensuremath{\rhd}}$}
\newcommand{\numsim}{$500$~} % The number of instances
\newcommand{\cfoa}{\textsf{CFO}_\alpha}
\newcommand{\multicell}[1]{\begin{tabular}[c]{@{}c@{}} #1 \end{tabular}}
\newcommand{\multicellleft}[1]{\begin{tabular}[l]{@{}l@{}} #1 \end{tabular}}

\ifodd 1
    \newcommand\rev[1]{{\color{red}#1}}
    \newcommand\revsu[1]{{\color{blue}#1}}
    \newcommand\outline[1]{{\color{brown}#1}}
    \newcommand{\com}[2]{\textbf{\color{blue} (COMMENT from [#1]: #2)}}
\else
    \newcommand\outline[1]{{#1}}
    \newcommand\revsu[1]{{#1}}
    \newcommand\rev[1]{{#1}}
    \newcommand\revr[1]{{#1}}
    \newcommand{\com}[2]{}
\fi




==> arxivSource/algs/approx-high-soc.tex <==

\begin{algorithm}[!tb]

    % \newcommand{\multiline}[1]{%
    %     \begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
    %       #1
    %     \end{tabularx}
    % }

    \caption{test$(s, d, \beta_0, T, \Omega, \epsilon_\beta, \epsilon_F)$}\label{alg:appro-high-soc-test}
    \begin{algorithmic}[1]
        % \SetInd{0.25em}{0.1em}
        \State $\delta_\beta \gets \frac{\epsilon_\beta B}{|V|+1}$, 
        $\underline{M}_{\beta} \gets - (|V|+1)$, 
        $\overline{M}_{\beta} \gets \lceil \frac{|V|+1}{\epsilon_\beta} \rceil$
        \State $\delta_F \gets \frac{\epsilon_F \Omega}{|V|+1}$, $M_F \gets \lceil \frac{|V|+1}{\epsilon_F}\rceil + |V| + 1 $
        \State $\psi \gets $ NULL
        \For{$i \gets \overline{M}_{\beta} \text{ to } \underline{M}_{\beta}, v \in V \cup \{s,d\}$ }
            \State $\psi' \gets \text{getMinT}(v,B,i\delta_\beta, \epsilon_\beta)$ 
            \State $\psi \gets \text{merge}(\psi', \psi)$
        \EndFor
        \State $\sigma(s,s,\cdot, \cdot, \cdot) \gets 0$
        \State $\sigma(s,v,\cdot, \cdot, \cdot) \gets \infty, \forall v \in V \backslash \{s\}$

        \For{$i_c \gets \overline{M}_{\beta} \text{ to } \underline{M}_{\beta}$,
        $i_v \gets \overline{M}_{\beta} \text{ to } \underline{M}_{\beta}$,
        $i_{ini} \gets \overline{M}_{\beta} \text{ to } \underline{M}_{\beta}$,}
        \For{$i_\rho \gets 1 \text{ to } M_F$,\, $i_F \gets 1 \text{ to } M_F$}
        \For{$u\in \cup \{s,d\},\, v \in V_c \cup \{s,d\}$}
            \State $\beta_c \gets i_c \delta_\beta$,
            $\beta_v \gets i_v \delta_\beta$,
            $\beta_{ini} \gets i_{ini} \delta_\beta$
            \State $\rho \gets i_\rho \delta_F$, 
            $\hat{F} \gets i_F \delta_F$, 
            % \State $t_c \gets \phi^{-1}(\beta_{ini}, \beta_c)$
            \State $t_c \gets \Phi_u^{-1}( \min\{ B, \beta_{ini} + \beta_c) \} - \Phi_u^{-1}(\beta_{ini})$
            \State $\tau \gets \psi(s, u, \beta_0, \beta_v)$
            \State $t_w \gets g_v(\beta_{ini}, t_c, \tau, \hat{F})$
            \State $t_r \gets \psi(u,v, \min \left\{ \beta_{ini} + \beta_c, B \right\}, \beta_v)$
            \State $\sigma_u \gets \sigma(s, u, \rho, \beta_0, \beta_{ini}) $
            \State $\tilde{\sigma} \gets \sigma_u + t_r + t_w + t_c $
            \State $\sigma_v \gets \sigma(s, v, \rho, \beta_0, \beta_v) $
            \If{ $\tilde{\sigma} \leq \sigma_v$ }
                \State $\sigma(s, v, \rho, \beta_0, \beta_v) \gets \tilde{\sigma}$
            \EndIf
        \EndFor
        \EndFor
        \EndFor
        % $\text{sol} \gets \text{NULL}$, 
        

        \State Let $i^*_\rho \in \left\{ 1,\cdots, M \right\}$ be the minimal $i_\rho$ such that $\sigma(s, d, i_\rho \delta_F, \beta_0, \lfloor \frac{\beta_{lb} -\epsilon B}{\delta_\beta}  \rfloor \delta_\beta ) \leq T $
        \If{$\rho^*$ exists}
            \State sol $\gets$ the solution corresponding to $\rho^*$
        \Else
            \State sol $\gets$ NULL
        \EndIf
        \State \Return sol
        
    \end{algorithmic}
\end{algorithm}

==> arxivSource/algs/approx-high.tex <==

\begin{algorithm}[!tb]

    % \newcommand{\multiline}[1]{%
    %     \begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
    %       #1
    %     \end{tabularx}
    % }

    \caption{solveCFO$(s,d,T,\beta_0, \epsilon)$ \textcolor{blue}{Not ready yet. This form of algorithm might be wrong...}}\label{alg:appro-high}
    \begin{algorithmic}[1]
        % \SetInd{0.25em}{0.1em}
        \State 
        % $\text{sol} \gets \text{NULL}$, 
        $\delta\gets\frac{\epsilon T}{|V|+1}$, $M\gets\lceil \frac{|V|+1}{\epsilon} \rceil + |V| + 1$
        \State $\rho(s,s, i\delta, \beta_0) \gets 0, \forall i \in \left\{ 1,...,M \right\}$
        \State $\rho(s,v, i\delta, \beta_0) \gets \infty, \forall i \in \left\{ 1,...,M \right\}, \forall v \in V \backslash \{s\}$
        \State $\beta_s \gets \beta_0$
        \State $\beta_v \gets -\infty, \forall v \in V \backslash \{s\}$
        \For{$i_c \gets 1$ to $M$, $i_w \gets 1$ to $M$, $i_{r} \gets 1$ to $M$, $i_{\tau} \gets 1$ to $M$}
            \State $t_c \gets i_c\delta,\, t_w \gets i_w\delta $
            \State $t_r \gets i_c\delta,\, \tau \gets i_{\tau}\delta $
            \If{$t_c \in [0, t_c^{ub}+\delta]$ and $t_w \in [t_w^{lb}, t_w^{ub}+\delta]$}
            \State $t_c \gets \min \left\{ t_c, t_c^{ub} \right\}$, $t_w \gets \min \left\{ t_w, t_w^{ub} \right\}$
            \For{$u \in \{s,d\} \cup V_c,\, v \in \{s,d\} \cup V_c $}
                \State $\tilde{\rho} \gets \rho(s, u, \tau, \beta_0) + F_u(\beta_u, t_c, \tau+t_w)$
                \State $\rho_{prev} \gets \rho(s, v, \tau + t_c + t_w + t_r)$
                \State { \Longunderstack[l]{$\tilde{\beta}\gets\beta(u,v,t_r,\beta_u+\phi(t_c,\beta_u))$ \\\; computed by calling Algorithm~\ref{alg:appro-low} \\\; with the same parameters and tolerance $\epsilon$}}.
                \If{$\tilde{\rho} < \rho_{prev} $ and $\tilde{\beta}\geq 0$}
                    \State $\rho(s,v,\tau+t_c+t_w,t_r) \gets \tilde{\rho}$
                    \State $\beta_v \gets \tilde{\beta}$
                \EndIf
                % \If{$t_e \in [t_e^{lb}, t_e^{ub}]$ }
                %     \State $\tilde{\beta} \gets \min\left\{ B, \beta(s,u, \tau, \beta_0) - c_e(t_e) \right\}$
                %     \If{$\tilde{\beta} \geq 0$}
                %         \State \Longunderstack[l]{$\beta(s,v,\tau+t_e,\beta_0)=$
                %         $\qquad\max\left\{\tilde{\beta},\beta(s,v,\tau+t_e,\beta_0)\right\}$%$\max\{\tilde{\beta},\beta(s,v,\tau+t_e, \beta_0)\}$
                %         % $  $
                %         }
                %     \EndIf
                % \EndIf
            \EndFor
            \EndIf
        \EndFor

        \If{\textcolor{blue}{TODO:}}
            \State sol $\gets$ the solution for ... % $\beta\left(s,d,(1+\epsilon)T_0,\beta_0\right)$
        \Else
            \State sol $\gets$ NULL
        \EndIf
        \State \Return sol
        
    \end{algorithmic}
\end{algorithm}

==> arxivSource/algs/approx-low-soc.tex <==

\begin{algorithm}[!tb]

    % \newcommand{\multiline}[1]{%
    %     \begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
    %       #1
    %     \end{tabularx}
    % }

    \caption{getMinT$(s,B_0,\beta_0, \epsilon)$}\label{alg:appro-low-soc}
    \begin{algorithmic}[1]
        % \SetInd{0.25em}{0.1em}
        % \State \textbf{Initialization Phase:} 
        % $\text{sol} \gets \text{NULL}$, 
        \State $\delta\gets\frac{\epsilon B_0}{|V|+1}$, 
        $\underline{M}\gets  -(|V| + 1) $, 
        $\overline{M}\gets \lceil \frac{|V|+1}{\epsilon} \rceil$
        \State  $\psi(s,s, \beta_0, i\delta) \gets 0, \forall i \in \left\{ \underline{M},...,\overline{M} \right\}$
        \State  $\psi(s,v, \beta_0, i\delta) \gets \infty, \forall i \in \left\{ \underline{M},...,\overline{M} \right\}, \forall v \in V \backslash \{s\}$
        \For{$i \gets \overline{M}$ to $\underline{M}$, }
            \For{$e = (u,v) \in E$}
            \For{$j \gets \lfloor \frac{c^{lb}_e}{\delta} \rfloor \text{ to } \lceil \frac{c^{ub}_e}{\delta} \rceil $}
                \State $\beta_u \gets i\delta, \hat{c} \gets j\delta$
                \State \begin{equation*}
                    % \setlength{\mathindent}{0pt}
                    % \hspace{-5mm}
                    t_e \gets \left\{  
                        \begin{aligned}
                            & t_e^{lb},& \text{if } j = \lceil \frac{c_e^{ub}}{\delta} \rceil, \\
                            & c_e^{-1}(\hat{c}), & \text{if } \hat{c} \in [c_e^{lb}, c_e^{ub}),  \\
                            & \infty, & \text{otherwise}.
                        \end{aligned}
                    \right.
                \end{equation*}
                \State $\beta_v \gets \min \{B, \beta_u - \hat{c}\}$
                \If{$ \beta_v \in [-\epsilon B, B]$}
                    \State $\tilde{\psi} \gets \psi(s, u, \beta_0, \beta_u) + t_e$
                    \State $\psi_{prev} \gets \psi(s, v, \beta_0, \beta_v) $
                    \State $\psi(s,v, \beta_0, \beta_f-\hat{c}) \gets \min \left\{ \tilde{\psi}, \psi_{prev}  \right\}$
                \EndIf
                % \If{$t_e \in [t_e^{lb}, t_e^{ub} + \delta]$ }
                %     \State $t_e \gets \min \left\{ t_e, t_e^{ub} \right\}$
                %     \State $\tilde{\psi} \gets \min\left\{ B, \psi(s,u, \tau, \beta_0) - c_e(t_e) \right\}$
                %     \If{$\tilde{\psi} \geq 0$}
                %         \State \Longunderstack[l]{$\psi(s,v,\tau+t_e,\beta_0)\gets$
                %         \\ $\qquad\max\left\{\tilde{\psi},\psi(s,v,\tau+i\delta,\beta_0)\right\}$%$\max\{\tilde{\beta},\beta(s,v,\tau+t_e, \beta_0)\}$
                %         % $  $
                %         }
                %     \EndIf
                % \EndIf
            \EndFor
            \EndFor
        \EndFor

        \State \Return $\psi$
        
    \end{algorithmic}
\end{algorithm}

==> arxivSource/algs/approx-low.tex <==

\begin{algorithm}[!tb]

    % \newcommand{\multiline}[1]{%
    %     \begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
    %       #1
    %     \end{tabularx}
    % }

    \caption{getMaxSoC$(s,T_0,\beta_0, \epsilon)$}\label{alg:appro-low}
    \begin{algorithmic}[1]
        % \SetInd{0.25em}{0.1em}
        % \State \textbf{Initialization Phase:} 
        % $\text{sol} \gets \text{NULL}$, 
        \State $\delta\gets\frac{\epsilon T_0}{|V|+1}$, $M\gets \left(   \lceil \frac{|V|+1}{\epsilon} \rceil + |V| + 1 \right)$
        \State  $\Omega(s,s, i\delta, \beta_0) \gets \beta_0, \forall i \in \left\{ 1,...,M \right\}$
        \State  $\Omega(s,v, i\delta, \beta_0) \gets - \infty, \forall i \in \left\{ 1,...,M \right\}, \forall v \in V \backslash \{s\}$
        \For{$i \gets 1$ to $M$, $j \gets 1$ to $M$}
            \For{$e = (u,v) \in E$}
                \State $t_e \gets i\delta, \tau \gets j\delta$
                \If{$t_e \in [t_e^{lb}, t_e^{ub} + \delta]$ }
                    \State $t_e \gets \min \left\{ t_e, t_e^{ub} \right\}$
                    \State $\tilde{\Omega} \gets \min\left\{ B, \Omega(s,u, \tau, \beta_0) - c_e(t_e) \right\}$
                    \If{$\tilde{\Omega} \geq 0$}
                        \State \Longunderstack[l]{$\Omega(s,v,\tau+t_e,\beta_0)\gets$
                        \\ $\qquad\max\left\{\tilde{\Omega},\Omega(s,v,\tau+i\delta,\beta_0)\right\}$%$\max\{\tilde{\beta},\beta(s,v,\tau+t_e, \beta_0)\}$
                        % $  $
                        }
                    \EndIf
                \EndIf
            \EndFor
        \EndFor

        % \If{$\beta\left(s,d,(1+\epsilon)T_0,\beta_0\right) \geq 0$}
        %     \State sol $\gets$ the solution for $\beta\left(s,d,(1+\epsilon)T_0,\beta_0\right)$
        % \Else
        %     \State sol $\gets$ NULL
        % \EndIf

        % \For{$k \gets 1$ to $K$}
        %     % \State Compute $\text{sol}^+$ with $\vec{\lambda}[k]$ by solving problem~\eqref{prob:dual} \label{alg:dualsub:primal}
        %     \If{$\delta_i^\beta[k] = 0$ and $\delta_i^\tau[k] = 0, \forall i\in \left\{ 1,...,N+1 \right\}$}
        %         \State \Return sol $\gets \text{sol}^+$  \label{alg:dualsub:optimal}
        %     \EndIf
        %     \If{$\delta_i^\beta[k] \leq 0$ and $\delta_i^\tau[k] \leq 0, \forall i\in \left\{ 1,...,N+1 \right\}$ \textbf{and} $\text{sol}^+$ has less objective }
        %         \State sol $\gets \text{sol}^+$ 
        %     \EndIf
        %     % \State $\hat{p} \gets \text{DFS}(\emptyset, p^\star, n)$
        %     % \If{$g(\hat{p}) < g(p^\star) $}
        %     %     \State $p^\star \gets \hat{p}$
        %     % \State Compute $\vec{\lambda}[k+1]$ according to~\eqref{eq:dualupdate}.
        % \EndFor
        \State \Return $\Omega$
        
    \end{algorithmic}
\end{algorithm}

==> arxivSource/algs/dfs.tex <==

\begin{algorithm}[htb]
    \caption{Iterative Deepening Approach}\label{alg:ida}
    \begin{algorithmic}[1]
        \State \textbf{Initialization:} $p^\star = \emptyset, N=|\csgpre{V}|$ \label{alg:ida:1}
        \For{$n \gets 2$ to $N$}
            \State $\hat{p} \gets \text{DFS}(\emptyset, p^\star, n)$
            \If{$g(\hat{p}) < g(p^\star) $}
                \State $p^\star \gets \hat{p}$
            \EndIf
        \EndFor
        \State \Return $p^\star$ \label{alg:ida:end}
        \State
        \Procedure{DFS}{$p$, $p^\star$, $n$} \label{alg:ida:dfs1}
            \If{$(|p| == n)$ and $(p_n == d)$ }
                \If{$g(p) < g(p^\star) $}
                    \State $p^\star \gets p$
                \EndIf
                \State \Return $p^\star$
            \EndIf
            \State $u \gets \text{tail}(p)$
            \For{ $\forall (u, v) \in \csgpre{E}$  }
                \State $p' \gets p \circ v$ 
                \If{TEST($p'$)}  \Comment{See Algorithm~\ref{alg:test}}
                    \State $p^\star \gets \text{DFS}(p', p^\star, n) $ 
                \EndIf
            \EndFor
            \State \Return $p^\star$
        \EndProcedure \label{alg:ida:dfsend}
    \end{algorithmic}
\end{algorithm}



==> arxivSource/algs/dualsub.tex <==

\begin{algorithm}[tb]
    \caption{A Dual Subgradient Method}\label{alg:dualsub}
    \begin{algorithmic}[1]
        \State \textbf{Initialization:} $\text{sol} \gets \text{NULL}$, $\vec{\lambda}[1] \gets 0$
        \For{$k \gets 1$ to $K$}
            \State Compute $\text{sol}^+$ with $\vec{\lambda}[k]$ by solving problem~\eqref{prob:dual} \label{alg:dualsub:primal}
            \If{$\delta_i^\beta[k] = 0$ and $\delta_i^\tau[k] = 0, \forall i\in \left\{ 1,...,N+1 \right\}$}
                \State \Return sol $\gets \text{sol}^+$  \label{alg:dualsub:optimal}
            \EndIf
            \If{$\delta_i^\beta[k] \leq 0$ and $\delta_i^\tau[k] \leq 0, \forall i\in \left\{ 1,...,N+1 \right\}$ \textbf{and} $\text{sol}^+$ has less objective }
                \State sol $\gets \text{sol}^+$ 
            \EndIf
            % \State $\hat{p} \gets \text{DFS}(\emptyset, p^\star, n)$
            % \If{$g(\hat{p}) < g(p^\star) $}
            %     \State $p^\star \gets \hat{p}$
            \State Compute $\vec{\lambda}[k+1]$ according to~\eqref{eq:dualupdate}.
        \EndFor
        \State \Return sol
        % \State
        % \Procedure{DFS}{$p$, $p^\star$, $n$} \label{alg:ida:dfs1}
        %     \If{$(|p| == n)$ and $(p_n == d)$ }
        %         \If{$g(p) < g(p^\star) $}
        %             \State $p^\star \gets p$
        %         \EndIf
        %         \State \Return $p^\star$
        %     \EndIf
        %     \State $u \gets \text{tail}(p)$
        %     \For{ $\forall (u, v) \in $  }
        %         \State $p' \gets p \circ v$ 
        %         \If{TEST($p'$)}  % \Comment{See Algorithm~\ref{alg:test}}
        %             \State $p^\star \gets \text{DFS}(p', p^\star, n) $ 
        %         \EndIf
        %     \EndFor
        %     \State \Return $p^\star$
        % \EndProcedure \label{alg:ida:dfsend}
    \end{algorithmic}
\end{algorithm}

==> arxivSource/algs/test.tex <==

\begin{algorithm}[htb]
    \caption{Candidate Test}\label{alg:test}
    \begin{algorithmic}[1]
        \Procedure{Test}{$p=[p_1,...,p_k]$, $p^\star$} 
        \If{ $\tilde{t}^{lb}(p) > T$} \label{alg:test:ddl}
            \State \Return false
        \EndIf
        \If{distance($p_k,d$) > distance($p_{k-1},d$)} \label{alg:test:distance}
            \State \Return false
        \EndIf
        \If{$\underline{g}(p) > g(p^\star)$} \label{alg:test:lb} \Comment{See~\eqref{prob:csso-lp}}
            \State \Return false
        \EndIf

        \State \Return true
           
        \EndProcedure 
    \end{algorithmic}
\end{algorithm}

==> arxivSource/arxiv/0.abstract.tex <==
\begin{abstract}
We study the carbon footprint optimization (CFO) of a heavy-duty e-truck traveling from an origin to a destination across a national highway network subject to a hard deadline, by optimizing path planning, speed planning, and intermediary charging planning.  Such a CFO problem is essential for carbon-friendly e-truck operations. However, it is notoriously challenging to solve due to (i) the hard deadline constraint, (ii) positive battery state-of-charge constraints, (iii) non-convex carbon footprint objective, and (iv) enormous geographical and temporal charging options with diverse carbon intensity. Indeed, we show that the CFO problem is NP-hard. As a key contribution, we show that under practical settings it is equivalent to finding a generalized restricted shortest path on a stage-expanded graph, which extends the original transportation graph to model charging options. Compared to alternative approaches, our formulation incurs low model complexity and reveals a problem structure useful for algorithm design. We exploit the insights to develop an efficient dual-subgradient algorithm that always converges. As another major contribution, we prove that (i) each iteration only incurs polynomial-time complexity, albeit it requires solving an integer charging planning problem optimally, and (ii) the algorithm generates optimal results if a condition is met and solutions with bounded optimality loss otherwise. Extensive simulations based on real-world traces show that our scheme reduces up to {28\%}  carbon footprint compared to baseline alternatives. The results also demonstrate that e-truck reduces 56\% carbon footprint than internal combustion engine trucks.
\end{abstract}
 % The formulation and algorithm are general and applicable to other electric mobility and energy storage management problems.

==> arxivSource/arxiv/0.preabmle.tex <==
\usepackage{amsthm}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}


%% To ensure 100% compatibility, please check the white list of
%% approved LaTeX packages to be used with the Master Article Template at
%% https://www.acm.org/publications/taps/whitelist-of-latex-packages 
%% before creating your document. The white list page provides 
%% information on how to submit additional LaTeX packages for 
%% review and adoption.
%% Fonts used in the template cannot be substituted; margin 
%% adjustments are not allowed.
%%
%%
%% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}




% \copyrightyear{2023} 
% \acmYear{2023} 
% \setcopyright{acmlicensed}\acmConference[e-Energy '23]{The 14th ACM
% International Conference on Future Energy Systems}{June 20--23,
% 2023}{Orlando, FL, USA}
% \acmBooktitle{The 14th ACM International Conference on Future Energy
% Systems (e-Energy '23), June 20--23, 2023, Orlando, FL, USA}
% \acmPrice{15.00}
% \acmDOI{10.1145/3575813.3595193}
% \acmISBN{979-8-4007-0032-3/23/06}


%%
%% Submission ID.
%% Use this when submitting an article to a sponsored event. You'll
%% receive a unique submission ID from the organizers
%% of the event, and this ID should be used as the parameter to this command.
%%\acmSubmissionID{123-A56-BU3}

%%
%% The majority of ACM publications use numbered citations and
%% references.  The command \citestyle{authoryear} switches to the
%% "author year" style.
%%
%% If you are preparing content for an event
%% sponsored by ACM SIGGRAPH, you must use the "author year" style of
%% citations and references.
%% Uncommenting
%% the next command will enable that style.
%%\citestyle{acmauthoryear}

%%
%% end of the preamble, start of the body of the document source.

==> arxivSource/arxiv/0.title.tex <==
\title{Follow the Sun and Go with the Wind:\\ Carbon Footprint Optimized Timely E-Truck Transportation}

\author{Junyan Su }
\affiliation{School of Data Science\\City University of Hong Kong 
  \institution{}
  \city{}
  \country{}
}

%\email{junyan.su@my.cityu.edu.hk}
\author{Qiulin Lin} % \\ School of Data Science\\City University of Hong Kong }
\affiliation{School of Data Science\\City University of Hong Kong
   \institution{}
   \city{}
   \country{}
}

\author{Minghua Chen}
\thanks{Corresponding author: Minghua Chen.}
\affiliation{%
  \institution{School of Data Science\\City University of Hong Kong}
  \city{}
  \country{}
}
%\email{minghua.chen@cityu.edu.hk}

% \author{Haibo Zeng}
% \affiliation{%
%   \institution{Electrical and Computer Engineering\\Virginia Tech}
%   \city{}
%   \country{}
% }
%\email{hbzeng@vt.edu}

%\renewcommand{\shortauthors}{Su and Chen}


% \begin{CCSXML}
% <ccs2012>
%    <concept>
%        <concept_id>10010405.10010481.10010485</concept_id>
%        <concept_desc>Applied computing~Transportation</concept_desc>
%        <concept_significance>500</concept_significance>
%        </concept>
%    <concept>
%        <concept_id>10002951.10003227.10003236</concept_id>
%        <concept_desc>Information systems~Spatial-temporal systems</concept_desc>
%        <concept_significance>300</concept_significance>
%        </concept>
%  </ccs2012>
% \end{CCSXML}
% 
% \ccsdesc[500]{Applied computing~Transportation}
% \ccsdesc[300]{Information systems~Spatial-temporal systems}
%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
% \keywords{electric truck, carbon footprint, timely transportation, }



==> arxivSource/arxiv/1.intro.tex <==

\section{Introduction}
% \com{MH}{perhaps follow the following logic flow more tightly to polish the intro: (i) trucking industry is essential, and decarbonizing it is critical for fighting climate change; (ii) e-truck is a promising endeavor with multi-facet benefits, including xxxx and reducing carbon emission; (iii) while e-truck produces no tailpipe emission on the road, it still incurs carbon footprint, which is balbala. (iii) in this paper, we study the carbon footprint optimization (CFO) of a heavy-duty e-truck traveling from an origin to a destination across a national highway network subject to a hard deadline, by optimizing path planning, speed planning, and intermediary charging planning.  Such a CFO problem is essential for maximizing the environmental benefit brought by e-trucks. However, it is notoriously challenging to solve due to the following challenges. (iv) discuss the four challenges: the hard deadline constraint,  positive battery state-of-charge constraints, non-convex carbon footprint objective, and enormous geographical and temporal charging options with diverse carbon intensity. (v) indeed, this important problem is more complicated and challenging than those in related studies for ICE truck and EV driving optimization and existing approaches are not directly appicable; see Sec. xx for more discussions. (vi) We carry out a comprehensive study for the CFO problem and make the following contributions: balbala}

In the United States, heavy-duty trucks deliver more than 10 billion tons of freight in 2021, representing 72.2\% of total domestic tonnage shipped. 80.4\% of the nation’s freight bills are from trucking which amounts to 875 billion US dollars~\cite{truckData2021}.
Despite their importance for the economy, heavy-duty trucks are a major source of Carbon Dioxide (\coo) emission, which is tied to climate change. With only $4\%$ of the total vehicle population, heavy-duty trucks produce  $25\%$ of the \coo\ emitted in the transportation sector, accounting for $8.8\%$ of the total carbon emissions in the US~\cite{davisTransportation2021}. To fight climate change, it is critical to de-carbonize the trucking industry.



Electrification of heavy-duty trucks is a promising endeavor with multi-facet benefits, including lower noise disturbance, better acceleration performance, better energy efficiency, and most notably, zero tailpipe emissions~\cite{bibra2022global} with great potential to de-carbonize the trucking industry.
However, while e-trucks do not generate direct \coo~emission during the operation, charging e-trucks incurs positive \emph{carbon footprint}, i.e., the \coo~emission during the production of electricity to be consumed by the e-truck. It is thus essential to evaluate the carbon footprint of e-trucks in contrast to the tailpipe emission for ICE trucks~\cite{zhou2020minimizing}.
% Indeed, e-trucks play a crucial role in de-carbonizing trucking industry as they are reported to be 51\%-67\% cleaner than ICE trucks in European Union~\cite{earl2018analysis}.
% \com{MH}{better to provide some concrete numbers with reference here to back up this statement.} 
{
% However, depending on the source of electricity (cf., Tab.~\ref{tab:fuel-co2}), charging e-trucks may still produce a significant amount of carbon emissions, which is the \emph{carbon footprint} of operating the e-trucks. 
% To unleash their full potential in decarbonization, it is essential to optimize the carbon footprint of e-trucks by considering the cleanness of the electricity.
% It is thus essential to optimize the carbon footprint of e-trucks to unleash their environment benefit.
}  
%while e-trucks do not generate direct \coo~emission during operation, it incurs positive \emph{carbon footprint} when charging, i.e., the \coo~emission during the production of electricity for charging the e-truck. %For example, suppose an e-truck charge at a charge station powered by a mix of energy sources (e.g., coal, natural gas, petroleum, and renewable). These energy resources are with different carbon-intensity (i.e., carbon footprint per unit electricity, unit: kg/kWh).  
%E-trucks are carbon-efficient only when charging at charging stations powered by a high penetration of renewable generations.
%in contrast to the tailpipe emission for ICE trucks~\cite{zhou2020minimizing}.}

\begin{figure}[!tb]
	\centering
	\includegraphics[width=\linewidth]{figs/varying-distri.pdf} 
    \vspace{-4mm}
	\caption{Spatial-temporal diversity of the carbon intensity~(kg/kWh) in the US~\cite{energyinformationadministrationeiaRealtime}. The whole country is divided to 13 regions. Each region includes one or multiple states. Carbon intensity is only provided for individual regions~\cite{energyinformationadministrationeiaRealtime}, thus one uniform color for all the states in a region.
    }%Left: different unit carbon footprint by regions; Right: time-varying unit carbon footprint due to fluctuating nature of the renewable.}
	\label{fig:price-distri}
\end{figure}

\input{tabs/co2-fuel.tex}


\begin{table*}[!tb]
    \centering
    % \resizebox*{\linewidth}{!}{
    %     \input{tabs/related-truck.tex}
    % }
    \input{tabs/related-truck.tex}
    %\input{tabs/related-ev.tex}
    \vspace{1mm}
    \caption{Model comparison between this work and the existing work for truck operations. 
    %$\dagger:$ ICET: internal combustion engine truck, \, BET: battery electric truck.
    }\label{tab:related-truck}
    \vspace{-0mm}
\end{table*}


In this paper, we study the carbon footprint optimization (CFO) of a heavy-duty e-truck traveling from an origin to a destination across a national highway network subject to a hard deadline, by exploring the complete design space of path planning, speed planning, and intermediary charging planning.  Such a CFO problem is central to maximizing the environmental benefit brought by e-trucks. However, it is notoriously challenging to solve due to the following.


\emph{The hard deadline constraint.} Transportation deadline is a common requirement in the trucking industry. In fact, timely delivery is not only necessary for perishable goods such as food~\cite{ashby1987protecting}, it is also commonly adapted in service-level agreements to guarantee delivery delay ~\cite{amazon}. Moreover, transportation tasks on online platforms (e.g., Uber Freight~\cite{uber}) are often associated with pickup/delivery time requirements, from which an end-to-end delivery deadline can be computed. Meanwhile, very often, considering deadline constraints can turn an easy problem, e.g., finding the fastest path between the origin and a destination, into an NP-hard counterpart~\cite{dengEnergyefficient2017}.

\emph{Positive battery State of Charge (SoC) constraints.}
Range anxiety is a common issue for e-trucks due to their limited capacity. Careful planning to prevent battery depletion for an e-truck is thus necessary during the transportation task. However, this requirement adds strong couplings to the traveling decisions between successive road segments, thus largely complicating the problem. 

% Due to the limited capacity of battery, an e-truck needs to avoid running out of battery during the trip. This requirement, while natural, adds strong couplings to the CFO problem and make it challenging to solve.
% Meanwhile, an e-truck may harvest energy with regenerative braking when traveling downhill.
% Meanwhile, an intermediary charging is often required for an e-truck with long-haul delivery tasks. 
% harvesting energy...

\emph{Non-convex carbon footprint objective.}
We consider an e-truck incurs the carbon footprint objective during intermediary charging.
End-use electricity often has a mix of different sources (e.g., coal, natural gas, petroleum, and renewable). Different sources have different carbon intensities (i.e., carbon footprint per unit electricity, unit: kg/kWh); see Tab.~\ref{tab:fuel-co2} for examples.
Among those sources, renewable have notable zero carbon intensity and thus is an eco-friendly type of source.
Meanwhile, renewable generation has a large variation in time and locations, resulting in spatial-temporal diversity of carbon intensity of electricity; see Fig.~\ref{fig:price-distri} for an illustration.
The diverse carbon intensity, along with the nonlinear charging characteristics of the battery, makes the carbon footprint objective non-convex and challenging to deal with.

% Therefore, charging with higher proportion of renewable is preferable for an e-truck to reduce the carbon footprint during a delivery task.
% which makes the carbon footprint objective non-convex with respect to time; 
% \textcolor{blue}{Need to revise later.}
% For example, as shown in Fig.~\ref{fig:price-distri}, the average carbon intensity is $0.87$ kg/kWh in California while $2.44$ kg/kWh in mid-east region. The carbon intensity also ranges from $0.5$ kg/kWh to $1.4$ kg/kWh during a week.
% Provided that recharging stops are often necessary for long-haul transportation for electric trucks due to their limited battery capacity,
% it is essential to decide recharging locations and moments by considering the spatial-temporal diversity of the renewable generation.

\emph{Enormous geographical and temporal charging options.}
Due to the fluctuating nature of the renewable, carbon intensity varies largely in both location and time. 
Jointly with path planning and speed planning, charging planning determines where and when to charge, how much to charge with diverse carbon intensity in different locations and time.
The design space is combinatorial in nature, with enormous options to consider, making the CFO problem uniquely challenging to solve.
% It is thus essential to jointly optimize path planning, speed planning, and intermediary charging planning in which path planning chooses greener charging stations, speed planning decides the moment of charging, and charging planning decides the charge amount and ensures feasibility.
% As reported in Sec~\ref{sec:simulation}, carbon-optimized planning saves 36\% carbon footprint as compared to baseline alternatives, indicating a significant potential for reducing the carbon footprint.
% However, joint consideration of those three design spaces leads to enormous decision spaces making CFO uniquely challenging to solve.

% To reduce the carbon footprint, the location and charging 
% \noindent\textbf{Contribution.}
% Overall, we make the following \textbf{contributions}: 
% \textcolor{blue}{Need to briefly remark challenges here.}
% a new objective \emph{carbon footprint} in timely e-truck transportation with recharging stops. 
%We propose a realistic model for a long-haul heavy-duty electric truck with recharging stops by optimizing path planning and speed planning. 
% Our work differentiates from existing studies in that the challenging objective is non-convex and depends on the previous path and speed decisions, making the existing methods inapplicable.

% \textcolor{blue}{}
%gives the electricity generation and resulting \coo\ emission for renewable and three major types of source. 
%For instance, Tesla announced a new model of battery electric truck Tesla Semi~\cite{teslaSemi} with a range of 500 miles.
%However, the \coo\ footprint will not really get reduced if the electricity is generated from fossil fuels. 
%In contrast, the carbon footprint of the electric truck can be higher than its internal combustion counterpart due to the transmission loss of the electricity~\cite{su2021Energy}.
%An electric truck is "green" only when the consumed electricity is derived from high proportion of clean source. If all the electricity is generated from the renewable, then the electric truck will have zero \coo\ footprint. 
%In addition, minimizing energy consumption does not lead to minimum \coo\ footprint. In contrast, as we will show in the experiments, bad planning of charging may cause higher \coo\ emission even if energy consumption is minimized. 

% In this paper, we study the Carbon Footprint Optimization (CFO) problem of minimizing the carbon footprint for a long-haul heavy-duty battery electric truck, traveling across the national highway network, with recharging stops under spatially and temporally varying renewable proportion, subject to a hard deadline constraint.

% \emph{Recharging stops} are often necessary for long-haul transportation for electric trucks due to the limited battery capacity. 
% We also need to consider the non-linearity of charging process with respect to time which is  a commonly adapted realistic model~\cite{baumShortest2019,montoyaElectric2017}. In practice, the charging rate is nearly linear until 80\% of the SoC. Then the charging rate decreases as SoC approaches the capacity limit, making the overall charging function concave~\cite{pelletier2017battery}.

% \emph{Path planning and speed planning} are thus critical to the charging decision, in which path planning chooses greener charging station and speed planning chooses charging time with higher renewable proportion. Meanwhile, a careful planning of the route and speed profile will lead to less energy consumption and thus less carbon footprint. 

Indeed, the CFO problem is more complicated and challenging than those in related studies for ICE truck and EV driving optimization and existing approaches are not directly applicable; see Sec.~\ref{sec:related} for more discussions. 
In this paper, we carry out a comprehensive study of the problem and make the following \textbf{contributions}: 

\trianglebullet 
% for CFO, which is built upon a key observation that significantly simplifies the problem. 
% We present a novel problem formulation of CFO  
We conduct the first study on \emph{carbon footprint optimization} (CFO).
We show that the problem is NP-hard. 
We then show that under practical settings, the CFO problem is equivalent to finding a generalized restricted shortest path on a stage-expanded graph, which extends the original transportation graph to incorporate charging options. 
Compared to alternative approaches, our novel formulation incurs low model complexity and reveals a problem structure useful for algorithm design.
% Building on this understanding, we then present a novel formulation that has low model complexity and reveals a problem structure useful for algorithm design.
% We compare our approach with three conceivable alternatives to demonstrate the novelty of our approach.

% Compared to alternative approaches, our formulation incurs low model complexity and reveals a problem structure useful for effective algorithm design.
% We compare our formulation with alternative approaches 
% and demonstrate that the formulation reveals a pro
% We present a novel subpath-based problem formulation for CFO and show that the problem is NP-hard. 
% Despite its novelty, the formulation is also insightful so that it allows us to tackle the four challenges by dualizing the constraints and decomposing the hard problem to several easier subproblems. 
% \textcolor{blue}{TODO:}

\trianglebullet 
We then exploit the structured insights from the formulation to develop an efficient dual-subgradient algorithm that always converges. 
We show that in our approach, each iteration only incurs polynomial-time complexity in graph size, albeit it requires solving an integer charging planning problem optimally.
We then further derive a condition under which our algorithm produces an optimal solution and a posterior performance bound when the condition is not satisfied.
% We prove that (i) each iteration only incurs polynomial-time complexity in graph size, albeit it requires solving a mixed-integer charging planning problem optimally, and (ii) the algorithm generates optimal results if a condition is met and solutions with bounded optimality loss otherwise.
% We thus design an efficient dual subgradient method by exploring the problem structure. Being a heuristic for a NP-hard problem, our approach has a favorable theoretical performance besides its outstanding empirical performance. In particular, we show that our iterative approach has polynomial time complexity per iteration, and always converges. Meanwhile, we derive a posterior performance bound and characterize a condition under which the produced solution is optimal.

\trianglebullet  
We carry out extensive numerical experiments using real-world traces over the US highway network to show the effectiveness of our approach in practice. 
The results show that our scheme reduces up to {28\%} carbon footprint as compared to a fastest-path alternative. 
We conduct a comparison between e-trucks and ICE trucks on their environmental impact. The results show that an e-truck achieves 56\% carbon reduction compared to its ICE counterpart.


==> arxivSource/arxiv/2.related.tex <==


\section{Related Work}\label{sec:related}


\textbf{Energy-Efficient Timely Transportation (E2T2).} E2T2 aims to find a path and its associated speed profile from an origin to a destination with minimum energy consumption, while satisfying a hard deadline~\cite{dengEnergyefficient2017,liuEnergyEfficient2018,xuRide2019}. It generalizes the NP-hard Restricted Shortest Path (RSP)~\cite{hassin1992approximation,lorenz2001simple,juttner2001lagrange} problem by introducing an additional design space of speed planing. 
E2T2 problem is first proposed in~\cite{dengEnergyefficient2017} and also shown to be NP-hard. E2T2 is then generalized to the scenario with multiple pickup/delivery locations with time windows in~\cite{liuEnergyEfficient2018}. Another extension of E2T2 has been studied in~\cite{xuRide2019}, where the driver can strategically wait at the rest area for better traffic condition. However, all these studies above are for conventional internal combustion engine (ICE) trucks. In this work, we study the problem for electric trucks with a new objective of minimizing the carbon footprint, imposing unique challenges to the problem due to the coupling nature of the State of Charge (SoC) constraints.
See Tab.~\ref{tab:related-truck} for a comparison of our work with related studies.

\textbf{Path and Speed Planning for Electric Vehicle} has long been an active research area. Path planning for EVs involves negative edge weights due to the regenerative system. 
Many variants of the RSP problem have been proposed for EVs by minimizing the energy consumption subject to a deadline~\cite{storandtQuick2012, liuConstrained2017,celaEnergy2014b}, or by finding the fastest path subject to the battery capacity limit~\cite{wangContextAware2013, baumShortest2019}. However, all these works only focus on path planning and ignore the design space of speed planning. More recent works consider both path planning and speed planning~\cite{baumModeling2020, baumSpeedConsumption2014, fontanaOptimal2013, hartmannEnergyEfficient2014,strehler2017energy}. 
For example, Baum et al.~\cite{baumModeling2020} seeks to find the fastest path with capacity limit by optimizing both path planning and speed planning for EVs without charging stops by the tradeoff function propagating technique. Strehler et al.~\cite{strehler2017energy} give theoretical insights to the path and speed planning problem for EVs and provide a fully polynomial time-approximation scheme (FPTAS) for the problem. Overall, all mentioned work and their approaches either do not apply to the CFO problem or incur large time complexity in the CFO problem; see also Table~\ref{tab:related-method} and Appendix~\ref{sec:novelty} for a comparison of conceivable approaches.
% Overall, all mentioned works above only consider the objective of time or energy, while a non-trivial objective \emph{carbon footprint} is considered in this work. The new objective is not only important to the environment, but also imposes new challenges to the problem.

\textbf{Variants of Vehicle Routing Problem (VRP).} VRP generalizes the NP-hard traveling salesman problem (TSP), where the operator has a fleet of vehicles to fulfill the requirement of a set of customers. The variants of VRP for EV are considered in
electric vehicle routing problem (EVRP)~\cite{schneiderElectric2014,goekeRouting2015,desaulniersExact2016,montoyaElectric2017}. 
Some other variants of VRP consider the environmental impacts of the routing decisions. For example, the green vehicle routing problem~\cite{erdougan2012green} considers VRP for alternative fuel vehicles.
The pollution routing problem~\cite{bektasPollutionRouting2011} considers minimizing the emission for conventional vehicles. 
The electric arc routing problem (eARP)~\cite{fernandez2022arc} considers minimizing the total travel time on an energy-indexed graph.
As a general observation, variants of VRP only consider path planning and are very complex. The existing methods for VRP do not scale to large-scale network. 
%Meanwhile, to our best knowledge, our objective carbon footprint
%For example, there are many variants of the vehicle routing problem (VRP) for EVs, namely the electric vehicle routing problem

%\subsection{Green Effort}
%How significant is minimizing CO2? How popular is the topic?

% \subsection{Other Work}
% \begin{itemize}
% 	\item Variants of the vehicle routing problem (VRP). However, approaches in this area does not scale to large road networks.
% 	\begin{itemize}
% 		\item The pollution routing problem~\cite{bektasPollutionRouting2011} considers minimizing the emission for the conventional vehicles.
% 		\item The electric vehicle routing problem (EVRP)~\cite{schneiderElectric2014,goekeRouting2015,desaulniersExact2016,montoyaElectric2017}
% 	\end{itemize}
% \end{itemize}

==> arxivSource/arxiv/3.prob.formulation.tex <==

\begin{figure}[!tb]
	\centering
	\includegraphics[width=0.9\linewidth]{figs/chargeFunc1.pdf}
    \vspace{-4mm}
	\caption{An example of charging function $\Phi$, and the corresponding SoC difference function $\phi$. The initial SoC is $\beta_v=0.67$. After charging for $20$ minutes, %the final SoC is $\beta_v'=0.92$. 
  the increment of SoC $\phi(t_{c}, \beta_i)=0.25$. The two dashed lines represent charging functions for different charging schemes.}
	\label{fig:charge}
    % \vspace{-10mm}
\end{figure}


\section{Problem Formulation}

\subsection{System Model}


\textbf{Transportation Graph and Energy Consumption.}
% We consider an electric truck running on a road network. 
We model the highway system as a directed graph $ \mathcal{G} = (\mathcal{V}, \mathcal{E}) $ where $\mathcal{V}=\mathcal{V}_r \cup \mathcal{V}_c$ is the set of nodes. 
Here $\mathcal{V}_r$ denotes the nodes for real road segments and $\mathcal{V}_c$ denotes the nodes for the charging stations.
We denote $\mathcal{E} \subset \mathcal{V} \times \mathcal{V}$  the set of edges. 
For each road segment $e \in \mathcal{E}$, we denote its length by $D_{e}$  and  its minimum (resp. maximum) speed limit by $R^{lb}_{e}$ (resp. $R^{ub}_{e}$). We define the minimum and maximum traveling time limit as $t_e^{lb}=D_e/R^{ub}_e$ and $t_e^{ub}=D_e/R^{lb}_e$.


% The energy consumption of an e-truck depends on many factors. In this paper, we consider a specific e-truck traveling across a national highway system. 

Without loss of generality, we assume homogeneous road condition on a road segment $e \in \mathcal{E}$, e.g., the road grade. Given the weight of an e-truck and the road grade, we model its energy consumption rate over a road segment $e\in \mathcal{E}$ as a convex function of the traveling speed as justified in~\cite{dengEnergyefficient2017}: %\textcolor{blue}{TODO: Add a plot of $f$}. 
$f_{e}(r_{e}): [R_{e}^{lb}, R_{e}^{ub}] \rightarrow \mathbb{R}$ (unit: kilowatts), where $r_e$ is the traveling speed. Note that for e-trucks, $f_{e}$ can take negative values over (downhill) road segments because of  regenerative breaking~\cite{baumShortest2019}. 
Because of the convexity of $f_{e}(\cdot)$, it suffices to assume that the e-truck travels on the road segment at constant speed~\cite[Lem. 1]{dengEnergyefficient2017} with no optimality loss.\footnote{{We ignore the acceleration/deceleration stage between road segments, as it usually occupies a small fraction of time/energy compared with that under the entire road segment.}} %takes less than 20 seconds (or several hundred meters long) for e-trucks~\cite{teslaSemi} while comparing with road segments for several miles, e.g., 3 miles on average  in the US highway system.}
We further define an \emph{energy consumption function} for an e-truck to traverse the road segment $e$ as $c_e(t_e) = t_e\cdot f_e(D_e/t_e)$. We note that $c_e(\cdot)$ is a perspective function of $f_e(\cdot)$ with linear transformation. As such $c_e(t_e)$ must be convex in $t_e$~\cite{boyd2004convex}.

%We assume that the time and energy consumption during the acceleration/deceleration stage are negligible, as it usually takes less than 20 seconds (or several hundred meters long) for e-trucks~\cite{teslaSemi} while they travel on road segments for several miles, e.g., 3 miles on average  in the US highway system.

% and the regenerative breaking system can recuperate energy with high efficiency. 
% \com{MH}{revise; refer to previous papers from the group on similar justification.}
% this stage is usually only several hundred meters long, and the corresponding time and fuel consumption are negligible compared to those of traveling along one road segment which is usually several miles long.

\textbf{E-Truck Charging.}
For each charging station node $v \in \mathcal{V}_c$, an e-truck can make two decisions: wait for $t_w \in [ {t}_w^{lb}, t_w^{ub} ]$ amount of time for lower carbon intensity and charge for $t_c \in [0, t_c^{ub}]$ amount of time. Here we use ${t}_w^{lb}$ to denote the time overhead for an e-truck driver to stop and pay bills, etc.
We denote the charging function at $v\in \mathcal{V}_c$ by a concave function $\Phi_{v}(t)$, which represents the charged SoC from zero after we charge for $t$ amount of time.\footnote{{Most e-trucks use lithium-ion batteries, which are often charged with the constant-current constant voltage (CC-CV) scheme~\cite{pelletier2017battery}. In the scheme, a battery is first charged by a constant current, and the SoC increases linearly until  $\sim$80\% of the capacity. After that, a constant voltage is held to avoid overcharging degradation, causing the current to decrease and the SoC to increase concavely.}} Given an initial SoC $\beta_v$  we can compute the increment of SoC after a charging time $t_c$ as % (see Fig.~\ref{fig:charge} for an illustration)
\begin{equation}
\phi_{v}(t_c, \beta_v) = \Phi_{v}(\Phi^{-1}_{v}(\beta_v) + t_{c}) - \beta_{v}. \label{eq:soc_difference_function}
\end{equation}
Here, $\Phi_v^{-1}$ is the inverse function of $\Phi_v$; see Fig.~\ref{fig:charge} for an illustration.
% We provide an illustration in Fig.~\ref{fig:charge}.

%\com{ql}{to edit. } Most of the battery electric trucks use lithium-ion battery as their energy storage systems, and they are often charged with the constant-current constant voltage (CC-CV) scheme~\cite{pelletier2017battery}. In the CC-CV scheme, the battery is first charged by a constant current. Thus SoC increases linearly with time until approximately 80\% of the SoC value. Then in the CV stage, a constant voltage is held to avoid overcharging degradation, causing the current to decreases and the SoC to increase concavely. See Fig.~\ref*{fig:cccv} for an illustration.
% In this paper, we assume the charging function to be increasing and concave, which covers the piece-wise linear model and the exponential model~\cite{liu2014joint} in the literature. 

{There could be multiple charging modes for e-trucks, e.g.,  fast charge and regular charge, which correspond to different charging functions (c.f. Fig.~\ref*{fig:charge}). Here, for simplicity, we assume the e-truck only applies the fast charging scheme at each charging station. We note that our approach can be easily extended to take multiple charging schemes into account. For example, we can model different charging schemes at a charging station by adding multiple charging nodes $i \in \mathcal{V}_c $ at the same location.}
%Here, we assume that an e-truck driver will always use the maximum charging rate limit and thus each charging station $e \in \mathcal{V}_c$ only has one specific charging function. This is because there is little benefit for an electric truck to charge below the rate limit.
%%e.g. Fig.~\ref{fig:charge} for an example.
%%\textcolor{blue}{charging rate limit?}
%Note that the charging function can be different at different charging station node $v \in \mathcal{V}_c$ so we can model different types of charging schemes (e.g., fast charge and regular charge, c.f. Fig.~\ref*{fig:charge}). We can also model different charging schemes at the same charging station by adding multiple charging nodes $i \in \mathcal{V}_c $ at the same location.



\textbf{Carbon Intensity and Carbon Footprint.} 
%We consider a 
For each charging station $v \in \mathcal{V}_c$,
% edge $(i,j) \in \mathcal{E}_c$, 
we define a continuous carbon intensity function $\pi_{v}(\tau)$ (unit: kg/kWh)
where $\tau$ is the arrival time instant at node $v$. We assume $\tau_0=0$ at the origin $s$ for ease of the presentation.
As illustrated in Fig.~\ref*{fig:price-distri}, the carbon intensity function $\pi_{v}(\cdot)$ largely varies in locations and time due to the geographical and temporal variation of the renewable generation. 
We note that the carbon-intensity information can be well forecasted at the hourly scale~\cite{majiDACF2022}.
% We remark that the function $\pi_v(\cdot)$ is in a general form. 
% We can write it as a combination of the carbon intensity and the monetary price $\pi_{v} = \pi_{v}^{c} + \gamma \pi_{v}^{m}$ with some weighting factor $\gamma > 0$, thus our model and approach are also applicable to other general scenarios like minimizing monetary cost with time-varying electricity prices.
Given the carbon intensity function $\pi_{v}(\cdot)$, if the e-truck with initial SoC $\beta_v$ starts charging at $\tau_v$ at station $v$ and charges $t_c$ time, the induced carbon footprint is 



\begin{align}
    F_{v}(\beta_v, t_{c}, \tau_v) = 
    \frac{1}{\eta} \int_{0}^{t_{c}} \pi_{v}(\tau_v + \xi) \frac{\partial_{-} \phi_{v}}{\partial t} (\xi, \beta_v) d\xi. \label{eq:carbon-footprint}
    % F_{v}(\beta_v, &t_{c}, \tau_i) = \nonumber \\
    % & \left\{  
    % \begin{aligned}
    % &\frac{1}{\eta} \int_{0}^{t_{c}} \pi_{v}(\tau_v + \xi) \frac{\partial_{-} \phi_{v}}{\partial t} (\xi, \beta_v) d\xi, &  (i,j) \in \mathcal{E}_c & \\
    % & 0, & (i,j) \in \mathcal{E}_r \cup \mathcal{E}_w &
    % \end{aligned}
    % \right.
\end{align}
Here, $ 0<\eta \leq 1$ is the charging efficiency of the battery. $\frac{\partial_{-} \phi_{v}}{\partial t}(\xi, \beta)$ is the left partial derivative with respect to $t$, which denotes the charging rate given the charging time $\xi$ and initial SoC $\beta$.
% \textcolor{blue}{TODO: add some explaination according to Reviewer A.}
%as the charging function $\Phi$ can be modeled by a piece-wise linear function~\cite{baumShortest2019}. 
For charging at station $v \in \mathcal{V}_c$, the carbon footprint depends on the initial SoC $\beta_v$, the charging time $t_{c}$ and the arrival time $\tau_v$. It is the integral of the product of the price function and charging rate and thus nonlinear and non-convex (see an example in Fig.~\ref{fig:obj}).


\subsection{Carbon Footprint Optimization Problem}
%In this section, we first discuss the design space of the problem and its formulation, after which we illustrate the novelty and key challenges. .

We study the problem of minimizing the carbon footprint of an e-truck traveling from the origin $s \in \mathcal{V}$ to the destination $d\in \mathcal{V}$, subject to the hard deadline $T$ and the SoC constraints. We consider that the e-truck with initial SoC $\beta_0$ and battery capacity $B$ can take at most $N$ charging stops during the trip. We assume $N$ is a given parameter to our problem. In practice, it is reasonable to limit the number of charging stops in a trip for a good experience. The number is usually small, e.g., 3 or 4 for a 1500-mile e-truck transportation. In our simulation, we set the number of charging stops to be no more than eight. 

\begin{figure}[!tb]
    \centering
    % \includegraphics[width=0.8\linewidth]{figs/CFO4.pdf}
    \includegraphics[width=.95\linewidth]{figs/stage-expended/stage-expended.pdf}
    \vspace{-3mm}
    % \caption{An example of stage-expanded graph with $N=1$ charging stop. Here, $u,v$ are two charging stations in the original transportation graph. There are two stages, each stage corresponds to a sub-path and a charging station (or destination) at the end of the subpath. The charging process only happens between two stages. The red line shows a feasible path in the stage-expanded graph.} \label{fig:ex-subpath}
    \caption{
        An example of stage-expanded graph with $N=2$ charging stops. Here, node $b,c,e$ are charging stations in the original transportation graph. % There are $3$ stages. At each stage, the e-truck travels towards the next charging station (or the destination), then wait and charge at the charging station and enter the next stage or stop at the destination.
    } 
    \label{fig:ex-subpath}
    % \vspace{-10mm}
\end{figure}

\textbf{A Stage-Expanded Graph.}
% \textcolor{blue}{TODO:}
One of the challenges for formulating the CFO problem is the lack of the arrival time information and the arrival SoC information in the original transportation graph $\mathcal{G}$. Those information are essential for objective evaluation in the charging planning. 
To incorporate those information and mitigate this challenge, we consider a \emph{stage-expanded graph}, which extends the original transportation graph to model the charging decisions. % \textcolor{blue}{Need to polish.}
% To prevent battery depletion and optimize the path, we need to keep track of the SoC and the arrival time at a charging station to determine the corresponding SoC increment in~\eqref{eq:soc_difference_function}
% \com{ql}{a better name for the function.} 
% and carbon footprint function in~\eqref{eq:carbon-footprint}. However, it is nontrivial to model the order of the charging stops in a path on the transportation graph $\mathcal{G}$, and it prevents us from determining the SoC and arrival time. Here, we consider a \emph{stage-expanded graph}, which extends the original transportation graph to model the charging decisions. 

In particular, we consider a stage-expanded graph $\mathcal{G}_{s}=(\mathcal{V}_s, \mathcal{E}_s)$ with $N+1$ stages. Here $\mathcal{V}_s$ contains $N+1$ copies of original node, i.e.,
$\mathcal{V}_s = \left\{ v^i : v \in \mathcal{V}, i \in \left\{ 1,...,N+1 \right\}  \right\}$. The edge set $\mathcal{E}_s$ keeps the original edges with additional connection between the same charging stations and destinations for two adjacent stages. That is, 
\begin{align*}
    \mathcal{E}_s  = & \left\{ (u^i, v^i) : (u,v) \in \mathcal{E}, i \in \left\{ 1,...,N+1 \right\} \right\}  \\
     & \cup \left\{ (v^i,v^{i+1}) : v \in \mathcal{V}_c \cup \left\{ d \right\}, i \in \left\{ 1,...,N \right\}  \right\}.
\end{align*}
When an e-truck at stage $i$ decides to charge at a charging station $v \in \mathcal{V}_c$, we model it travels through a virtual stage transition edge $(v^i,v^{i+1})$. 
At each stage, the e-truck travels towards the next charging station (or the destination), then wait and charge at the charging station and enter the next stage or stop at the destination.
Note that the e-truck can charge less than $N$ times, arrive the destination at stage $i<N+1$ and then travel across stages through virtual edges between destinations and arrive the final stage.
We provide an illustration in Fig.~\ref{fig:ex-subpath}. 
% The stage transition happens when an e-truck decides to charge at charging station $v \in \mathcal{V}$.
% At each of the first $N$ stages, we determine one charging stop and the subpath for traveling to the stop. And the last stage is to travel from the last charging stop to the destination.  

As we shall see in the following, 
the stage-expanded graph naturally incorporates the information of the arrival time and the arrival SoC, making it easier to model the charging decisions.
We shall also discuss the benefits of such a stage-expanded graph and compare it conceivable alternatives later in Sec.~\ref{sec:challenge} after we formulate the CFO problem.
% It naturally provides the information of the order of the charging stops and makes it easy to compute SoC and arrival time at each charging stop. 
% To this end, we formulate the problem as finding a generalized restricted shortest path on such a stage-expanded graph. 
% We note that our formulation is novel and reveals the problem structure that will facilitate the algorithm design in the next section. Please refer to our discussion in Sec.~\ref{sec:challenge} and see a comparison with alternative approaches in Table~\ref{tab:related-method}.


\textbf{Path and Charging Station Selection.}
%  \textbf{Decision Variables and Simple Constraints.} 
{A path in the stage-expanded graph consists of $N+1$ subpaths connecting the source, no more than $N$ charging stations and the destination. We use binary variables to represent the choice of charging stops at each stage and road segments in each subpath. } %We define decision variables regarding path planning and speed planning on the subpath at each stage

 In particular, for each charging station $v\in \mathcal{V}_c$, we define a binary charging station selection variable $y_v^i \in \left\{ 0,1 \right\}$ and $y_v^i=1$ means we want to choose charging station $v$ as our $i$-th charging stop. For each subpath $i \in \left\{ 1,...,N+1 \right\}$ and road segment $e\in \mathcal{E}$, we define a binary path selection variable $x_e^i \in \left\{ 0,1 \right\}$ and $x_e^i=1$ means we want to travel through road segment $e$ for $i$-th subpath. 
For ease of presentation, we stack the variables 
$\vec{x}^i=\{ x_e^i \}_{e \in \mathcal{E}}$, $\vec{x}=\{ \vec{x}^i \}_{i=1}^{N+1}$ and
$\vec{y}^i=\{ y_e^i \}_{e \in \mathcal{E}}$, $\vec{y}=\{ \vec{y}^i \}_{i=1}^{N+1}$. We define the feasible set of $(\vec{x}, \vec{y})$ as follows:

\begin{subequations}
    \begin{align}
        \mathcal{P} =  \Biggl\{
            & \left( \vec{x}, \vec{y} \right) |\, 
            x_e^i \in \left\{ 0,1 \right\},\ \forall e \in \mathcal{E}, i \in \left\{ 1,...,N+1 \right\} \\
            & y_v^i\in \left\{ 0,1 \right\},\forall  v\in \mathcal{V}, i \in \left\{ 0,...,N+1 \right\} \\
            & \sum_{e \in \text{Out}(v) } x_e^i - \sum_{e \in \text{In}(v) } x_e^i = y_v^{i-1} - y_v^i, \, \forall  v \in \mathcal{V}, i\in\left\{ 1,...,N+1 \right\} \label{eq:pathset:flow} \\
            & \sum_{v\in \mathcal{V}} y_v^i =1, \sum_{v \in \tilde{\mathcal{V}}_c  } y_v^i = 1, \, \forall i \in \left\{ 0,1,...,N+1 \right\} \label{eq:pathset:cs} \\
            & y^0_s = 1, y_d^{N+1} = 1 \label{eq:pathset:bound}
            \Biggr\}.
    \end{align}
\end{subequations}



%%%%%%%% illustration of the stage-based grapha%%%%%%%%%%%%%%%%%%%
% \begin{figure}[!tb]
%     \input{figs/ex-subpath.tex}
%     \vspace*{-1mm}
%     \caption{An example of sub-paths for $N=2$ charging stations.} \label{fig:ex-subpath}
%     \vspace*{-5mm}
% \end{figure}

% \begin{figure}[!tb]
%     \centering
%     \includegraphics[width=\linewidth]{figs/CFO.pdf}
%     \caption{An example...}
%     \label{fig:my_label}
% \end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Here, $\tilde{\mathcal{V}}_c = \mathcal{V}_c \cup \{s,d\} $. Out($v$) and In($v$) are the set of outgoing and incoming edges of node $v$, respectively. Constraint~\eqref{eq:pathset:flow} is the flow conservation requirement for each subpath. Constraint~\eqref{eq:pathset:cs} ensures that only one charging station is selected for each stage. Constraint~\eqref{eq:pathset:bound} defines that boundary case at the origin $s$ and the destination $d$. We remark that  $\mathcal{P}$ also covers path with charging stops less than $N$ as we can choose the same charging stops at adjacent stages.
% and time decision $t_e^i \in [t^{lb}_e, t^{ub}_e]$. Here, 
% Besides, for each charging station $v\in \mathcal{V}_c$, we also define a binary charging station selection variable $y_v^i \in \left\{ 0,1 \right\}$ and $y_v^i=1$ means we want to choose charging station $v$ as our $i$-th recharging stop. We denote by $t_w^i, t_c^i$ the waiting time and charging time at $i$-th recharging stop respectively. We also denote by $\beta_v^i, \tau_v^i$ the initial SoC and the moment we enter the $i$-th recharging stop, respectively. Fig.~\ref{fig:ex-subpath} gives an example with $N=2$ recharging stops.

\textbf{Speed and Charging Planning.}
We then define the decision variables for speed planning and charging planning. For each subpath $i$ and road road segment $e$, we denote the traveling time as $t_e^i$. We also denote by $t_w^{i,v}, t_c^{i,v}$ the waiting and charging time for charging station $v$ as $i$-th charging stop.
We also stack the variables as 
$\vec{t}^i=\left\{ t_e^i \right\}_{e\in \mathcal{E}}$, 
$\vec{t}_w^i=\left\{ t_w^{i,v} \right\}_{v\in \tilde{\mathcal{V}}_c}$, 
$\vec{t}_c^i=\left\{ t_c^{i,v} \right\}_{v\in \tilde{\mathcal{V}}_c}$, 
$\vec{t}=\left\{ \left( \vec{t}^i, \vec{t}^i_w, \vec{t}^i_c \right)  \right\}_{i=0}^{N+1}$. The corresponding feasible set is given by
\begin{subequations}
\begin{align}
    \mathcal{T} = \Biggl\{ 
        \vec{t}\,|\, &t_e^i \in [t_e^{lb}, t_e^{ub}], \forall e\in \mathcal{E}, i \in \left\{ 1,...,N+1 \right\},  \\
        &t_w^{i,v} \in [t_w^{lb}, t_w^{ub}], t_c^{i,v} \in [0, t_c^{ub}], \forall v \in \tilde{\mathcal{V}}_c, i \in \left\{ 1,...,N \right\}, \\
        & t_w^0 = t_c^0 = 0, 
    \Biggr\}.
\end{align}
\end{subequations}




\textbf{Time Constraints.} We denote $\tau_v^i$ the moment of an e-truck entering the charging station $v$ at $i$-th stop. It enables us to allocate the total allowed travel time $T$ to the subpath at each stage. We also stack the variable as $
\vec{\tau}=\left\{ \tau_v^i \right\}_{v\in \tilde{\mathcal{V}}_c, i\in \left\{ 0,...N+1 \right\}}$ and its feasible set is given by


\begin{align}
    % \mathcal{T}_\tau = \Biggl\{  \vec{\tau} \,|\,  &\tau_v^i \in [0, T], \forall v \in \tilde{\mathcal{V}}_c, i \in \left\{ 0,...,N+1 \right\}, \tau_d^{N+1} \leq T \label{cons:tau:bound}
    \mathcal{T}_\tau = \Biggl\{  \vec{\tau} \,|\,  &\tau_v^i \in [0, T], \forall v \in \tilde{\mathcal{V}}_c, i \in \left\{ 0,...,N+1 \right\} \label{cons:tau:bound}
    \Biggr\}.
\end{align}

We consider the constraint that the traveling time and charging time are within the scheduled time window for $i$-th subpath, $i \in \left\{ 1,...,N+1 \right\}$:

\newcommand{\sumE}{\sum_{e\in \mathcal{E}}}
\newcommand{\sumV}{\sum_{v\in \mathcal{V}_c}}
\begin{equation}
    \begin{aligned}
        \delta_i^\tau(\vec{x}, \vec{y}, \vec{t}, \vec{\tau}) &= \sumE x_e^i t_e^i  + \sumV y_v^{i-1} \left( t_w^{i-1,v} + t_c^{i-1,v} \right) \\ 
    & - \sumV \left( y_v^i \tau_v^i - y_v^{i-1} \tau_v^{i-1} \right) \leq 0.
    \end{aligned}
\end{equation}
Here, the first two terms are the traveling time on $i$-th subpath and the spent time for $(i-1)$-th stop. The third term is the total scheduled time duration between $(i-1)$-th stop and $i$-th stop.
% We also define $t_w^{0,s}=t_c^{0,s}=0$, $\tau_s^0=0, \tau_d^{N+1}=T$ to define the boundary case at origin $s$ and destination $d$.

\textbf{SoC Constraints.} It is complicated to keep track of the SoC at each road segment. In practice, we see that the regenerative braking only contributes a small fraction of energy to the e-truck~\cite{su2021Energy}. With such a practical observation, we show that with a small reservation requirement at the SoC when entering a charging stop at a stage, it is sufficient to guarantee the positive SoC in the entire subpath at that stage. 

In particular, we denote by $\beta_v^i$ the SoC entering charging station $v$ at $i$-th stop. We
stack the variable as $
\vec{\beta}=\left\{ \beta_v^i \right\}_{v\in \tilde{\mathcal{V}}_c, i\in \left\{ 0,...N+1 \right\}}$, and its feasible set is given by

\begin{align}
    \mathcal{S}_\alpha = \Biggl\{ \vec{\beta}  \,|\, 
    &\beta_v^i \in [\alpha B, B], \forall v \in \tilde{\mathcal{V}}_c, i \in \left\{ 0,...,N+1 \right\}, \beta_s^0 = \beta_0 \label{cons:betatau:bound}
    \Biggr\}.
\end{align}

Here, $\alpha \in [0,1)$ denotes the ratio of a conservative lower bound for SoC when an e-truck entering a charging station. We consider the initial SoC at the source as $\beta_0$.


We define the SoC constraint that the e-truck does not run out of battery when entering $i$-th stop:
\begin{equation}
    \begin{aligned}
        \delta_i^\beta(\vec{x}, \vec{y}, \vec{t}, \vec{\beta}) &= \sumE x_e^i c_e(t_e^i)  + \sumV y_v^i \beta_v^i \\ 
        & - \sumV y_v^{i-1} \left( \beta_v^{i-1} + \phi_v(\beta_v^{i-1}, t_c^{i-1,v}) \right) \leq 0.
    \end{aligned} \label{cons:soc}
\end{equation}
Here, the first term is the total energy consumption for $i$-th subpath, the second term is the  SoC when the e-truck enters the $i$-th stop, the third term is the SoC when the e-truck leaves the $(i-1)$-th stop. 
%\rev{ Note that the constraint~\eqref{cons:soc} ensures positive SoC at each recharging stop. However, it is not sufficient for guaranteeing positive SOC at all times as the SOC may be below zero at a road segment and get recharged by regenerative braking later. } 


% To ensure positive SoC on each road segment, we define the following indicator function. % \com{JY}{Maybe need to write the explicit form later, may be put it to appendix.}
% \begin{align}
%     \delta_i^{\beta +}(\vec{x}, \vec{y}, \vec{t}, \vec{\beta}) =
%    \left\{  
%     \begin{aligned}
%         &1, &\text{if positive SoC on subpath $i$} \\
%         &0, &\text{otherwise}
%     \end{aligned}
%    \right. \label{func:soc:pos}
% \end{align}

We show that a small $\alpha$ is sufficient to ensure SoC feasibility during a subpath, as along as the harvested energy due to regenerative brake is relatively small.
% The side effect of this constraint is given by
% we introduce a conservative factor $\alpha$
\begin{lemma}\label{lem:alpha:feasible}
    % \textcolor{blue}{TODO}
    Let an e-truck travels along a subpath with $n$ road segments to a charging stop, along with its energy consumption on each road segment $[c_1,...,c_n]$. If the harvested energy is relatively small and satisfies
    
        \begin{align}
            \frac{1}{2} \sum_{i=1}^{n} \left( |c_i| - c_i \right) & \leq \frac{\alpha}{2(1-\alpha)} \sum_{i=1}^{n} c_i, \label{ineq:recharge} %\\
          %  \beta_0 - \sum_{i=1}^{n} c_i & \geq \alpha B
        \end{align}
    then the SoC at the charging stop being no less than $\alpha\cdot B$ implies that the e-truck always has a non-negative SoC during this subpath.
    % If the ratio between 
    % $\alpha B$ is sufficient to ensure SoC feasibility during a subpath. Meanwhile, the optimality loss is at most $\alpha$.
\end{lemma}
% \begin{proof}
%     See Appendix~\ref{sec:lem:alpha:feasible} 
% \end{proof}
We leave the proof in Appendix~\ref{sec:lem:alpha:feasible}. Note that the harvested energy (i.e., left hand side of~\eqref{ineq:recharge}) for an e-truck traveling across national highway system is indeed small~\cite{su2021Energy}. Because the maximum permissible grade along the US highway is no larger than $6\%$~\cite{hancock2013policy}, there is little energy that can be harvested.
Meanwhile, our simulation in Sec.~\ref{sec:simulation} shows that $\alpha=0.05$ is sufficient to ensure non-negative SoC for most of the instances in our simulation. {Moreover, it also shows that it incurs a small performance gap by comparing it with a lower bound where $\alpha$ is set as zero. %i.e., CFO$_0$ (CFO$_\alpha$ with $\alpha=0$).} \com{ql}{place for it.}



% Note that 
% We also denote $\beta_s^0 = \beta_0$ as the initial SoC at the origin $s$.

\begin{table*}[!tb]
    \centering
    \input{tabs/method-novelty.tex}
    %\input{tabs/related-ev.tex}
    \caption{ Comparison of conceivable problem modelings, formulations, and algorithms for the CFO problem. 
    }
    %\input{tabs/related-ev.tex}
    \label{tab:related-method}
\end{table*}

\textbf{Problem Formulation.} To this end, we are ready to formulate the \emph{Carbon Footprint Optimization} (CFO) problem as follows:

\newcommand{\FvObj}{F_v(t_c^{i,v}, t_w^{i,v}, \beta_v^{i}, \tau_v^{i})}

% \begin{subequations}
%     \begin{align}
%       \textsf{CFO}:\;
%       \min \;& \sum_{i=1}^{N} \sum_{v \in \mathcal{V}_c}^{} y^{i}_{v} \FvObj \label{obj:cfo}  \\
%         \text{s.t. }\; 
%         & \delta_i^\tau(\vec{x}, \vec{y}, \vec{t}, \vec{\tau}) \leq 0,\,  \forall i \in \left\{ 1,...,N+1 \right\} \label{cons:ilp:ddl} \\ 
%         & \delta_i^\beta(\vec{x}, \vec{y}, \vec{t}, \vec{\beta}) \leq 0 , \, \forall i \in \left\{ 1,...,N+1 \right\} \label{cons:ilp:soc0}\\
%         & \delta_i^{\beta+}(\vec{x}, \vec{y}, \vec{t}, \vec{\beta})=1 , \, \forall i \in \left\{ 1,...,N+1 \right\} \label{cons:soc:pos} \\
%         % & \sumV y_v^i \left(  \beta_v^i + \phi_v(\beta_v^i, t_c^{i,v}) \right) \leq B, \, \forall i \in \left\{ 1,...N \right\} \label{cons:ilp:socB} \\
%         % & \tau_{d}^{N+1} = T, t_w^{0,s}=t_c^{0,s} = 0, \beta_s^0 = \beta_0 \label{cons:cfo:bound} \\
%         \text{var.} \; & (\vec{x},\vec{y}) \in \mathcal{P},  (\vec{\beta}, \vec{\tau}) \in \mathcal{S}_0, \vec{t} \in \mathcal{T}.
%         % & \beta_v^i \in [\beta^{lb},B], \tau_v^i \in [0,T], \, \forall v \in \mathcal{V}, i \in \left\{ 1,...,N \right\} \label{cons:cfo:box}
%     \end{align}\label{prob:cfo}
% \end{subequations}


%Here, we aim to minimize the carbon footprint objective~\eqref{obj:cfo}. Constraint~\eqref{cons:ilp:ddl} is the time scheduling constraint for each subpath. Constraints~\eqref{cons:ilp:soc0} and \eqref{cons:soc:pos} are the SoC constraints for each subpath. 
%% Constraints~\eqref{cons:cfo:bound} are the constraints for boundary cases.
%\rev{Notice that the constraint~\eqref{cons:soc:pos} is rather complicated. It introduces coupling between each two successive road segments and explicit expanding it may lead to a larger number of constraints. As a key observation, we find that under practical settings, we can simplify \textsf{CFO} to the following formulation.}
% which motivates us to consider the following modified version \textsf{CFO}

%%\rev{Notice that the constraint~\eqref{cons:soc:pos} is rather complicated as it coupled the decision between any two road seg However, we observe that as the regenerative brake provides a small fraction of energy, it is sufficient to require a small reserved energy $\alpha$ at the charging station to ensure the positive SOC during a subpath. It   motivates us to consider the following modified version \textsf{CFO}}
\begin{subequations}
    \begin{align}
      \textsf{CFO}:\;
      \min \;& \sum_{i=1}^{N} \sum_{v \in \mathcal{V}_c}^{} y^{i}_{v} \FvObj \label{obj:cfo:a} \\
        \text{s.t. }\; 
        & \delta_i^\tau(\vec{x}, \vec{y}, \vec{t}, \vec{\tau}) \leq 0,\,  \forall i \in \left\{ 1,...,N+1 \right\}  \label{cons:cfoa:ddl} \\ 
        & \delta_i^\beta(\vec{x}, \vec{y}, \vec{t}, \vec{\beta}) \leq 0 , \, \forall i \in \left\{ 1,...,N+1 \right\} \label{cons:cfoa:soc0} \\
        \text{var.} \; & (\vec{x},\vec{y}) \in \mathcal{P},  \vec{\beta} \in \mathcal{S}_{\alpha},  \vec{\tau}\in \mathcal{T}_\tau , \vec{t} \in \mathcal{T}. \label{cons:cfoa:var}
    \end{align}\label{prob:cfo:a}
\end{subequations}


Here, we aim to minimize the carbon footprint objective~\eqref{obj:cfo:a}. Constraint~\eqref{cons:cfoa:ddl} is the time scheduling constraint for each subpath. Constraints~\eqref{cons:cfoa:soc0} is the SoC constraints for each subpath. We summarize the notations in Tab.~\ref{tab:notation}. 

We give the hardness result of the problem in the follow theorem. %In \textsf{CFO}, we drop the complicated constraint~\eqref{cons:soc:pos} and add a conservative lower bound $\beta_v^i \geq \alpha B $ with $\alpha \in (0,1)$ as shown in~\eqref{cons:cfoa:var}.

%% Note that the SoC constraint~\eqref{cons:soc} does not consider the SoC feasibility during the subpath. It is possible that an e-truck has a negative SoC in the middle of a subpath but has a positive SoC when entering the next the charging station, due to the regenerative system.
% To address this, we define the conservative SoC lower bound $\beta_v^i \geq \beta^{lb}=\alpha B, \alpha \in (0,1)$ in~\eqref{cons:betatau:beta} to ensure an e-truck reserves $\alpha B$ amount of energy when entering an charging station. 
% A typical value of the recharging ratio in~\eqref{ineq:recharge} is $\frac{\alpha}{2(1-\alpha)}=0.03 \Rightarrow \alpha = 0.057$ and it is sufficient to ensure non-negative SoC for all instances in our simulation.
% \textcolor{blue}{TODO: discussion on the optimality loss.}
% Meanwhile, the optimality loss introduced by the lower bound $\beta^{lb}=\alpha B$ is also small:
% \begin{lemma}
%     The optimality loss introduced by $\beta^{lb}=\alpha B$ is at most $\alpha$?
% \end{lemma}
% \begin{proof}
%     \textcolor{blue}{TODO: Not sure. Things can be tricky...}  
% \end{proof}
% Fig.~\ref{fig:alphaSoC} illustrates the idea of this constraint.



% \begin{figure}[!tb]
%     \includegraphics[width=.75\linewidth]{figs/socAlpha.pdf}
%     \vspace{-1mm}
%     \caption{A example of $\alpha=0.05$ to ensure SoC feasibility during a subpath.}\label{fig:alphaSoC}
% \end{figure}


\begin{theorem}\label{thm:nphard}
    \textsf{CFO} is NP-hard.
    % \vspace{-3mm}
\end{theorem}
% \begin{proof}
%     See Appendix~\ref{sec:thm:nphard} 
% \end{proof}
Please refer to Appendix~\ref{sec:thm:nphard} for the proof. The NP-hardness of the CFO problem comes from the fact that a special case of the CFO problem is PASO problem~\cite{dengEnergyefficient2017} that considers the path planning and speed planning for energy-efficient timely transportation with ICE trucks.


\subsection{Remark on Challenges and Novelty}\label{sec:challenge}
% \textcolor{blue}{Need to revise according to abstract and revised problem formulation section.}

We first remark on four outstanding challenges of the CFO problem, after which we discuss the novelty of our formulation and its significance for tackling those challenges.

\noindent\textbf{Remark on Challenges.}
The first challenge comes from optimal path planning and speed planning under the hard deadline constraint, which already makes the problem NP-hard.  This challenge exists in both the CFO problem and the E2T2 problem for ICE trucks, e.g.,~\cite{dengEnergyefficient2017}. The following three challenges are unique to e-truck and CFO.

The second challenge is the positive battery SoC requirement for each road segment, which adds strong couplings to the problem. One of the conventional ways is to explicitly define variables and constraints on each road segment (c.f., EVRP~\cite{montoyaElectric2017}) and obtain a large Mixed-Integer Programming (MIP). 
However, the resulting MIP is still challenging to solve because general-purpose methods usually do not scale well on MIP.  
We mitigate this challenge in our formulation with a key observation (Lemma~\ref{lem:alpha:feasible}) that it is sufficient to restrict the SoC only when entering each charging stop (and the destination) by a conservative lower bound, i.e.,~\eqref{cons:soc}. As reported in Sec.~\ref{sec:simulation}, such simplification only incurs a small performance loss.
% Our formulation $\cfoa$ tackles this challenge by identifying a special structure of CFO that the harvested energy is relatively small so that we can replace the complicated constraint~\eqref{cons:soc:pos} with a small lower bound and only check the positive SoC requirement at each recharging stop.
% The resulting SoC constraint~\eqref{cons:soc} becomes much easier to handle as we will see the Sec.~\ref{sec:method}.
% adding a conservative lower bound and dropping the constraint~\eqref{cons:soc:pos}. 

The third challenge comes from the non-convex objective, which is unique to the CFO problem. 
% Also, we are the first to consider carbon footprint optimization in the electric mobility literature. 
% As illustrated in Fig.~\ref{fig:obj}, 
The objective is time-varying and highly non-convex with respect to $\tau$ due to the fluctuating nature of renewable. 
Large-scale non-convex problems are in general challenging to solve. Our problem formulation reveals an elegant problem structure that allows us to decompose the large non-convex problem into a number of significantly less-complex subproblems, which can be efficiently solved by global optimization tools, as we will show in Sec.~\ref{sec:method}.

The last challenge comes from enormous geographical and temporal charging options with diverse carbon intensity. 
% Due to the spatial-temporal diversity of carbon intensity, it is critical to decide the moment and location to charge. 
The charging station selection configuration space has a combinatorial nature. A straightforward search over locations results in an exponential runtime with respect to $N$. 
% We tackle this challenge by dualizing the constraints and assigning a constraint-respect cost to each charging station. We can then apply a simple shortest-path algorithm with those augmented costs on an extended graph.
To tackle this challenge, our formulation extends the transportation graph to a stage-expanded graph to model charging options. 
%As we will see in Sec.~\ref{sec:method}, this extension 
This extension significantly reduces the searching space to a polynomial number and allows us to systematically search charging stations with constraint-respect costs via Lagrangian relaxation.

\noindent\textbf{Remark on Novelty.}
Overall, those four challenges make the CFO problem notoriously challenging to solve.
In the following, we remark the novelty of our approach by
comparing our approach with several conceivable alternatives that are applicable to the CFO problem. We summarize the comparison in Tab.~\ref{tab:related-method}. % and provide the detailed discussion in Appendix~\ref{sec:novelty}.

The first direction of alternatives (c.f., the first row and the second row in Tab.~\ref{tab:related-method}) resorts to directly formulate the CFO problem as a Mixed Integer Program (MIP) and solve it with general-purpose methods (e.g., branch and bound). However, the resulting MIP is still challenging to solve. The general-purpose methods usually do not scale well to large problems as they do not carefully explore the problem structure. 

The second direction of alternative expands the graph with discretized state $\beta$ and $\tau$ (c.f. the third row in Tab.~\ref{tab:related-method}). Once the expanded graph is constructed, the CFO problem can be transformed to a shortest path problem on the expanded graph. However, the graph is $(T\cdot B)/\epsilon^2$ times of the original graph, making the approach fail to scale to large networks with favorable accuracy.

In contrast, our formulation in~\eqref{prob:cfo:a} enjoys the benefits for the both worlds. It has a low-complexity stage-expanded graph model, which does not involve discretizing the time or SoC. Moreover, the formulation reveals an elegant problem structure for effective algorithm design. 
In the next section, we shall exploit the understanding and design an efficient dual-subgradient method that has good theoretical and empirical performance.
We also provide a detailed comparison in Appendix~\ref{sec:novelty}
% \textcolor{blue}{TODO:}


% We leave the detailed discussion in Sec.~\ref{sec:novelty}.

% Yet, we carefully design the novel problem formulation~\eqref{prob:cfo:a} such that those challenges become tractable by a dual-based approach in the next section.

% We conclude this section by a remark on the novelty of our problem formulation~\eqref{prob:cfo:a}.

% is to expand the charging station graph instead of original graph (e.f., second row of Tab.~\ref{tab:related-method}). In 
% The advantage is that 
% The first row is a straightforward idea, that is, to directly discretize the decisions and search over the graph via a label-setting method~\cite{baumSpeedConsumption2014}. However, this method usually generates exponential number of labels and suffers from the curse of dimensionality. 

% \textcolor{blue}{TODO: more discussions here.}
% We carefully design the novel problem formulation~\eqref{prob:cfo:a} such that those challenges become tractable by a dual-based approach in the next section.

% A conventional formulation for~\eqref{}



==> arxivSource/arxiv/4.1.csg.tex <==

% A prefix for charging station graph (csg)
\newcommand{\csgpre}[1]{\tilde{\mathcal{#1}}}
\newcommand{\exgpre}[1]{\hat{\mathcal{#1}}}

% \item We can add a virtual charging station at the destination $d$ for notation convenience, since there is no benefit to charge and wait at the end.

% In this section, we will ...
\subsection{Charging Station Graph}
\textcolor{blue}{TODO: Might need to rewrite to be compatible with the method described below}.
One of the core challenges in \textsf{CFO} is to ensure the SoC feasibility between two charging stations. 
% It is unclear an electric truck 
To address this, we consider a new graph $\csgpre{G} = (\csgpre{V}, \csgpre{E})$ on charging stations.
Here $\csgpre{V} = \mathcal{V}_c \cup \{s,d\} $ is the set of charging stations along with two points origin $s$ and destination $d$. 
The construction of the edge set $\csgpre{E}$ requires more efforts. 
We want to eliminate charging station pairs $(i,j)$ that $j$ is not reachable from $i$ without intermediate recharging.
In particular, for each $i\in \csgpre{V} $ and $j \in \csgpre{V}$, we define $C_{ij}(\tau)$ as the minimum energy consumption traveling from $i$ to $j$ in the original graph~$\mathcal{G}$ without charging stops, subject to deadline $\tau$.
In particular, $C_{ij}(\tau)$ is the optimal value of the \textsf{PASO} problem with deadline $\tau$.
\begin{equation}
\begin{aligned}
   C_{ij}(\tau) = \min_{\vec{t} \in \mathcal{T}, \vec{x} \in \mathcal{X}_{ij}^r }\;& \sum_{(u,v) \in \mathcal{E}_r}^{} x_{uv} c_{uv}(t_{uv})   \\
    \text{s.t. }\;& \sum_{(u,v)\in \mathcal{E}_r} x_{uv} t_{uv} \leq \tau
\end{aligned} \label{prob:paso}
\end{equation}
Note that computing the optimal value of the problem~\eqref{prob:paso} is also NP-hard. However, we can obtain an upper bound of problem~\eqref{prob:paso} with small optimality loss by efficient heuristics (e.g.,~\cite{dengEnergyefficient2017}). Our method in the following is still applicable if we replace the value of $C_{ij}(\tau)$ with its upper bound.

% Another issue, however, requires more efforts to tackle
% $C_{ij}(T)$ can be shown to be non-increasing.
% We need to ignore regenerative system here to ensure the SoC feasibility.

For each $i\in \csgpre{V}$ and $j \in \csgpre{V}$, define the $t_{ij}^{fast}$ and $t_{ij}^{slow}$ as the minimum traveling time and maximum traveling time respectively between origin $i$ and destination $j$ without intermediate recharging stops. 
Then we can denote the set of $\csgpre{E}$ as 
\begin{align}
    \csgpre{E} = \left\{ (i,j) \in \csgpre{V} \times \csgpre{V} : C_{ij}(t^{slow}_{ij}) \leq \alpha B \right\} \label{set:csedge}
\end{align}
That is, there is an edge between $i$ and $j$ only when $j$ is reachable from $i$ without intermediate recharging stops. Here $0 \leq \alpha \leq 1$ is a constant to address the negative value of $c_{uv}(\cdot)$ in~\eqref{prob:paso} due to the regenerative system. In particular, because $c_{uv}(\cdot)$ can have negative value, the difference between maximum SoC and minimum SoC can be larger than the summation of $c_{uv}(\cdot)$ as illustrated in Fig.~\ref{fig:soc-alpha}. So we use $\alpha B$ as a soft penalty to ensure the SoC constraint between $i$ and $j$. 
Note that the worst case rarely happens in practice and the regenerative system of an electric truck has little impact during the whole path~\cite{su2021Energy}. Therefore, it is sufficient to choose a fairly large $\alpha$ (e.g., $0.95$) in practice which only introduce little optimality loss.

\begin{figure}[!tb]
    \includegraphics[width=.9\linewidth]{figs/socAlpha.pdf}
    \vspace{-4mm}
    \caption{SoC profile along a path. 
    We use $\alpha$ to give a soft penalty to ensure the SoC constraint.
    }\label{fig:soc-alpha}
    \vspace{-5mm}
\end{figure}

For each edge $(i,j) \in \csgpre{E}$, we define three decision variables related to time planning $t_{ij}^r$, $t_{ij}^w$, $t_{ij}^c$, denoting the amount of time for driving on the real road segment, waiting at the charging station, and charing at the charging station, respectively.
We define the objective function $\tilde{F}_{ij}$ the same as the objective function for the charging station $j$. 
For each $(i,j)\in \csgpre{E}$, we assign a time lower bound and time upper bound for the time driving on road $t_{ij}^r$:
% We can then define the time limit for real road part of edge $(i,j) \in \csgpre{E}$.
\begin{align}
    \tilde{t}_{ij}^{ub} = t_{ij}^{slow}, \qquad
    \tilde{t}_{ij}^{lb} =
    \left\{  
    \begin{aligned}
        & t_{ij}^{fast} &\, \text{if }  C_{ij}(t_{ij}^{fast}) \leq \alpha B, \\
        & C_{ij}^{-1}(\alpha B) &\, \text{otherwise.}
    \end{aligned}
    \right.
\end{align} 
Here, $C_{ij}^{-1}(\cdot)$ is the inverse function of $C_{ij}(\cdot)$. Note that $C_{ij}(\tau)$ is a non-decreasing function with respect to $\tau$ since increase $\tau$ will enlarge the constraint set for the problem~\eqref{prob:paso}. 
Therefore, we can always found the (upper bound) value of $C_{ij}^{-1}(\cdot)$ by a simple bisection.
Therefore, given any path on $\csgpre{G}$, there is always a time schedule that satisfies the SoC constraint, since one can always fully charge the battery before going to the next charging station.

==> arxivSource/arxiv/4.1.expanded-graph.tex <==

\subsection{Time-Expanded and Battery-Expanded Graph}
The CFO problem remains challenging on the charging station graph due to the coupling of decisions on each edge. That is, the decisions of driving time, waiting time and charging time at the current edge affects carbon-intensities of the following charging stations. To address this, we construct a new time-expanded and battery-expanded graph $\exgpre{G}=(\exgpre{V}, \exgpre{E})$ from the charging station graph $\csgpre{G}=(\csgpre{V},\csgpre{E})$. 
In particular, for each node $i \in \csgpre{V}$, we add $(N_{\tau}+1)(N_{\beta}+1)$ copies to the new node set $(i, i_\beta, i_\tau) \in \exgpre{V}$ for all $i_\beta = 0,...,N_\beta$ and $i_\tau = 0,...,N_\tau$. Here $N_\beta$ and $N_\tau$ are the number of discretized states for $\beta$ and $\tau$ respectively.
For each edge $(i,j) \in \csgpre{E}$, we add the edge $((i,i_\beta, i_\tau), (j, j_\beta, j_\tau))$ to the new edge set $\exgpre{E}$. 
An edge $((i,i_\beta, i_\tau), (j, j_\beta, j_\tau))$ means we require the e-truck to travel from node $i$ to $j$ with initial SoC $i_\beta B / N_\beta$, initial arrival time $i_\tau T / N_\tau$ at node $i$ and 
final SoC $j_\beta B / N_\beta$, final arrival time $j_\tau T / N_\tau$ at node $j$.
The cost for the edge $((i,i_\beta, i_\tau), (j, j_\beta, j_\tau))$ is given by
\begin{subequations}
    \begin{align}
        \min_{t^w, t^r, t^c}\;&  F_{ij}(\beta_i, t^c, \tau_i + t^w) \\
        \text{s.t. }\;& \tau_j = \tau_i + t^w + t^r + t^c \label{cons:exg:tau} \\
        & \beta_j = \beta_i + \phi(t^c, \beta_i) - C_{ij}(t^r_{ij}) \label{cons:exg:soc} \\
        & \beta_i = i_\beta B / N_\beta,  \,
        \beta_j = j_\beta B / N_\beta,  \\
        & \tau_i = i_\tau T / N_\tau, \,
        \tau_j = j_\tau T / N_\tau, \\
        & t^w \geq t^w_0, \tilde{t}^{lb}_{ij} \leq t^r \leq \tilde{t}^{ub}_{ij}, t^c \geq 0.
    \end{align} \label{prob:exg}
\end{subequations}

We discard the edge if problem~\eqref{prob:exg} is infeasible.
Despite the complexity of problem~\eqref{prob:exg} at the first glance, we can actually convert it to a single-variable optimization problem over an interval. Given on-road travel time $t^r$, we can uniquely determine $t^c$ by constraint~\eqref{cons:exg:soc} and then determine $t^w$ by constraint~\eqref{cons:exg:tau}. Then problem~\eqref{prob:exg} can be efficiently solved via classic algorithms (e.g. golden-section search~\cite{avriel1966optimally} or Powell's method~\cite{powell1964efficient}).
\textcolor{blue}{TODO: Maybe add explicit formulation?}

% The infeasible problem?

By constructing the expanded graph $\exgpre{G}$, we achieve to distribute the coupling decisions to different nodes and edges on the new graph. 
This allows us to simply apply a shortest path algorithm (e.g. Dijkstra) on the expanded graph $\exgpre{G}$ from node $(s, \lceil \beta_0/N_\beta \rceil, 0)$ to a virtual destination node $\hat{d}$. Here, we additionally add the node $\hat{d}$ and zero-weight edges $((d, i_\beta, i_\tau) , \hat{d})$ for all $i_\beta = 0,...,N_\beta$ and $i_\tau = 0,...,N_\tau$ for auxiliary purpose. Once obtain the path, we can retrieve the speed planning and charing scheduling decisions by solving problem~\eqref{prob:exg} along the given path.

We remark that by discretize the SoC and traveling time, we discard some of the feasible solutions because problem~\eqref{prob:exg} is not always feasible. 
% However, ()
\textcolor{blue}{TODO: Maybe we can provide a optimality bound in the following subsection}


\subsection{Performance Analysis}
\begin{itemize}
    \item Time complexity
    \begin{itemize}
        \item For constructing the graph.
        \item For solving one instance of CFO problem.
    \end{itemize}
    \item Optimality gap.
\end{itemize}

\subsection{Implementation Details}
\begin{itemize}
    \item Reducing the number of edges.
\end{itemize}

% \noindent\textbf{Time Complexity.}
% \\Complexity for constructing the graph: 
% \\Complexity for solving an instance of CFO.
% 
% \textbf{Performance guarantee:}


==> arxivSource/arxiv/4.1.ida.tex <==

\subsection{An Iterative Deepening Approach}
% In practice, a human driver may want to reduce the number of recharging stops. 
% The idea behind is that in practice, we can 
In practice, the number of recharging stops of a trip should not be too large if we take the human drivers' experience into account. Besides, large number of recharging stops may have little marginal benefit while significantly increases the time complexity. 
Based on those observations, we propose an iterative deepening approach by iteratively allowing more recharging stops in a path.
% At each iteration, we fix the number of 

\noindent\textbf{Time Scheduling and Speed Optimization.}
Let us first consider the case where a path $p = [p_1, ..., p_n]$ on $\csgpre{G}$ is given. Then the problem remains to solve the following \emph{charge scheduling and speed optimization} (CSSO) problem on the charging station graph.

\newcommand{\pip}{ {p_{i} p_{i+1}} }
\begin{subequations}
\begin{align}
   g(p) = \min_{\vec{t}, \vec{\beta}, \vec{\tau}}\;&  \sum_{i=1}^{n-1} 
   F_{p_i p_{i+1}}\left(\hat{\beta}_{p_i} , t_{p_i p_{i+1}}^c, \tau_{p_{i}} + t^w_{p_i p_{i+1}} + t^c_{p_i p_{i+1}} \right) \label{obj:spd} \\
    \text{s.t. }\;& \hat{\beta}_{p_i} = \beta_{p_i} - C_{p_i p_{i+1}}(t_{p_i p_{i+1}}^r) \geq 0, \forall i \in [1,n-1] \label{cons:spd:bhat} \\
    & \beta_{p_{i+1}} = \hat{\beta}_{p_{i}} + \phi(t^c_{p_i p_{i+1}}, \hat{\beta}_{p_i}), \forall i \in [1,n-1] \label{cons:spd:b} \\
    & \tau_{p_{i+1}} = \tau_{p_i} + t^r_{p_{i} p_{i+1}} + t^w_{\pip} + t^c_{\pip} , \forall i \in [1,n-1] \label{cons:spd:tau} \\
    & \sum_{i=1}^{n-1} \left(   t^r_{p_{i} p_{i+1}} + t^w_{\pip} + t^c_{\pip} \right) \leq T \label{cons:spd:ddl} \\
    & t^c_{\pip}  \geq 0, \; t^w_{\pip} \geq w_0, , \forall i \in [1,n-1] \label{cons:spd:box1} \\
    & \tilde{t}^{lb}_{\pip} \leq  t^r_{\pip} \leq \tilde{t}^{lb}_{\pip} , \forall i \in [1,n-1] \label{cons:spd:box2} \\
    & \beta_{p_1} = \beta_0, \, \tau_{p_1} = 0 \label{cons:spd:init}
\end{align} \label{prob:csso}
\end{subequations}
We additionally set $g(p)=\infty$ if the above problem is infeasible or $p=\emptyset$.
Here, the objective~\eqref{obj:spd} is the same as before. We introduce an auxiliary variable $\hat{\beta}$ in~\eqref{cons:spd:bhat} for notational convenience. 
Constraint~\eqref{cons:spd:bhat} is to ensure the SoC constraint. Constraints~\eqref{cons:spd:b} and \eqref{cons:spd:tau} are state variable constraints similar as before. Constraint~\eqref{cons:spd:ddl} is to satisfy the deadline constraint. 
Constraints~\eqref{cons:spd:box1} and \eqref{cons:spd:box2} are the box constraints on the time decision variables.
Constraint~\eqref{cons:spd:init} defines the initial conditions for $\beta$ and $\tau$. 
Note that the CSSO problem~\eqref{prob:csso} is defined on the charging graph~$\csgpre{G}$ and thus has much smaller size as compared to the CFO problem~\eqref{prob:cfo}. A typical size of~\eqref{prob:csso} is $n=10$ on the US national highway network.

Even though we reduce the problem to a specific path on the charging garph~$\csgpre{G}$, the CSSO problem ~\eqref{prob:csso} is still non-convex due to the non-convex objective~\eqref{obj:spd} and non-convex constraints~\eqref{cons:spd:bhat} and~\eqref{cons:spd:b}. 
Therefore, it is still difficult to obtain the global minimum. 
If our approach, however, an upper bound of $g(p)$ can also be used without further modification. Thus, we can use local minimization algorithm and solvers (e.g., NLopt~\cite{johnson2014nlopt}) to solve problem~\eqref{prob:csso}. 

\noindent\textbf{An Iterative Deepening Approach.} 
After defining the CSSO problem and $g(p)$, we are ready to reformulate the \textsf{CFO} problem in a iterative deepening manner on $\csgpre{G}$:
\begin{align}
    % \textsf{CFO-ID}: \quad 
    \min_{n\in \left\{ 2,...,|\csgpre{V}| \right\}}\; \min_{p \in \mathcal{P}_n} g(p)  \label{prob:cfo-id}
\end{align}
Here $|\csgpre{V}|$ is the number of nodes on $\csgpre{G}$. We denote $\mathcal{P}_n$ is the set of all paths from $s$ to $d$ with $n$ nodes:
\begin{equation}
\begin{aligned}
    \mathcal{P}_n = \Big\{ p = [p_1, &...,p_n] : p_1 = s,\, p_n = d, \text{ and } 
    \\ & (p_i, p_{i+1}) \in \csgpre{E},\, \forall i \in \left\{ 1,...,n-1 \right\} \Big\}
\end{aligned}
\end{equation}
We set $\mathcal{P}_n = \emptyset$ if no such path exists.
Problem~\eqref{prob:cfo-id} gives us a new perspective of solving \textsf{CFO} problem. 
We can first fix the number of nodes $n$ in a path, find the best path within $\mathcal{P}_n$, and increase the number of node in the next iteration. The overall procedure is outlined in Algorithm~\ref{alg:ida}.  Lines~\ref{alg:ida:1}-\ref{alg:ida:end} correspond to the outer minimization in problem~\eqref{prob:cfo-id} and the inner minimization problem is solved by a depth first search (DFS) procedure (lines~\ref{alg:ida:dfs1}-\ref{alg:ida:dfsend}). 
Note that in practice, it is sufficient to set the total number of outer iterations $N$ to a relatively small number to let Algorithm~\ref{alg:ida} produce high-quality solutions.

\input{algs/dfs.tex}
\input{algs/test.tex}

In the DFS procedure, for a path $p=[p_1,...,p_k]$, we use $\text{tail}(p) = p_k$ to denote the last node of $p$ and $|p|=k$ to denote the number nodes in $p$. We also use $p'=p\circ v = [p_1,...,p_k,v]$ to denote the concatenation of a path $p$ and a node $v$. The DFS procedure is defined in a recursive manner, if the searched path $p$ has exactly $n$ nodes, then we update the current best path $p^\star$ if necessary. 
Otherwise, we construct a new path $p'$ by the concatenation of $p$ and a out neighbor of tail($p$), recursively call DFS on $p'$.

\noindent\textbf{Candidate Test.}
Note that even through $n$ is relatively small in practice, the number of candidates $|\mathcal{P}_n| = O(|\csgpre{V}|^n)$ can still be very large, which leads to high computational cost. To reduce the computational cost, a candidate test procedure is therefore necessary to prune unnecessary branches in the DFS search tree.
A good candidate test procedure can significantly prune the DFS search space and speedup our algorithm. 

We provide several criteria to test a promising candidate path $p$ as outlined in Algorithm~\ref{alg:test}. 
% The first two conditions are straightforward. 
We first check if the minimum travel time already exceeds the deadline $T$ in line~\ref{alg:test:ddl} where we use $\tilde{t}^{lb}(p)$ to denote the minimum travel time of $p$. 
The second condition in line~\ref{alg:test:distance} is to check if path $p$ is heading towards the destination, where distance($u,v$) denotes the straight line distance between two nodes $u$ and $v$.
This condition is a heuristic to avoid path with back road.
The third condition in line~\ref{alg:test:lb} check the objective lower bound $\underline{g}(p)$ with the current best objective value $g(p^\star)$ and prune the sub-optimal branches.
% The problem remains on how to obtain a tight lower bound $\underline{g}(p)$. In 
There are many ways to obtain a lower bound of $g(p)$. In the following, we provide simple yet effective way by relaxing problem~\eqref{prob:csso} to a simple linear programming (LP). 
For each node $i\in \mathcal{V}_c$, we denote the lower bound of carbon intensity by
\begin{equation}
\underline{\pi}_i = \min_{ 0 \leq \tau \leq T} \pi_i(\tau)
\end{equation}
Given a path $p = [p_1, ..., p_k]$, we compute the lower bound $\underline{g}(p)$ by solving the following \textsf{csso-LP} problem.
\begin{subequations}
\begin{align}
    \underline{g}(p) = \min_{\Delta \beta}\;& \sum_{i=1}^{k-1} \underline{\pi}_{p_i} \Delta \beta_{p_i} \label{obj:lp} \\
    \text{s.t. }\;&  0 \leq \Delta \beta_{p_i} \leq B, \forall i \in \left\{ 1,...,k-1 \right\} \\
    & \beta_0 + \sum_{i=1}^{k-1} \Delta \beta_{p_i} \geq \sum_{i=1}^{k-1} C_{p_i p_{i+1}}\left(t^{ub}_{p_i p_{i+1}} \right) \label{cons:lp:soc}
\end{align} \label{prob:csso-lp}
\end{subequations}
Here, we replace the objective~\eqref{obj:spd} by its lower bound~\eqref{obj:lp} and reduce the complicated constraints in~\eqref{prob:csso} to a simple constraint~\eqref{cons:lp:soc}, which only require the overall energy charged to the battery is greater than or equal to the minimum energy consumption along the path $p$.
Note that the right hand side of~\eqref{cons:lp:soc} can be pre-computed and thus is a constant. Therefore, problem~\eqref{prob:csso-lp} can be easily solved by greedily allocate charged energy $\Delta \beta$ with minimum carbon intensity.
Meanwhile, we can show that $\underline{g}(p)$ is indeed a lower bound of $g(p)$ by the following Lemma.
\begin{lemma}
 $\forall p=[p_1,...,p_k]$ on graph $\csgpre{G}$, we have $\underline{g}(p) \leq g(p)$. 
\end{lemma}
\begin{proof}[Proof]
    Given a path $p=[p_1,...,p_k]$, for every feasible solution $\vec{t}, \vec{\beta}, \vec{\tau}$ of problem~\eqref{prob:csso}, we can compute a feasible solution in problem~\eqref{prob:csso-lp} :
    \begin{equation}
        \Delta \beta_{p_{i+1}} = \phi(t^c_{p_i p_{i+1}}, \hat{\beta}_{p_i}), \forall i \in \left\{ 1,...,k-1 \right\}
    \end{equation}
    which leads to a lower objective
    \begin{equation}
        \begin{aligned}
       \underline{g}(p) 
       & \leq \sum_{i=1}^{k-1} \underline{\pi}_{p_i} \Delta \beta_{p_i} \\
       & \leq  \sum_{i=1}^{k-1} F_{p_i p_{i+1}}\left(\hat{\beta}_{p_i} , t_{p_i p_{i+1}}^c, \tau_{p_{i}} + t^w_{p_i p_{i+1}} + t^c_{p_i p_{i+1}} \right)
        \end{aligned}
    \end{equation}
    This inequality holds for any feasible solution of problem~\eqref{prob:csso}. Therefore, we have $\underline{g}(p) \leq g(p)$.
    % This is true because every feasible solution of csso can be transformed to a feasible solution of csso-LP with lower objective value.
\end{proof}

% Overall, we provide a te
% Therefore, we can

% \noindent\textbf{Implementation Details.} 
% \begin{itemize}
%     \item The edge order of dfs.
% \end{itemize}

==> arxivSource/arxiv/4.admm.tex <==
\section{An ADMM Based Method}

One of the challenges of \textsf{CFO} lies in the coupling constraints~\eqref{cons:cfo:soc} and~\eqref{cons:cfo:tau} along the selected path. 
In this section, we use the splitting technique and leverage the idea from the alternating direction method of multipliers~(ADMM)~\cite{boyd2011distributed} to decouple the constraints. 
After decomposition, the update steps of ADMM can be easily tackled by solving a number of small-size subproblems and a shortest path problem.
In particular, we reformulate the \textsf{CFO} problem by introducing auxiliary variables $\vec{\beta'}$ and $\vec{\tau'}$.
\begin{align}
    \min_{
        \substack{
        \vec{\beta'} \in \mathcal{B} , \vec{\tau'} \in \mathcal{S},  \\
        \vec{\beta} \in \mathcal{B} , \vec{\tau} \in \mathcal{S},  \\
        \vec{t} \in \mathcal{T}, \vec{x} \in \mathcal{X} 
        }}
        \;& \sum_{(i,j)\in \mathcal{E}} x_{ij} F_{ij}(\beta_i, t_{ij}, \tau_i) \label{obj:cfop}  \\
    \text{s.t. }\;
    & x_{ij} \cdot \left( \beta_j' - \min \left\{ B,  \beta_i - c_{ij}(t_{ij}, \beta_i) \right\} \right)  = 0, \, \forall (i,j) \in \mathcal{E} \label{cons:cfop:soc} \\
    & x_{ij} \cdot \left(   \tau_j' - \tau_i - t_{ij} \right) = 0, \, \forall (i,j) \in \mathcal{E} \label{cons:cfop:tau} \\
    & x_{ij} (\beta_j - \beta_j') = 0, \forall (i,j) \in \mathcal{E} \label{cons:cfop:beq} \\
    & x_{ij} (\tau_j - \tau_j') = 0, \forall (i,j) \in \mathcal{E} \label{cons:cfop:taueq}
\end{align}
Here, we replace $\beta_j$ with $\beta_j'$ in the SoC constraint~\eqref{cons:cfop:soc} and replace $\tau_j$ with $\tau_j'$ in the traveling time constraint~\eqref{cons:cfop:tau}. We introduce additional constraints~\eqref{cons:cfop:beq} and~\eqref{cons:cfop:taueq} to make sure the auxiliary variables equal to the original variables along the selected path. 
The augmented Lagrangian is given by:
\newcommand{\gij}{g_{ij}(t_{ij}, \beta_i, \beta_j, \tau_i, \beta_j', \tau_j', \lambda_{ij}^\beta, \lambda^\tau_{ij}, \mu_{ij}^\beta, \mu_{ij}^\tau)}
\newcommand{\dualvec}{\vec{\lambda}^\beta, \vec{\lambda}^\tau, \vec{\mu}^\beta, \vec{\mu}^\tau}
\newcommand{\dualveck}{\vec{\lambda}^{\beta k}, \vec{\lambda}^{\tau k}, \vec{\mu}^{\beta k}, \vec{\mu}^{\tau k}}
\begin{align}
    &\mathcal{L}_{\rho}(\vec{t}, \vec{x}, \vec{\beta}, \vec{\tau}, \vec{\beta}', \vec{\tau}', \dualvec) = \nonumber \\
    &\sum_{(i,j)\in \mathcal{E}} x_{ij} \gij
\end{align}
where $\dualvec$ are the dual variables for the constraints \eqref{cons:cfop:soc}-\eqref{cons:cfop:taueq} respectively. The function $g_{ij}$ is given by
\begin{align}
     & \gij  = \\
     &F_{ij}(\beta_i, t_{ij}, \tau_i)  \label{gij:obj} \\
     &+ L_{\rho}(\lambda^\beta_{ij}, \beta_j' - \min \left\{ B,  \beta_i - c_{ij}(t_{ij}, \beta_i) \right\} ) \label{gij:lamb} \\
     &+  L_{\rho}(\mu^{\beta}_{ij}, \beta_j - \beta_j' ) \label{gij:mub}  \\
     & + L_{\rho}(\lambda^\tau_{ij}, \tau_{j}' - \tau_i - t_{ij} )
     + L_{\rho}(\mu^{\tau}_{ij}, \tau_j - \tau_j') \label{gij:tau}
      % + \mu^\tau_{ij} \left( \tau_i - \tau_i' \right)  + \frac{\rho}{2} \left( \tau_i - \tau_i' \right)^2
\end{align}
where auxiliary function $L\rho(\lambda, z)$ is given by
\begin{equation*}
    L_{\rho}(\lambda, z) = \lambda z + \frac{\rho}{2} z^2
\end{equation*}
where $\rho > 0$ is a penalty term for the equality constraints. An iteration of ADMM for solving problem~\eqref{obj:cfop} consists of the following steps:

1) path-update step 
\begin{align}
    &(\vec{x}^{k+1},\vec{\beta}'^{k+1},\vec{\tau}'^{k+1}) = \nonumber  \\
    & \qquad  \arg\min_{
        \substack{
        \vec{x} \in \mathcal{X}, \vec{\beta}' \in \mathcal{B}, \\ \vec{\tau}' \in \mathcal{S} 
        }}
        \mathcal{L}_{\rho}(\vec{t}^{k}, \vec{x}, \vec{\beta}^k, \vec{\tau}^k, \vec{\beta}', \vec{\tau}', \dualveck) \label{admm:pathupdate}
\end{align}

2) t-update step
\begin{align}
    &(\vec{t}^{k+1}, \vec{\beta}^{k+1},\vec{\tau}^{k+1}) = \nonumber  \\
    & \qquad  \arg\min_{
        \substack{
        \vec{t} \in \mathcal{T} , \vec{\beta} \in \mathcal{B}, \\
        \vec{\tau} \in \mathcal{S}
        }} 
    \mathcal{L}_{\rho}(\vec{t}, \vec{x}^{k+1}, \vec{\beta}, \vec{\tau}, \vec{\beta}'^{k+1}, \vec{\tau}'^{k+1}, \dualveck) \label{admm:tupdate}
\end{align}

3) dual-update step, for each $(i,j) \in \mathcal{E}$ such that $x^{k+1}_{ij}=1$
\begin{align}
    \begin{split}
    \lambda_{ij}^{\beta (k+1)} &= 
          \lambda_{ij}^{\beta k} + \rho \left(\beta_j'^{k+1} - \min \left\{ B, \beta_i^{k+1} - c_{ij}(t_{ij}^{k+1}, \beta_i^{k+1}   \right\}\right) \\
    \lambda_{ij}^{\tau (k+1)} 
        &= \lambda_{ij}^{\tau k} + \rho \left( \tau_j'^{k+1}  - \tau_i^{k+1} - t_{ij}^{k+1} \right) \\
    \mu_{ij}^{\beta (k+1)} &= \mu_{ij}^{\beta k} + \rho \left( \beta_j^k - \beta_j'^k \right) \\
    \mu_{ij}^{\tau (k+1)} &= \mu_{ij}^{\tau k} + \rho \left( \tau_j^k - \tau_j'^k \right) 
    \end{split}\label{admm:dualupdate}
\end{align}

% As compare to the method of multipliers, which 
% The path-update step and the t-update step can be treated as a single \emph{Gauss-Seidel} pass~\cite{boyd2011distributed} over the two sets of variables, which is a approximately
% Given the dual variables, instead of jointly optimize $L_{\rho}$ given 
The path-update step~\eqref{admm:pathupdate} and the t-update step~\eqref{admm:tupdate} can be treated as an inexact minimization step for the primal minimization of all the primal variables with given dual variables. Then the dual variables are updated in~\eqref{admm:dualupdate} by a simple dual ascent step with step size $\rho$.
The first two steps are still complicated at the first glance. 
However, as we will discuss later, both the path-update step and the t-update step can be efficiently solved by decomposing them into small subproblems. 
% Therefore, by splitting the coupled variables $\vec{\beta}$, $\vec{\tau}$ with auxiliary variables $\vec{\beta}'$, $\vec{\tau}'$, we develop an ADMM based algorithm whose iteration can be efficiently solved by solving decoupled subproblems. 
% Next, we will discuss details on how to solve the path-update step and t-update step.
% We first remark some overall observations here and then discuss how to solve the first two steps later.
% Finally, the dual-update step~\eqref{admm:dualupdate} is simply a dual ascent step with step size $\rho$.
% Therefore, both path-

\noindent
\textbf{Solution for path-update step.}
In the path-update step~\eqref{admm:pathupdate}, we optimize over the path $\vec{x}$ and the auxiliary variables $\vec{\beta}'$ and $\vec{\tau}'$. 
For each edge $(i,j)\in \mathcal{E}$, the value of $g_{ij}$ only depends on $\beta_j'$ and $\tau_j'$. Therefore, we can separately optimize the function $g_{ij}$ for each $(i,j)$ and then obtain the solution of the path-update step by solving a shortest path problem with the optimal value of $g_{ij}$ as the weight for each edge. 
In particular, for each edge $(i,j)\in \mathcal{E}$, we observe the relevant terms in $g_{ij}$. The objective term~\eqref{gij:obj} is constant with respect to $\beta_j'$ and $\tau_j'$. The following terms~\eqref{gij:lamb}-\eqref{gij:tau} is a quadratic function with respect to both $\beta_j'$ and $\tau_j'$. Therefore, we can obtain the optimal values of $g_{ij}$ by finding the minimal value of a quadratic function within a interval. Therefore, for each $(i,j) \in \mathcal{E}$, the solutions are given by
\begin{align}
    \begin{split}
    \tilde{\tau}_j'^{k+1} &= \frac{1}{2} \tau_j^{k} + \frac{1}{2} (\tau_i^{k} + t_{ij}^{k} ) + \frac{1}{2\rho} ( \mu_{ij}^{\tau k} - \lambda_{ij}^{\tau k} ) \\
    \tau_j'^{k+1} &=  \Pi(\tilde{\tau}_j'^{k+1},\, 0,\,T) \\
    \tilde{\beta}_j'^{k+1} &= \frac{1}{2} \beta_j^{k} + \frac{1}{2}  \min \left\{ B, \beta_i^k - c_{ij}^{k}(t_{ij}^{k}, \beta_i^{k}) \right\}  + \frac{1}{2\rho} ( \mu_{ij}^{\beta k} - \lambda_{ij}^{\beta k} ) \\
    \beta_j'^{k+1} &=  \Pi(\tilde{\beta}_j'^{k+1},\, 0,\,B) \\
    \end{split}
\end{align}
Here, the projection function $\Pi(x, l, u)$ projects the value of $x$ to the interval $[l,u]$, i.e.,
\begin{align}
    \Pi(x, l, u) = \left\{  
    \begin{aligned}
        &l,\, &\text{if}\; x &< l \\
        &x,\, &\text{if}\; l &\leq x \leq u \\
        &u,\, &\text{if}\; x &> u
    \end{aligned}
    \right.
\end{align}
By substituting the updated $\tau_j'^{k+1}$, $\beta_j'^{k+1}$ back to $g_{ij}$ we obtain the new weight for edge $(i,j)$. We can then use those computed weights to solve a shortest path problem and obtain the updated path selection variable $\vec{x}$. 

\noindent
\textbf{Solution for t-update step.}
In the t-update step~\eqref{admm:tupdate}, we optimize over the variables $\vec{t}$, $\vec{\beta}$, and $\vec{\tau}$. By exploring the structure of $\mathcal{L}_{\rho}$, we can solve this step by decomposing it into a number of small subproblems with three variables $t_{ij}$, $\beta_i$ and $\tau_i$. 
In particular, for each selected edge pair $(l,i)$,$(i,j)$ such that $x_{li}=1$ and $x_{ij}=1$, we solve the following subproblem:\footnote{To deal with the case where $i=s$ is the origin, we additionally $x_{0s}=1$ and $\mu_{0s} = 0$. Then the subproblem also needs to be solved for $l=0$ and $i=s$. with additionally constraint $\beta_s = \beta_0$ and $\tau_s = 0$.}

\begin{align}
    \min_{\beta_i, t_{ij}, \tau_i} \; &F_{ij}(\beta_i, t_{ij}, \tau_i)   \label{admm:tupdate:obj}
     \\ & + L_{\rho}(\lambda^\beta_{ij}, \beta_j'^{k+1} - \min \left\{ B,  \beta_i - c_{ij}(t_{ij}, \beta_i) \right\} )  \label{admm:tupdate:lamb}
     \\ & + L_{\rho}(\lambda^\tau_{ij}, \tau_{j}'^{k+1} - \tau_i - t_{ij} )
     \\ & +  L_{\rho}(\mu^{\beta}_{li}, \beta_i - \beta_i'^{k+1} )  
     + L_{\rho}(\mu^{\tau}_{li}, \tau_i - \tau_i'^{k+1}) \label{admm:tupdate:mu}  \\
     \text{s.t.} \;& 0 \leq \beta_i \leq B, \quad t_{ij}^{lb} \leq t_{ij} \leq t_{ij}^{ub}, \quad 0 \leq \tau_i \leq T
      % + \mu^\tau_{ij} \left( \tau_i - \tau_i' \right)  + \frac{\rho}{2} \left( \tau_i - \tau_i' \right)^2
\end{align}
Note that the objective function of the above is slightly different from function $g_{ij}$. We use the index $i$ instead of $j$ in the additive term~\eqref{admm:tupdate:mu} and change the corresponding dual variables. We make this adjustment to make sure the above subproblem only depends on the three variables $t_{ij}$, $\beta_i$ and $\tau_i$. 

The objective of the above subproblem~\eqref{admm:tupdate:obj}-\eqref{admm:tupdate:mu} may have different forms for different types of edges. For example, $F_{ij} \equiv 0$ for the non-charging edge $(i,j) \in \mathcal{E}_w \cup \mathcal{E}_r$ and $c_{ij} \equiv 0$ for the waiting edge $(i,j) \in \mathcal{E}_w$. Therefore, the subproblem can be largely simplified for non-charging edges. For the charging edges, however, we encounter a non-convex term $F_{ij}$ in the objective, making the subproblem more difficult to solve. 
Fortunately, the subproblem has only three variables within a finite box (if we additionally add a constraint $t_{ij} \leq T$). 
One straightforward method is the exhaustive grid search to find the global minimum of the above subproblem with complexity 
$O\left( \left( \frac{\max\{B,T\}}{\epsilon} \right)^3 \right)$ 
where $\epsilon$ is the accuracy tolerance. In practice, we can use better ways to divide the search domain via e.g., Branch and Bound (BnB) or the DIviding Rectangles (DIRECT) method~\cite{jones1993lipschitzian,gablonsky2001locally}. 

% \noindent
% \textbf{Termination Condition.}
% Unfortunately, the convergence of ADMM is not guaranteed for non-convex problem. 

\noindent
\textbf{Time Complexity.}
% We summarize our approach in Algorithm~xxx. 
Let $n=|\mathcal{V}|$ be the number of nodes and $m=|\mathcal{E}|$ the number of edges in the graph. The path-update step involves updating the weights for edge each edge with complexity $O(m)$ and solving a shortest path problem with negative weights. If we use Bellman-Ford algorithm~\cite{bellman1958routing}, the complexity is $O(mn)$. The complexity of the t-update step is
$O\left( m \left( \max\{B,T\}/\epsilon \right)^3 \right)$.
The complexity is $O(m)$ for the dual-update step. 
Therefore, the overall time complexity of one iteration is $O\left(mn+ m \left( \max\{B,T\}/\epsilon \right)^3\right)$.

\noindent
\textbf{Discussions.}

% Note that the augmented Lagrangian $\mathcal{L}_\rho$ is the sum of the product of the path selection variable $x_{ij}$ and corresponding weight $g_{ij}$. 





==> arxivSource/arxiv/4.approach.tex <==
\section{An Efficient Algorithm with Performance Guarantee}\label{sec:method}

% \textcolor{blue}{TODO: need to add more discussion later.}
In this section, we develop an efficient dual-subgradient algorithm for solving the \textsf{CFO} problem with performance guarantee, by exploring the structural insights of the formulation in~\eqref{prob:cfo:a}.
% Its special structures allow us decompose the dual function into a number of small subproblems and a shortest path problem on an extended graph. We then update the dual variables by the subgradient method. 
% by exploring the problem structures of our novel problem formulation~\eqref{prob:cfo:a}. 
% We resort the partially-relaxed dual problem and solve the dual function given any dual variables. We then 

\subsection{The Dual Problem}

% \textcolor{blue}{TODO: need to add more discussion and words between the formulas.}
We obtain a partially-relaxed dual problem of \textsf{CFO} in~\eqref{prob:cfo:a} by relaxing  the constraints~\eqref{cons:cfoa:ddl} and~\eqref{cons:cfoa:soc0} with dual variable $\lambda_i^\tau$ and $\lambda_i^\beta$, respectively. The Lagrangian function is given by
\begin{align*}
    L(\vec{x}, \vec{y}, \vec{t}, \vec{\beta}, \vec{\tau}, \vec{\lambda}) =&  \sum_{i=1}^{N} \sum_{v\in \mathcal{V}_c}^{} \FvObj  \\
    & + \sum_{i=1}^{N+1} \lambda_i^\tau \delta_i^\tau(\vec{x}, \vec{y}, \vec{t}, \vec{\tau}) 
    +  \sum_{i=1}^{N+1} \lambda_i^\beta \delta_i^\beta(\vec{x}, \vec{y}, \vec{t}, \vec{\beta}),
\end{align*}
where $\vec{\lambda} = (\vec{\lambda}^\beta, \vec{\lambda}^\tau)$. The corresponding dual problem is given by
\begin{align}
    \max_{\vec{\lambda} \geq 0} D ( \vec{\lambda} ) = \max_{\vec{\lambda} \geq 0} 
    \min_{
        \substack{
        (\vec{x},\vec{y}) \in \mathcal{P},  \\ \vec{\beta} \in \mathcal{S}_{\alpha},  \vec{\tau}\in \mathcal{T}_\tau , \vec{t} \in \mathcal{T}
        }} L(\vec{x}, \vec{y}, \vec{t}, \vec{\beta}, \vec{\tau}, \vec{\lambda}).
        \label{prob:dual0}
\end{align}
Given $\vec{\lambda}$, we observe the problem of $D(\vec{\lambda})$ is a two-level problem where the inner level consists of a number of small subproblems and the outer level is a combinatorial problem over the feasible set $\mathcal{P}$. That is, 
\begin{subequations}
    \begin{align}
    D(\vec{\lambda}) & =
         D_1(\vec{\lambda})  
        + \min_{(\vec{x}, \vec{y})  \in \mathcal{P}} 
        \Biggl(  \sum_{i=1}^{N+1} \sumE x_e^i \underbrace{ \min_{t_e^i \in [t_e^{lb}, t_e^{ub}]} g_e^i(\vec{\lambda}, t_e^i) 
        }_{\text{speed planning}} \\
        + &  \sum_{i=1}^{N} \sumV y_v^i 
        \underbrace{
        \min_{\substack{
                t_c^{i,v} \in [0, t_c^{ub}], t_w^{i,v} \in [t_w^{lb}, t_w^{ub}], \\
                \beta_v^i \in [\beta^{lb}, B], \tau_v^i \in [0, T]
            }} 
        h_v^i(\vec{\lambda}, t_c^{i,v}, t_w^{i,v}, \beta_{v}^{i}, \tau_{v}^{i})  
        }_{\text{charging planning}}
        \Biggr) ,
       %  \\ & = D_1(\vec{\lambda}) +  \min_{(\vec{x},\vec{y}) \in \mathcal{P}} \sum_{i=1}^{N+1} \sum_{e\in \mathcal{E}}^{} w_e^i(\vec{\lambda}) x_e^i + \sum_{i=1}^{N} \sum_{v \in \mathcal{V}_c}^{} \sigma_v^i(\vec{\lambda}) y^i_v 
    \end{align} \label{prob:dual}
\end{subequations}
where $D_1(\vec{\lambda}) =  - \lambda_{N+1}^\tau T - \beta_0 \lambda^\beta_1$ is a constant for any given $\vec{\lambda}$ and
\begin{equation}
    g_e^i(\vec{\lambda}, t_e^i)  =  \lambda_i^\tau t_e^i + \lambda_i^\beta c^e(t_e^i)
    \label{func:g}
\end{equation}
represents the trade-off between the traveling time $t_e^i$ and the energy consumption $c_e(t_e^i)$ for each road segment $e\in \mathcal{E}$. The function
\begin{subequations}
    \begin{align}
        & h_v^i(\vec{\lambda}, t_c^{i,v}, t_w^{i,v}, \beta_v^i, \tau_v^i) 
         =  \FvObj + \lambda_{i+1}^\tau \left( t_w^{i,v} + t_c^{i,v} \right) \\
        &\qquad\quad  +  \left( \lambda_{i+1}^\tau - \lambda_{i}^\tau \right) \tau_v^i 
         % & + \left( \mu_i^{l} - \mu_{i+1}^{l} + \mu_i^{u} \right) \beta_v^i  
          + \left( \lambda_i^\beta - \lambda_{i+1}^\beta \right) \beta_v^i  
        % + \left( -\mu_{i+1}^{l} + \mu_i^{u}  \right) \phi_v(\beta_v^i, t_c^{i,v})
         -\lambda^\beta_{i+1} \phi_v\left(\beta_v^i, t_c^{i,v}\right)
    \end{align} \label{func:h}
\end{subequations}
represents the trade-off between the objective and the constraints. Next, we define 
\begin{subequations}
    \begin{align}
        w_e^i(\vec{\lambda}) &= \min_{t_e^i \in [t_e^{lb}, t_e^{ub}]} g_e^i(\vec{\lambda}, t_e^i), \label{prob:w} \\
        \sigma_v^i(\vec{\lambda}) &=  \min_{\substack{
                    t_c^{i,v} \in [0, t_c^{ub}], t_w^{i,v} \in [t_w^{lb}, t_w^{ub}], \\
                    \beta_v^i \in [\alpha B, B], \tau_v^i \in [0, T]
                }} 
            h_v^i(\vec{\lambda}, t_c^{i,v}, t_w^{i,v}, \beta_{v}^{i}, \tau_{v}^{i}). \label{prob:sigma}
    \end{align}
\end{subequations}
Here, $w_e^i(\vec{\lambda})$ can be computed by solving a single-variable convex optimization problem because $g_e^i(\vec{\lambda}, t_e^i)$ is convex with respect to $t_e^i$. The computation of $\sigma_v^i(\vec{\lambda})$ requires more effort, where we need to solve a 4-variable non-convex optimization problem over box constraints. Fortunately, the dimension of the subproblem~\eqref{prob:sigma} is fixed. Therefore, we can obtain $\sigma(\vec{\lambda})$ in $O( M^4/\epsilon_1^4 )$ with a Branch and Bound (BnB) scheme~\cite{boyd2007branch}. Here $M=\max\{ t_c^{ub}, t_w^{ub}, B, T\}$ is the diameter of the box constraint in subproblem~\eqref{prob:sigma} and $\epsilon_1$ is the accuracy.
% \textcolor{blue}{TODO: see details in Appendix~??.}

\noindent \textbf{Solving the Outer Level Problem.}
After solving the inner level subproblems~\eqref{prob:w} and \eqref{prob:sigma}, the dual function can be written as follows:
\begin{align}
    \hspace{-1mm} D(\vec{\lambda}) = & D_1(\vec{\lambda}) +  \min_{(\vec{x},\vec{y}) \in \mathcal{P}} \sum_{i=1}^{N+1} \sum_{e\in \mathcal{E}}^{} w_e^i(\vec{\lambda}) x_e^i + \sum_{i=1}^{N} \sum_{v \in \mathcal{V}_c}^{} \sigma_v^i(\vec{\lambda}) y^i_v. \label{prob:ilp}
\end{align}
The problem in~\eqref{prob:ilp}, at first glance, is an integer linear program (ILP) which is in general challenging to solve.
% In the outer problem~\eqref{prob:ilp}, 
However, after exploring the problem structure,
we can see that each charging station $v$ is associated with a cost $\sigma_v^i$ if it is the $i$-th charging stop, and each road segment $e$ is with a cost $w_e^i$ if it is in $i$-th subpath. Our goal is to find $N$ charging stops and $N+1$ subpaths with the minimum total cost. We observe that given any charging station selection, optimal subpaths can be determined by the shortest paths. Correspondingly, we can construct an extended graph consisting of $N$ layers of charging stations with cost $\sigma_v^i$ and edges between any two nodes in the consecutive layers with weight determined by the shortest paths. We can then find the optimal charge stop selection by the shortest path on the extended charging station graph. This idea leads to a novel two-level shortest path algorithm. 
%At first glance, this problem is challenging because it is a combinatorial problem with feasible set $\mathcal{P}$. Fortunately, by carefully exploring the problem structure, 
%We are able to solve the outer problem~\eqref{prob:ilp} by constructing an extended graph among the charge stations and apply a two-level shortest path algorithm on the extended graph.}

\begin{figure}[!tb]
    \resizebox{.7\linewidth}{!}{
    \input{figs/ex-ext-graph} 
    }
    \vspace*{-1mm}
    \caption{An example of the extended graph with $N=2$. In the original graph, we have two charging stations $u$ and $v$.}
    \vspace*{-1mm}
\end{figure}
   
In particular, we construct an extended graph $\mathcal{G}_{ex}=(\mathcal{V}_{ex}, \mathcal{E}_{ex})$, where the node set $\mathcal{V}_{ex}$ contains $s,d$ and $N$ copies of charging stations, i.e., 
\begin{align}
    \mathcal{V}_{ex} = \left\{ s,d \right\} \cup \left\{ v^i \, |v \in \mathcal{V}_c, i \in \left\{ 1,...,N \right\} \,   \right\}.
\end{align}
For each $u,v \in \mathcal{V}_c$ and $i\in \left\{ 1,...,N \right\}$, we construct an edge between $u^{i}$ and $v^{i+1}$ with cost 
$ \sigma_{u}^{i}(\vec{\lambda}) + SP^{i+1}(u, v)$
where $SP^{i+1}(u,v)$ is the cost of shortest path between $(u,v)$ on the original graph $\mathcal{G}$ with weight $w_e^{i+1}(\vec{\lambda})$. Similarly, we construct edges $(s,v^1), \forall v \in \mathcal{V}_c$ with weights $SP^1(s,v)$ and construct edges $(u^N, d), \forall v \in \mathcal{V}_c$ with weights $\sigma_v^{N} + SP^{N+1}(u^N, d)$.
By construction, we have the following lemma:

\begin{lemma}
    A shortest path on $\mathcal{G}_{ex}$ corresponds to an optimal solution to ILP problem in~\eqref{prob:ilp}.
\end{lemma}
% \begin{proof}
%     \textcolor{blue}{TODO} By construction, ...
% \end{proof}

Hence, we can solve the ILP problem~\eqref{prob:ilp} by applying a shortest path algorithm to the extended graph $\mathcal{G}_{ex}$ with low time complexity. 
Overall, given any $\vec{\lambda}$, we can compute the value of $D(\vec{\lambda})$ by first solving a number of subproblems~\eqref{prob:w} and~\eqref{prob:sigma} and then solving the outer problem~\eqref{prob:ilp} with shortest algorithms on an extended graph.

%     % \item Time complexity:
%     % \begin{itemize}
%     %     \item Shortest path for each CS pair: $O\left( (N+1) |\mathcal{V}_c| \left( |E|+|V|\log(|V|)\right)\right)$ (can be reduced)
%     %     \item Shortest path on the extended graph: $O(N |\mathcal{V}_c|^2)$
%     % \end{itemize}
% \end{itemize}



\subsection{A Dual Subgradient Algorithm}

% It is straightforward to verify that 
We use the dual subgradient method to iteratively update the dual variable $\vec{\lambda}$. In particular, we denote by $\vec{\lambda}[k]$ the dual variable at $k$-th iteration. Then we update the dual variable as follows:
\begin{subequations}
    \begin{align}
        % \lambda_i^\beta[k+1] &= \lambda_i^\beta[k] + \theta_k \left(\delta_i^\beta[k]\right)_+ \\
        % \lambda_i^\tau[k+1] &= \lambda_i^\tau[k] + \theta_k \left(\delta_i^\tau[k]\right)_+
        \lambda_i^\beta[k+1] &= \Biggl( \lambda_i^\beta[k] + \theta_k 
         \underbrace{ 
            \delta_i^\beta \left(\vec{x}^*[k], \vec{y}^*[k], \vec{t}^*[k], \vec{\beta}^*[k]\right)
        }_{\delta_i^\beta[k]}
          \Biggr)_+,  \\
        \lambda_i^\tau[k+1] &=\Biggl(\lambda_i^\tau[k] + \theta_k 
        \underbrace{
            \delta_i^\tau \left(\vec{x}^*[k], \vec{y}^*[k], \vec{t}^*[k], \vec{\tau}^*[k]\right)  }_{\delta_i^\tau[k]}
        \Biggr)_+.
    \end{align}\label{eq:dualupdate}
\end{subequations}
Here, $\vec{x}^*[k], \vec{y}^*[k], \vec{t}^*[k], \vec{\beta}^*[k], \vec{\tau}^*[k]$ are the solutions of the computed from the subproblems~\eqref{prob:ilp},~\eqref{prob:w}, and~\eqref{prob:sigma} with $\vec{\lambda}[k]$. 
The values $\delta_i^\beta[k]$ and $\delta_i^\tau[k]$ are thus the corresponding subgradients of $D(\vec{\lambda})$ for each components.
% $\delta_i^\beta[k]=\delta_i^\beta \left(\vec{x}^*[k], \vec{y}^*[k], \vec{t}^*[k], \vec{\beta}^*[k]\right)$
The notation $(a)_+$ denotes  $\max\{0,a\}$. The step size at $k$-th iteration is denoted as $\theta_k$. 

\input{algs/dualsub.tex}

The overall algorithm is summarized in Algorithm~\ref{alg:dualsub}.
From a high-level perspective, the dual variables $\vec{\lambda}$ can be interpreted as the price for the scheduled deadline and SoC. 
For example, a higher $\lambda^\beta_i$ gives more weight on the constraint $\delta_i^\beta$ and has multiple effects. First, it gives more weight for the energy cost in ~\eqref{func:g}, thus resulting in a larger traveling time in the edge subproblem~\eqref{prob:w}. Meanwhile, a higher $\lambda^\beta_i$ results in a lower scheduled SoC $\beta_v^i$ at $i$-th stop but a higher $\beta_v^{i-1}$ and more charging time $t_c^{i,v}$ at $(i-1)$-th stop. It means that a higher $\lambda^\beta_i$ results in a larger difference of scheduled $SoC$ between charging stops $(i-1)$ and $i$. A similar interpretation applies to the dual variable $\lambda^\tau_i$. 
Overall, Alg.~\ref{alg:dualsub} seeks to find a solution that balances the objective and the constraint cost and adjusts the dual variable via the subgradient direction.
% Despite \rev{???} having an intuitive interpretation, Alg.~\ref{alg:dualsub} always converges with a posterior performance bound as illustrated in the next subsection.
% In the next subsection, 

% The dual function $D(\vec{\lambda})$ is a weighted sum of the carbon footprint cost and the constraint cost. 
% \textcolor{blue}{TODO: More intuitive discussion...}
% The idea behind the update rule~\eqref{eq:dualupdate} is straightforward. 


\subsection{Performance Analysis}

% \textcolor{blue}{TODO: echo the abstract.}
% As one of the major contribution, 
In this subsection, as one of the key contributions, we show that (i) our algorithm always converges with a rate of $O(1/\sqrt{K})$ where $K$ is the number of iteration, (ii) each iteration only incurs polynomial-time complexity in graph size, and (iii) it generates optimal results if a condition is met and solutions with bounded loss otherwise.

\noindent \textbf{Convergence Rate.}
Similar to standard subgradient methods~\cite{boyd2003subgradient}, algorithm~\ref{alg:dualsub} also converges to dual optimal value at a rate of $O(1/\sqrt{K})$.

\begin{theorem}\label{thm:converge}
    Let $D^*$ be the optimal dual objective and let $\overline{D}_K$ be the maximum dual value over $K$ iterations in algorithm~\ref{alg:dualsub}. With constant step size $\theta_k = \frac{1}{\sqrt{K}}$, we have,  for some constant $C$,
    \begin{align}
        D^* - \overline{D}_K \leq \frac{C}{\sqrt{K}}.
    \end{align}
   
\end{theorem}
% \begin{proof}
%     See Appendix~\ref{sec:thm:converge}.
% \end{proof}
The proof is in Appendix~\ref{sec:thm:converge}. It shows that a constant step size $\theta_k=1/\sqrt{K}$ is sufficient to achieve a convergence rate of $O(1/\sqrt{K})$. However, one may achieve better empirical convergence by adaptively updating the step sizes~\cite{bazaraa1981Choice}. Besides, another improvement can be achieved by modifying the subgradient directions~\cite{camerini1975Improving}.

% \textcolor{blue}{TODO: Discussion on how to recover the primal solution.}

\noindent \textbf{Time Complexity.}
We summarize the time complexity analysis of Alg.~\ref{alg:dualsub} in the following Proposition.
\begin{proposition}\label{prop:complexity}
    The time complexity per iteration of Alg.~\ref{alg:dualsub} is 
    % $$O \left( \frac{1}{\epsilon_0^2}  \left( \left( N+1 \right) |\mathcal{V}_c| |\mathcal{V}| |\mathcal{E}| + N |\mathcal{V}_c| \frac{M^4}{\epsilon_1^4} \right)  \right)$$
    \begin{align}
        O  \left( \left( N+1 \right) |\mathcal{V}_c| |\mathcal{V}| |\mathcal{E}| + N |\mathcal{V}_c| \frac{M^4}{\epsilon_1^4} \right) \label{eq:complexity}
    \end{align},
    where $M = \left\{ t_c^{ub}, t_w^{ub}, B, T \right\}$ and $\epsilon_1$ is the required accuracy for solving the subproblems~\eqref{prob:sigma}
\end{proposition}
The proof is in Appendix~\ref{sec:prop:complexity}. 
Proposition~\ref{prop:complexity} states that at each iteration , Alg.~\ref{alg:dualsub} incurs only polynomial time complexity in graph size, albeit it requires solving the ILP subproblem in~\eqref{prob:sigma} optimally.
Meanwhile, Theorem~\ref{thm:converge} guarantees that Alg.~\ref{alg:dualsub} converges to a solution with accuracy $\epsilon_0$ in $O(1/\epsilon_0^2)$ iterations. We can derive the total time complexity of Alg.~\ref{alg:dualsub} by combining Proposition~\ref{prop:complexity} and Theorem~\ref{thm:converge}.
% Note that the major computational burden in practice comes from the first term in~\eqref{eq:complexity} which requires solving shortest path for all pairs of charging stations.

% We remark that the most time-consuming part is the computation of shortest path for all pairs of charging stations. 
% Therefore, our approach is parallelizable and enjoys the advantage of modern multi-core CPUs.

% In summary, after rearranging terms, the overall time complexity for running Algorithm~\ref{alg:dualsub} is given by
% $$O \left( \frac{1}{\epsilon_0^2}  \left( \left( N+1 \right) |\mathcal{V}_c| |\mathcal{V}| |\mathcal{E}| + N |\mathcal{V}_c| \frac{M^4}{\epsilon_1^4} \right)  \right)$$
% where $\epsilon_0$ is the accuracy for solving the dual problem~\eqref{prob:dual0}.


\noindent \textbf{Optimality Gap.}
Note that in the dual subgradient method, a convergence to dual optimal does not imply a convergence to the primal optimal as there might be a duality gap.
To this end, we provide the following bound on the optimality gap.
% Therefore, 
% To bound the op
\begin{theorem}\label{thm:optimal}
    Let OPT be the optimal objective to the problem in~\eqref{prob:cfo:a}.
    If Alg.~\ref{alg:dualsub} produces a feasible solution updated at iteration $k$ with objective ALG, then the optimality gap is bounded by
    \begin{align}
        ALG - OPT \leq  - \sum_{i=1}^{N+1} \left( \lambda_i^\beta[k] \delta_i^\beta[k] + \lambda_i^\tau[k] \delta_i^\tau[k] \right). \label{ineq:postbound}
    \end{align}
\end{theorem}
% \begin{proof}
%     See Appendix~\ref{sec:thm:optimal}.
% \end{proof}

% As reported later in Sec.~\ref{sec:simulation}, we observe that the computed posterior bounds are less than xx\%, suggesting good performance with favorable time complexity. 
The proof is in Appendix~\ref{sec:thm:optimal}. The posterior bound~\eqref{ineq:postbound} simply comes from the weak duality.
Meanwhile, we can compute it at each iteration in Alg.~\ref{alg:dualsub} and use it for early termination upon certain accuracy.
Moreover, Theorem~\ref{thm:optimal} also provides an optimality condition of the produced solution by the following corollary.
\begin{corollary}
    If Alg.~\ref{alg:dualsub} returns a feasible solution in line~\ref{alg:dualsub:optimal}, then the solution is optimal.
\end{corollary}

Note that Theorem~\ref{thm:optimal} requires Alg.\ref{alg:dualsub} to produce a feasible solution, which is not guaranteed in dual-based methods. In the case where Alg.\ref{alg:dualsub} does not find a feasible solution, we re-optimize the speed planning and charging planning with the given path in the last iteration of Alg.~\ref{alg:dualsub} and try to recover a feasible primal solution. As seen in Sec.~\ref{sec:simulation}, this recovery scheme always finds a feasible solution.
% We leave it as a future work to extend Alg.~\ref{alg:dualsub} to produce a guaranteed primal solution. 
% \com{JY}{Our current solution is very herustic, we will try to put it to appendix.}

% . Even worse, 

% In this section, we design an efficient dual-subgradient algorithm for solving a partially-relaxed dual problem of the two-truck platooning problem, in which only a subset of the constraints are relaxed. While a fully-relaxed dual problem is always convex, the partially-relaxed one is not. Indeed, it is still a combinatorial problem and can be challenging to solve. As a key contribution, we explore the problem structure to show that it can be solved optimally in polynomial time by a dual-subgradient algorithm. We derive a posterior bound on the optimality gap when a feasible primal solution is recovered from the dual optimal solution. We resort to the separate driving solution when no feasible primal solution is recovered.

%

% \input{4.1.ida.tex}
% \input{4.1.csg.tex}
% \input{4.1.expanded-graph.tex}

==> arxivSource/arxiv/5.simulation.tex <==
% \newpage
\section{Numerical Experiments}\label{sec:simulation}

\newcommand{\algcarbon}{\textsf{CARBON}}
\newcommand{\algenergy}{\textsf{ENERGY}}
\newcommand{\algfast}{\textsf{FAST}}
\newcommand{\algfastspeed}{\textsf{FAST-S}}
\newcommand{\algfastspeedcharge}{\textsf{FAST-SC}}



% \textcolor{blue}{TODO: add deviations of the performance elevation.}

% \textcolor{blue}{TODO: add comparison with MILP.}
% \textcolor{blue}{TODO: add ablation study. Need to add discussion.}

% \textcolor{blue}{TODO: add discussion on the battery life.}

% \textcolor{blue}{TODO: add comparison with MILP.}

In this section, we evaluate the performance of our algorithm by simulations using real-world traces over the US highway network. 
Our objectives are 
(i) to study the behavior of the carbon-optimized solutions.
(ii) to study the performance of the proposed approach as compare to  baselines and the impact of path planning, speed planning, charging planning, respectively; 
(iii) to study the impact of conservative ratio $\alpha$; 
(iv) to compare the carbon footprint between electric trucks and ICE trucks, and study the environmental benefit of electric trucks. 
% \textcolor{blue}{Need to revise.}

\subsection{Experiment Setup}

\begin{figure}
    \includegraphics[width=0.8\linewidth]{figs/carbon-map.pdf}
    \centering
    \resizebox{.8\linewidth}{!}{
    \begin{tabular}{lcccc}
    %\begin{tabularx}{\linewidth}{llcc}
        \toprule
        & \multicell{Carbon \\ footprint (kg)} & \multicell{Energy \\ (kWh)} & \multicell{Distance \\ (miles)} &  \multicell{Time \\ (hours)} \\
        \midrule
        \algfast & 1022.0 & 1633.7  & 919.9& 19.3 \\
        \algenergy & 637.3 & 1239.7 & 879.8& 24.0\\
        \algcarbon & 413.6 & 1487.5 & 946.9& 24.0\\
        % \algenergy & 637.3 (37.6\%) & 1239.7 (24.1\%) & 879.8& 24.0\\
        % \algcarbon & 413.6 (59.6\%) & 1487.5 (9.0\%) & 946.9& 24.0\\
        % Reduction  & 40.0\% & 16.6\% & -8\% & 0\%\\ 
       \bottomrule
    \end{tabular}
    }
    \caption{The illustration of carbon-optimized and energy-optimized solutions from Dallas, TX to Carmel, IN. 
    In the figure, the shaded area represents the period of charging process.
    % In the table, the third row is the relative reduction of \algcarbon~as compared to~\algfast.
    } \label{fig:ons-instance}
\end{figure}

\emph{Transportation network.} We collect the highway network data from the Map-based Educational Tools for Algorithm Learning (METAL) project~\cite{metalproject}. 
The constructed network consists of $84,504$ nodes and $178,238$ directed edges. We collect the real-time road speed data from HERE map~\cite{heremap}.
The grade of each road segment is derived from the elevations of its end nodes provided by the Shuttle Radar Topography Mission (SRTM)~\cite{farr2007shuttle} project. 
We also pre-process the road network and merge the adjacent road segments with similar grades with tolerance $0.5\%$ to reduce the computational complexity.
%The \textsf{NHS} graph is then pre-processed as follows: (i) non-intersection roads with the same grade (we use $0.4\%$ as the span of a grade level) are merged into a single road segment, and (ii) the ``eastern" US is divided into $22$ regions as shown in Fig.~\ref{fig:usa-map}, where the node nearest to each region's center is used as the source and destination nodes in the experiments. After pre-processing, the number of nodes is $38213$ and the number of edges (road segments) is $82781$. 
%

\emph{Energy consumption model.}
We use the simulator \emph{FASTSim}~\cite{gonderFuture2018} to collect the energy consumption data with driving speed (from $10$ mph to $70$ mph with a step of $0.2$ mph) at different grades (from $-6\%$ to $6\%$ with a step of $0.25\%$)\footnote{We note that the maximum grade allowed for the inter-state highway is a 6-meter difference in elevation every 100 meters road length in the United States~\cite{hancock2013policy}.}. 
Then we fit the energy consumption data with cubic polynomial functions. 
We use the parameters of Tesla Semi~\cite{teslaSemi} for the electric truck model with the battery capacity $B=1,000$ kWh and the total weight of $36$ tons. We assume the e-truck is fully charged at the origin, i.e., $\beta_0 = B$.
% The main parameters of the truck models are summarized in Table~\ref{tab:truckParam}. 

\emph{Origin-destination pair.} We collect origin-destination pairs from the Freight Analysis Framework (FAF)~\cite{hwang2016freight}. We select \numsim origin-destination pairs with distances longer than 800 miles. Those pairs represent 950 billion dollars of freight by trucks in 2017. 
Tab.~\ref{tab:src-des} illustrates a subset of the selected origin-destination pairs in the US starting from Los Angeles.
% Fig.~\ref{fig:src-des-map} illustrates a subset of the selected origin-destination pairs in the US start from California.

\input{tabs/src.des.tex}

\emph{Charging station data.}
%Since the charging station for electric trucks is currently rare, 
%we use the locations of fuel stations to represent the locations of charging stations.
We collect the location data of charging stations from the OpenStreetMap~(OSM)~\cite{OpenStreetMap} and add each location to the nearest road segment in the constructed graph.
The collected data yields $2,555$ charging stations.
% (with $\alpha=0.95$ in~\eqref{set:csedge}) for the charging station graph $\csgpre{G}$.
We approximate the charging functions with a piecewise linear function using six break points at $0\%, 80\%, 85\%, 90\%, 95\%, 100\%$ SoC~\cite{baumShortest2019}. 
The resulting charging function can charge the studied electric truck from $0\%$ to $80\%$ in $48$ minutes. See~Fig.\ref{fig:charge} for an illustration. 
We collect the electricity generation data from Energy Information Administration~(EIA)~\cite{eia2021monthly} and obtain a piecewise linear carbon intensity function $\pi(\cdot)$ for each charging station~(See Fig.~\ref*{fig:price-distri}).

\begin{figure*}[tb]
    \includegraphics[width=.95\linewidth]{figs/cfo-baseline-bar.pdf}
    \vspace{-5mm}
    \caption{Simulation results for \numsim instances. The carbon (energy) reduction is also computed with respect to \algfast. 
    % \textcolor{blue}{TODO: We are still waiting for more data.}
    } \label{fig:baseline}
\end{figure*}

% \begin{figure}
%     \includegraphics[width=.75\linewidth]{figs/src-des-map.pdf}
%     \caption{Selected origin-destination pairs start from California.}
%     \label{fig:src-des-map}
% \end{figure}

In the simulation, we implement and compare the following conceivable alternatives.

\trianglebullet\ \algcarbon: our carbon footprint minimizing approach. 

\trianglebullet\ \algenergy: our approach with the objective of minimizing energy consumption by setting the carbon intensity function $\pi(\cdot) \equiv 1$.

\trianglebullet\ \algfast: our approach with the objective of minimizing total travel and charging time by changing the objective and following the similar dualization procedure in Sec.~\ref{sec:method}.

\trianglebullet\ \algfastspeed: the same path of FAST with the speed planning.

\trianglebullet\ \algfastspeedcharge: the same path of FAST with the speed planning and charge planning.

\subsection{Behavior of Carbon-Optimized Solution}
We first study a transportation task from Dallas, TX to Carmel, IN. We compare the solution of \algfast, \algcarbon~and \algenergy~and present them in Fig.~\ref{fig:ons-instance}. We observe that \algcarbon~tends to "follow the sun and go with the wind" to charge the electricity with the low carbon intensity and achieves a 59.6\% carbon reduction as compared to \algfast~and 35.2\% as compared to \algenergy.
To achieve such a large carbon reduction, \algcarbon~charge a small amount of energy at the first and the third charging station to ensure the sufficient SoC on road while charge more at the second charging station for lower carbon footprint.
Meanwhile, the detour to the greener charging station leads to a slightly longer total distance and slightly more energy consumption as compared to the energy-optimized solution.
We find similar observations in the next subsection where we conduct the simulation over all 500 origin-destinations.
% The similar observations can be found in the next subsection 
% \textcolor{blue}{TODO: add discussion.}


% \trianglebullet\ FAST: the fastest path baseline. To ensure SoC feasibility, we construct an auxiliary \emph{charging station graph} $\mathcal{G}_a = ()$ where the set of node $\mathcal{V}_a$ contains $s,d$ and all the charging stations. We add an edge between two nodes $u,v \in \mathcal{V}_a$ if there is an SoC feasible path between $u,v$ without recharging. We compute and set the weight of each edge $(u,v)$ to the minimum traveling time from $u$ to $v$ with capacity limit $B$. We then apply a shortest path algorithm on $\mathcal{G}_a$ and obtain the location of charging stops. 
% We compute the speed planning and path planning decisions between two charging stations $u,v$ via solving an E2T2 problem~\cite{dengEnergyefficient2017} with the objective of minimizing traveling time subject to the capacity limit $B$. 
% We fully charge the battery at each charging stop.


% \subsection{Comparison with MIP formulation}
% \textcolor{blue}{Implement other methods in the literature? MIP can be difficult to implement. We might not have enough time...}

\subsection{Comparison with Baselines}

We then conduct simulations on \numsim~ origin~destination pairs. For each pair, we denote by $T_f$ the total travel time of \algfast~ and set deadlines from $1.1T_f$ to $1.5T_f$. We call the ratio between the deadline and $T_f$ the \emph{delay factor}.
The start time is set to 4 PM, Jan 1st, 2022. We set the number of charging stops $N$ of \algcarbon~and \algenergy~the same as \algfast. 
{In these typical settings, the number of charging stops is no more than eight.} 
We set the ratio of conservative lower bound $\alpha=0.05$. 
\algcarbon~produces feasible solutions for $96\%$ of all instances. 
For infeasible solutions, we increase $\alpha$ until it produces a feasible solution. A maximum value of $\alpha=0.12$ guarantees \algcarbon~ to produce feasible solutions for all instances.

% \begin{figure}[tb]
%     \includegraphics[width=.9\linewidth]{figs/cfo-bar.pdf}
%     \caption{Traveling time and carbon footprint comparison among baselines for a typical origin-destination pair from California to Ohio with deadline $64$ hours. IDA-C saves $27\%$ carbon footprint as compared to fastest path~(FAST) and saves $9\%$ carbon footprint as compared to minimizing energy only (IDA-E). 
%     %\textcolor{blue}{TODO:!!! The data in this whole section may not be the final numbers/figures. I put it here just for illustration purpose.} 
%     } \label{fig:barplot}
%     \vspace{-1mm}
% \end{figure}



% \noindent \textbf{Discussion on $\alpha$.} Throughout the simulation, 


We show the simulation results in Fig.~\ref{fig:baseline}.
All the results are mean values over \numsim origin-destination pairs and the error bars represent the standard deviations. Fig.~\ref{fig:baseline}(a) and Fig.~\ref{fig:baseline}(b) give the the carbon (resp. energy) reduction of different baselines as compared to \algfast. We observe that as the deadline gets relaxed, the carbon (and energy) reduction of all the baselines increases. 
Moreover, different components of the design space contribute differently into such reduction as we shall discuss in the following.

\noindent\textbf{Benefit of Carbon-Optimized Solution.}
We first compare \algcarbon~and \algenergy.
As shown in Fig.~\ref{fig:baseline}(a), while the carbon footprint of both approaches decrease as the deadline increases, \algcarbon~benefits more from the relaxed deadline and achieves higher carbon reduction.
In particular, , \algcarbon~achieves {19\%} carbon reduction as compared to \algfast~baseline under the typical setting when the delay factor is $1.2$ and up to {28\%} when the delay factor is $1.5$.
Meanwhile, as compared to its energy-efficient counterpart \algenergy, \algcarbon~achieves {9\%} carbon reduction when the delay factor is $1.2$ and {13\%} when the delay factor is $1.5$.
% and achieves \textcolor{blue}{xx\%} carbon reduction as compared to its energy-efficient counterpart \algenergy.
This difference mainly comes from the fact that minimizing energy simply ignores the temporal diversity of the renewable and loses part of the optimization space.
Therefore, minimizing energy consumption does not necessarily lead to a minimum carbon footprint. It is essential to consider the carbon footprint objective when studying the environmental impact of e-trucks.
Meanwhile, we also observe from Fig.~\ref{fig:baseline}(b) that the difference of energy reduction between \algcarbon~and \algenergy~is less than {3\%}.
This means that a carbon-efficient route is also energy-efficient.

\noindent\textbf{Impact of Speed Planning.} We then investigate \algfastspeed~to study the impact of speed planning. When the delay factor is $1.2$. \algfastspeed~saves {15\%} carbon footprint and {12\%} energy as compared to \algfast. As compared to \algenergy, \algfastspeed~saves {3\%} additional carbon footprint. This additional saving comes from the fact that the optimized speed plan re-schedules the travel time of each stage such that the e-truck charges greener electricity at each stage.

\noindent\textbf{Impact of Charging Planning.} We then compare \algfastspeed~and \algfastspeedcharge~to study the impact of charging planning. We observe that when the delay factor is $1.2$, \algfastspeedcharge~saves {2.5\%} additional carbon footprint as compared to \algfastspeed ~because \algfastspeedcharge~takes the advantage of charging planning such that the e-truck can wait for the lower carbon intensity.

\noindent\textbf{Impact of Path Planning.} We then compare \algfastspeedcharge~and \algcarbon~to study the impact of path planning.
We observe that when the delay factor is $1.2$, \algcarbon~saves {2\%} additional carbon footprint as compared to \algfastspeedcharge~because e-truck can select greener charging stations with path planning.

% \textcolor{blue}{TODO: still waiting for the data.}

% We observe that as the deadline gets relaxed, the total spent time of both \algcarbon and \algenergy increase as expected (Fig.~\ref{fig:baseline}(a)). Meanwhile, the two algorithms behave differently in allocating the extra time. While \algenergy tends to spend more time traveling on road and drive slowly to reduce energy consumption, \algcarbon utilizes the extra time from the relaxed deadline to both save energy and wait for cleaner electricity.

% We also compare the energy consumption and present the results in Fig.~\ref{fig:baseline}(b). We observe that as the deadline increases, both \algenergy and \algcarbon save more energy as compared to FAST. Meanwhile, the difference of energy reduction is less than 2\% between \algenergy and \algcarbon. 
% This means that a carbon-efficient route is also energy-efficient.

% We observe that when the delay factor is 
% In particular, under a typical setting when the delay factor is $1.2$

% Fig.~\ref{fig:baseline}(a) gives the normalized time mix of \algenergy and \algcarbon with respect to FAST. 
% Fig.~\ref{fig:baseline}(b) and Fig.~\ref{fig:baseline}(c) respectively give the relative carbon reduction and relative energy reduction of \algcarbon and \algenergy with respect to FAST. 

% The results are 

% \textcolor{blue}{TODO: discussion on $\alpha$?}
% We set the conservative ratio $\alpha=0.05$

% \subsection{Impact of Truck Departure Time}
% 
% In this subsection, we study the impact of truck departure time.
% 
% \begin{figure}[tb]
%     \includegraphics[width=.8\linewidth]{figs/cfo-st.pdf}
%     \caption{Comparison of carbon footprint under different departure time.} \label{fig:departure}
%     \vspace{-1mm}
% \end{figure}

\subsection{Impact of Conservative Ratio $\alpha$}

\begin{figure}[tb]
    \centering
    \includegraphics[width=.7\linewidth]{figs/alpha.pdf}
    \vspace*{-4mm}
    \caption{Impact of conservative ratio $\alpha$. 
        % \textcolor{blue}{Might be updated later.} 
    }\label{fig:alpha:performance}
    % \vspace*{-4mm}
\end{figure}

In this subsection, we study the impact of the conservative ratio $\alpha$. We run \algcarbon~on \numsim origin-destination pairs for $\alpha$ ranging from $0.0$ to $0.12$. 
{For each $\alpha$, we check the SoC at each road segment of the solutions and report the percentage of  solutions violating positive SoC among all \numsim origin-destination pairs. In addition, we notice that \textsf{CFO} with $\alpha=0$ (named $\textsf{CFO}_{0}$) provides a lower bound to the \textsf{CFO} with positive SoC constraints at all road segments but no reservation requirement. We thus define performance loss of \algcarbon~with \textsf{CFO} as its relative error with respect to the \algcarbon~with $\textsf{CFO}_{0}$, i.e.,
$$
\text{Performance Loss} = \frac{ALG_{\alpha}-ALG_{0}}{ALG_{0}},
$$
where $ALG_{\alpha}$ is the objective value of solutions by \algcarbon~for \textsf{CFO}.
The results are presented in Fig.~\ref{fig:alpha:performance}. }
We observe that when $\alpha=0$, there are {26\%} of infeasible solutions while a small increment of $\alpha$ leads to a large feasibility improvement, e.g., $\alpha=0.02$ with {12\%} of infeasible solutions. 
We observe that $\alpha=0.12$ is sufficient to guarantee feasibility for all \numsim origin-destination pairs. Meanwhile, we observe the performance loss introduced by $\alpha$ grows almost linearly with respect to $\alpha$. In a typical selection when $\alpha=0.06$, $96\%$ of solutions are feasible while the performance loss is only {$3.3\%$}. In the most conservative case when $\alpha=0.12$ that guarantees the feasibility of all the solutions, the performance loss is {$6.7\%$}.
Thus, by introducing the conservative ratio $\alpha$, we significantly simplify the coupling SoC constraint while ensuring feasibility with minor performance loss.

% \textcolor{blue}{TODO: Need to update the numbers when more results are ready.}



\subsection{Comparison with ICE Trucks}

In this subsection, we study the environmental benefits of electric trucks as compared to ICE trucks. 
We use the parameters of Kenworth T800 trailer~\cite{kenworthT800} for the ICE truck model with the same total weight of $36$ tons. 
For the ICE truck, we compute the energy-efficient path plan and speed plan by the dual-based method in~\cite{dengEnergyefficient2017}.
We use the \coo\ factor value of diesel  from EIA~\cite{eiaCO2Factors} to transform the fuel consumption of the ICE truck to its direct carbon emission. The data suggest that if an ICE truck is powered by diesel, it will produce 9.88 kg \coo\ per gallon, or equivalently 0.25 kg \coo\ emission per kWh.
The simulation results are presented in Tab.~\ref{tab:ice:cmp}. We observe that the e-truck saves 55.9\% carbon as compared to the ICE truck under a delay factor $1.2$.

There are several factors that contribute to such carbon reduction. First, e-trucks consume less energy due to the high efficiency of electric motors and the regenerative braking system. 
Second, with the increasing integration of renewable generations for e-truck charging, the carbon footprint of an electric truck reduces. 
Third, our joint optimization of path planning, speed planning and charging planning leads an e-truck to charge clean electricity with low carbon intensity. 
Overall, these factors together lead to a significant reduction of the carbon footprint of the electric truck as compared to the ICE truck.

% \begin{figure}[tb]
%     \includegraphics[width=.8\linewidth]{figs/cfo-ice-bar.pdf}
%     \caption{Comparison of carbon footprint of ICE truck and electric truck.} \label{fig:ice}
%     \vspace{-1mm}
% \end{figure}

\input{tabs/ice-cmp.tex}


==> arxivSource/arxiv/6.discussion.tex <==
\section{Discussion}

% \textcolor{blue}{TODO.}

\noindent\textbf{Battery Degradation.} The modeling and prediction of battery degradation is in general difficult and still an active research area~\cite{hu2020battery}. Among many factors that affects the battery degradation, the most relevant ones for the transportation tasks are charge or discharge rate and the depth of discharge (DoD)~\cite{pelletier2017battery}. 
A high charge rate or a high DoD may accelerate the battery degradation.
To prolong the battery lifetime, we can add a battery degradation cost in the objective. 
We can model different charging mode by adding multiple charging stations at the same location, where a charging mode with the higher rate incur higher degradation cost.
To prevent large DoD, we can also add a degradation cost if the arrival SoC is lower than certain value.

% There are many factors that affects battery degradation 

% \noindent\textbf{Imperfect Knowledge of Traffic Condition and Carbon Intensity.}
\noindent\textbf{Dynamic Traffic Condition.}
% \noindent\textbf{Imperfect Knowledge of Traffic Condition and Carbon Intensity.}
% 
In the real world, the traffic conditions can be time-varying. To adapt variable traffic conditions in our formulation, we can incorporate the phase-based traffic model~\cite{xuRide2019} into our stage-expanded graph, where the traffic condition is approximately static at each phase. 
Then we can treat the combination of the stage and the traffic phase as the new stage and apply our approach.
% We leave it as a future direction to consider imperfect information of traffic condition.
% \textcolor{blue}{TODO: add more discussion.} 

\noindent\textbf{Applications Beyond CFO.}
We remark that our approach has applications beyond this paper. For example, it is also applicable to general routing problem for electric/ICE vehicles with energy consumption and monetary objective. 
Our approach is also applicable to the subproblem for electric vehicle routing problem (EVRP) in a branch-price-and-cut framework~\cite{desaulniersExact2016}.
% We conclude this paper with several interesting future directions {including (i) involving dynamic traffic condition and (ii) handling uncertain carbon footprint function due to the fluctuated renewable generation.} 
% (i) In the real world, the traffic conditions can be time-varying while our current formulation does not consider such variable traffic conditions. We leave it as a future direction to adapt variable traffic conditions in the formulation. (ii) As many generalized RSP~\cite{dengEnergyefficient2017,liuEnergyEfficient2018} is weakly NP-hard and admits fully polynomial-time approximation scheme (FPTAS), it is an interesting question that if CFO is also weakly NP-hard. Note that existing study~\cite{strehler2017energy} does not simply apply to CFO due to the non-convex carbon footprint objective. 
% There are several interesting future directions. For example, how to adapt the model with dynamic traffic conditions, and how to select the number of charging stops, etc.
% The formulation and algorithm are general and applicable to other electric mobility and energy storage management problems.
% is applicable to general scenarios for electric 

% Future Directions:
% \begin{itemize}
%     \item Adapt dynamic traffic condition.
%     \item More sophisticated way to recover primal solution.
%     \item Extension to discard the SoC simplification assumption.
%     \item Better ways to select the number of charging stops.
%     \item Bound optimality loss introduced by $\alpha$.
%     \item Is CFO weakly NP-hard?
%     \item Better way to solve the non-convex subproblem.
%     \item Comparison with other methods in the literature.
% \end{itemize}

==> arxivSource/arxiv/7.1.alt.comare.tex <==

\subsection{Discussion on Alternative Approaches}\label{sec:novelty}
% \com{JY}{Move it to the appendix later? Keep it for now for proof reading.}

In the first alternative,
%  follows a different direction of approaching CFO. 
we directly formulate the CFO problem as a Mixed Integer Programming (MIP). Then we apply an general-purpose method for MIP (e.g., branch and bound) to the formulated problem. As a general observation, the first alternative does not explore the problem structure and only works for problems with hundreds of variables. It usually incurs significant computational burden in larger problems.

The second alternative involves constructing a time-expanded and battery-expanded graph similar in~\cite{strehler2017energy}. For each node $v\in \mathcal{V}$, we add some copies $v_{\beta,\tau}$ of $v$ to the expanded graph. Each copy $v_{\beta,\tau}$ represents a specific SoC $\beta$ and arrival time $\tau$. We add an new edge between $u_{\beta_1, \tau_1}$ and $v_{\beta_2, \tau_2}$ if there is an edge between $(u,v)$ on the original graph and there is a feasible speed choice that corresponds to energy consumption $\beta_2 - \beta_1$ and travel time $\tau_2 - \tau_1$. 
If $v\in \mathcal{V}_c$ is a charging station, we then add an edge between $v_{\beta_1,\tau_1}$ and $v_{\beta_2,\tau_2}$ that corresponds to certain charging decisions. We also assign corresponding weight to this type of edge accordingly. Then the CFO problem can be transformed to a shortest path problem and solved via standard shortest path algorithms e.g., Dijkstra algorithm. 
Although the formulated problem is simple, the second alternative has the drawback that it may exclude feasible solutions of the original problem for inaccurate discretization and may even disconnect origin and destination~\cite{strehler2017energy}. 
Therefore, the constructed expanded graph can be significantly larger than the original graph, and becomes intractable for long-haul tasks. 

% The second alternative is an improvement for the first alternative (e.f., second row of Tab.~\ref{tab:related-method}). 
% Instead of expanding the original graph, we expand the \emph{charging station graph} that only takes $ \tilde{\mathcal{V}}_c = \left\{ s,d \right\} \cup \mathcal{V}_c$ as its set of node. For the expanded graph, we follow the similar procedure to add several copies to the new graph and construct new edges. For any pair of node $(u_{\beta_1,\tau_1}, v_{\beta_2, \tau_2})$ in the expanded graph, we add an edge between them if there is an energy-efficient path between them with the energy consumption less than $\beta_2 - \beta_1$ and travel time less than $\tau_2 - \tau_1$. 
% As compared to the first alternative, the second alternative has less requirement on the accuracy because of larger decision space on the edge. Moreover, the expanded graph size is smaller if $|\mathcal{V}_c| << |\mathcal{V}|$. 
% However, the construction of the expanded graph requires to solve NP-hard E2T2 problem for each pair of charging stations, which does not scale to large-scale network.

The third alternative combines the two directions together. 
We use the battery-expanded graph to deal with the nonlinearity of the energy consumption function and the charging function. If the carbon-intensity function is piecewise linear, then the CFO problem can be formulated as an Mixed Integer Linear Program (MILP) which is less complex than the MIP in the first alternative. We can apply a branch and cut method to the MILP and obtain solutions.
Similar idea can be found in~\cite{fernandez2022arc}.
Similar to the first alternative, the third alternative resorts to solve a MILP with a general-purpose method. It still incurs large computational burden as the problem size grows because MILP is challenging to solve.

Overall, the conceivable alternatives have high model complexity or fail to explore the problem structure, leading to overall high time complexity. In contrast, our novel problem formulation in~\eqref{prob:cfo:a} keeps a low-complexity model and reveals an elegant problem structure that allows us design an dual-subgradient algorithm that has good performance theoretically and empirically.

==> arxivSource/arxiv/7.conclusion.tex <==
% \section{Concluding Remarks}
\section{Conclusion}

In this paper, we present the first study in the literature on the \emph{Carbon Footprint Optimization} (CFO) problem of a heavy-duty e-truck traveling from an origin to a destination across a national highway network subject to a hard deadline, by optimizing path planning, speed planning, and intermediary charging planning.
We show that the problem is NP-hard and under practical settings it is equivalent to finding a generalized RSP on a novel stage-expanded graph, which extends the original transportation graph to model charging options. 
Our problem formulation incurs low model complexity and reveals a problem structure that leads us to an efficient dual-subgradient algorithm with a strong performance guarantee.
Extensive simulation results over the US national highway network show that our solutions reduce up to 28\% carbon footprint compared to the baseline alternatives.
The results also demonstrate the carbon efficiency of e-trucks over ICE trucks.
% Future directions include dynamic traffic condition and imperfect carbon intensity prediction.
% The results also show that the e-truck can achieve 56\% carbon reduction as compared to its ICE counterpart.



==> arxivSource/arxiv/8.ack.tex <==
\section*{Acknowledgement}
% \begin{acks}
The authors would like to thank the anonymous reviewers for their insightful comments that help further improve this work. 
The work presented in this paper was supported in part by a General Research Fund from Research Grants Council, Hong Kong (Project No. 14207520).
% \end{acks}


==> arxivSource/figs/ex-ext-graph.tex <==

\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
    thick,main node/.style={circle,draw,font=\sffamily\Large\bfseries}]

    \node[main node] (s) {$s$};
    \node[main node] (u1) [above right of=s] {$u^1$} ;
    \node[main node] (u2) [right of=u1] {$u^2$};
    \node[main node] (v1) [below right of=s] {$v^1$} ;
    \node[main node] (v2) [right of=v1] {$v^2$};
    \node[main node] (d) [above right of=v2] {$d$};

    % \node[main node] (d) [right of=3] {d};

    % need to add library \usetikzlibrary{positioning}
    % \node [below =0mm and 1.5mm of 2, ] {\footnotesize{$\substack{t_c^1, t_w^1, \\ \beta^1_{v_1}, \tau^1_{v_1},  y_{v_1}^1=1}$}};
    % \node [below =0mm and 1.5mm of 3, ] {\footnotesize{$\substack{t_c^2, t_w^2, \\ \beta^2_{v_2}, \tau^2_{v_2},  y_{v_2}^2=1}$}};
    % \node [below =0mm and 1.5mm of 4, ] {\footnotesize{$\beta^3, \tau^3=T$}};

    \path[every node/.style={font=\sffamily\small}]
    (s) edge  node [above, rotate=45]  {\footnotesize{$\text{SP}^1(s,u)$}} (u1) 
    (s) edge  node [below, rotate=-45] {\footnotesize{$\text{SP}^1(s,v)$}} (v1) 
    (u1) edge  node [anchor=center, above left, midway, rotate=-55] {\footnotesize{$\sigma^1_u + \text{SP}^2(u,v)$}} (v2) 
    (u1) edge  node [anchor=center, above, midway] {\footnotesize{$\sigma^1_u$}} (u2) 
    (v1) edge  node [anchor=center, above, midway] {\footnotesize{$\sigma^1_v$}} (v2) 
    (v1) edge  node [anchor=center, above left, midway, rotate=55]  {\footnotesize{$\sigma^1_v + \text{SP}^2(v,u)$}} (u2) 
    (u2) edge  node [anchor=center, above, midway, rotate=-45]  {\footnotesize{$\sigma^2_u + \text{SP}^3(u,d)$}} (d) 
    (v2) edge  node [anchor=center, above, midway, rotate=45]  {\footnotesize{$\sigma^2_v + \text{SP}^3(v,d)$}} (d) 
    ;
    % (2) edge [bend left] node [above] {$\vec{x}^2, \vec{t}^2$} (3)
    % (3) edge [bend left] node [above] {$\vec{x}^3, \vec{t}^3$} (4);
                
\end{tikzpicture}

==> arxivSource/figs/ex-subpath.tex <==

\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2cm,
thick,main node/.style={circle,draw,font=\sffamily\Large\bfseries}]

    \node[main node] (1) {s};
    \node[main node] (2) [right of=1] {$v_1$} ;
    \node[main node] (3) [right of=2] {$v_2$};
    \node[main node] (4) [right of=3] {d};
    % need to add library \usetikzlibrary{positioning}
    \node [below =0mm and 1.5mm of 1, ] {\footnotesize{$\substack{t_c^0=0, t_w^0=0, \\ \beta^0_{s}=\beta_0, \tau^0_{s}=0}$}};
    \node [below =0mm and 1.5mm of 2, ] {\footnotesize{$\substack{t_c^1, t_w^1, \\ \beta^1_{v_1}, \tau^1_{v_1},  y_{v_1}^1=1}$}};
    \node [below =0mm and 1.5mm of 3, ] {\footnotesize{$\substack{t_c^2, t_w^2, \\ \beta^2_{v_2}, \tau^2_{v_2},  y_{v_2}^2=1}$}};
    \node [below =0mm and 1.5mm of 4, ] {\footnotesize{$\beta^3, \tau^3=T$}};

    \path[every node/.style={font=\sffamily\small}]
    (1) edge [bend left] node [above] {$\vec{x}^1, \vec{t}^1$} (2) 
    (2) edge [bend left] node [above] {$\vec{x}^2, \vec{t}^2$} (3)
    (3) edge [bend left] node [above] {$\vec{x}^3, \vec{t}^3$} (4);
            
\end{tikzpicture}
    

==> arxivSource/tabs/co2-fuel.tex <==
\begin{table}[!tb]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lllll}
        \toprule
        & Coal & Natural gas & Petroleum & Renewable \\
        \midrule
        Carbon Intensity (kg/kWh) & 1.02 & 0.39 & 0.91 & 0 \\
        Total emission (tons) & 7.86 $\times 10^8$ & 6.35 $\times 10^8$& 1.6 $\times 10^7$ & 0\\
        Electricity (kWh) & 7.73 $\times 10^{11}$ & 1.62$\times 10^{12}$ & 1.75 $\times 10^{10}$ & $7.92\times 10^{11}$  \\
        \bottomrule
    \end{tabular}
    } % end of resizebox
    \vspace{1mm}
    \caption{U.S electricity generation and resulting \coo\ emissions by major type of source in 2020~\cite[Tab.~7.2a, Tab.~11.6]{eia2021monthly}}\label{tab:fuel-co2}
    \vspace{-6mm}
\end{table}

==> arxivSource/tabs/graph-size.tex <==
\begin{table}[htb]
    \begin{tabular}{lll}
        \toprule
     & \#nodes & \#edges \\
     \midrule
    Original graph & 84,504 & 178,238 \\
    Charging station graph & 2,555 & 787,259 \\
    Expanded graph & ?? & ?? \\
    \bottomrule
    \end{tabular}
    \caption[]{Size of different graphs.}
\end{table}

==> arxivSource/tabs/ice-cmp.tex <==

\begin{table}[tb]
    \centering
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccc}
        \toprule
        Delay Factor & 1.1 & 1.2 & 1.3 & 1.4 & 1.5 \\
        \midrule
        \algenergy  & 50.8\% & 51.4\% & 52.4\% & 53.6\% & 54.1\% \\
        \algcarbon  & 54.7\% & 55.9\% & 57.1\% & 58.3\% & 59.2\% \\
        \bottomrule
    \end{tabular}
    % } % end of resizebox
    \vspace{1mm}
    \caption{Average carbon reduction with respect to ICE truck over \numsim~origin-destination pairs.}\label{tab:ice:cmp}
    \vspace{-6mm}
\end{table}

==> arxivSource/tabs/method-novelty-old.tex <==

\newcommand\tikzmark[1]{%
    \tikz[remember picture]  \coordinate (#1){};%
}
% \newcommand{\multicell}[1]{\begin{tabular}[c]{@{}c@{}} #1 \end{tabular}}
% \newcommand{\multicellleft}[1]{\begin{tabular}[l]{@{}l@{}} #1 \end{tabular}}
\newcommand{\cmark}{\ding{51}}% \usepackage{pifont}
\newcommand{\xmark}{\ding{55}}%
\resizebox{\linewidth}{!}{
\begin{NiceTabular}{llll | lll}
\toprule
Graph Model in Formulation & Problem & $\#$Variables & \multicell{$\#$Constraints} & Algorithm & Complexity & Optimality \\ \midrule
% \cite{baumShortest2019} &Charging function propagating & Generalized RSP &  $|\mathcal{V}| + |\mathcal{E}|$ & - & Exponential & Exact \\
% Label setting + discrete decisions & \xmark & Exponential & - \\
% \cite{strehler2017energy} & FPTAS & Generalized RSP &  $|\mathcal{V}| + |\mathcal{E}|$ & - & Polynomial & Pre-set $\epsilon$ \\
% \multicellleft{Label-setting with \\ decision discretization} & Generalized RSP  & $ O\left( K^{|\mathcal{V}|} \right)^\dagger$ & - & Exponential & Subject to $K$ \\ \hline
Original graph  & MIP & $ O \left( |\mathcal{V}| + |\mathcal{E}| \right)$ & $ O\left( |\mathcal{V}| + |\mathcal{E}| \right) $ & Branch and bound  & Exponential & Optimal \\ \midrule
\multicellleft{Battery-expanded graph} & MILP$^\dagger$ & \tikzmark{milpVar} $ O \left( B / \epsilon \left( |\mathcal{V}| + |\mathcal{E}| \right)\right)$ & $ O \left( B / \epsilon \left( |\mathcal{V}| + |\mathcal{E}| \right)\right)$ & Branch and cut & Exponential & Optimal \\ \midrule
\multicellleft{Time-expanded and \\ battery-expanded graph} &  Shortest Path &  \tikzmark{spVar}  $  \left( (T \cdot B)/\epsilon^2 \right) \left(|\mathcal{V}| + |\mathcal{E}| \right)$ &  $ \left( (T \cdot B)/\epsilon^2 \right) \left(|\mathcal{V}| + |\mathcal{E}| \right)$ & Bellman-Ford  & Polynomial &  $O(\epsilon)$ to optimal \\ \midrule
% \multicellleft{Time-expanded and \\ battery-expanded \\ charging station graph} & Shortest Path & $ \left( (T \cdot B)/\epsilon^2 \right) |\mathcal{V}_c|^2 $ & - & Polynomial & Subject to $\epsilon$ \\ \hline
% \cite{fernandez2022arc} & Expanded graph &  ILP & $ \left( B/\epsilon \right) |\mathcal{E}| $ & $ \left( B/\epsilon \right) |\mathcal{E}| $  & Exponential & - \\
% \midrule
\textbf{Our stage-expanded graph} & Generalized RSP$^{\ddagger}$ & \tikzmark{ourVar} $O\left( N |\mathcal{E}| + N |\mathcal{V}| \right)$ & $O\left( N \left( |\mathcal{E}| + |\mathcal{V}| \right) \right)$ & \multicell{Dual subgradient}  & Polynomial & Posterior bound \\ \bottomrule 
\end{NiceTabular}
}
\footnotesize{$^{\dagger}$: Provided that the carbon intensity function is approximated by a piecewise linear function. \quad $^\ddagger$: RSP stands for restricted shortest path.}


\tikzset{arrow/.style ={draw, line width=1.5pt,dashed}}
% \newcommand{\drawArrowTxt}[2]{
%     \node[draw=none,red,anchor=west,text width=3cm] at ($(#1.east)+(0.8cm,0)$) {#2};
%     \draw [red,arrow]  ($(#1.east)+(0.8cm,0)$) -- +(-0.5cm,0);
% }
\begin{tikzpicture}[remember picture,overlay,->]
    \draw[red] (milpVar) -- (spVar);
    % \drawArrowTxt{milpVar}{Table legend} 
\end{tikzpicture}


==> arxivSource/tabs/method-novelty.tex <==

\newcommand\tikzmark[1]{%
    \tikz[remember picture]  \coordinate[anchor=center] (#1){};%
}
\definecolor{m1color}{rgb}{0.36, 0.54, 0.66}
\definecolor{m2color}{rgb}{1.0, 0.49, 0.0}
% \newcommand{\multicell}[1]{\begin{tabular}[c]{@{}c@{}} #1 \end{tabular}}
% \newcommand{\multicellleft}[1]{\begin{tabular}[l]{@{}l@{}} #1 \end{tabular}}
\newcommand{\cmark}{\ding{51}}% \usepackage{pifont}
\newcommand{\xmark}{\ding{55}}%
\resizebox{\linewidth}{!}{
\begin{NiceTabular}{lll| lll}
\toprule
Graph Model in Formulation & Problem & Model Complexity & Algorithm & Complexity & Optimality \\ \midrule
% \cite{baumShortest2019} &Charging function propagating & Generalized RSP &  $|\mathcal{V}| + |\mathcal{E}|$ & - & Exponential & Exact \\
% Label setting + discrete decisions & \xmark & Exponential & - \\
% \cite{strehler2017energy} & FPTAS & Generalized RSP &  $|\mathcal{V}| + |\mathcal{E}|$ & - & Polynomial & Pre-set $\epsilon$ \\
% \multicellleft{Label-setting with \\ decision discretization} & Generalized RSP  & $ O\left( K^{|\mathcal{V}|} \right)^\dagger$ & - & Exponential & Subject to $K$ \\ \hline
Original graph  & MIP & $ O \left( |\mathcal{V}| + |\mathcal{E}| \right)$ &  \tikzmark{mipAlg}Branch and bound  & \multicellleft{Exponential to \\ $|\mathcal{V}|$ and $|\mathcal{E}|$}  & Optimal \\ \midrule
\multicellleft{Battery-expanded graph} & MILP$^\dagger$ & \tikzmark{milpVar} $ O \left( B / \epsilon \left( |\mathcal{V}| + |\mathcal{E}| \right)\right)$ & Branch and cut  & \multicellleft{Exponential to \\ $|\mathcal{V}|$, $|\mathcal{E}|$, and $B/\epsilon$}& $O(\epsilon)$ to optimal  \tikzmark{milpOptEnd} \\ \midrule
\multicellleft{Time-expanded and \\ battery-expanded graph} &  Shortest Path &  \tikzmark{spVar}  $  \left( (T \cdot B)/\epsilon^2 \right) \left(|\mathcal{V}| + |\mathcal{E}| \right)$ &  Bellman-Ford  & \multicellleft{Polynomial to \\ $|\mathcal{V}|, |\mathcal{E}|, T/\epsilon \text{ and } B/\epsilon$} &  $O(\epsilon)$ to optimal \\ \midrule
% \multicellleft{Time-expanded and \\ battery-expanded \\ charging station graph} & Shortest Path & $ \left( (T \cdot B)/\epsilon^2 \right) |\mathcal{V}_c|^2 $ & - & Polynomial & Subject to $\epsilon$ \\ \hline
% \cite{fernandez2022arc} & Expanded graph &  ILP & $ \left( B/\epsilon \right) |\mathcal{E}| $ & $ \left( B/\epsilon \right) |\mathcal{E}| $  & Exponential & - \\
% \midrule
\textbf{Our stage-expanded graph} & Generalized RSP$^{\ddagger}$ & \tikzmark{ourVar} $O\big( N \left(|\mathcal{E}| + |\mathcal{V}| \right) \big)$ \tikzmark{ourVarEnd} & \tikzmark{ourAlg}\multicell{Dual subgradient}  & \multicellleft{Polynomial to \\ $|\mathcal{V}|, |\mathcal{E}|, \text{ and } N$} & Posterior bound \tikzmark{ourAlgEnd}\\ \bottomrule 
\end{NiceTabular}
}
\raggedright % left aligned
\footnotesize{$^{\dagger}$: Provided that the carbon intensity function is approximated by a piecewise linear function. \quad $^\ddagger$: RSP stands for restricted shortest path.}
\\ \textcolor{m1color}{\textbf{Message 1:}} Compared with battery-expanded graphs, our stage-expanded graph has a low model complexity because th number of stages $N\leq 10$ in practice.
\\ \textcolor{m2color}{\textbf{Message 2:}} Compared with MIP formulations, our formulation reveals an elegant problem structure that leads to an efficient algorithm with favorable performance.

\tikzset{arrow/.style ={draw, line width=1.5pt,dashed}}
% \newcommand{\drawArrowTxt}[2]{
%     \node[draw=none,red,anchor=west,text width=3cm] at ($(#1.east)+(0.8cm,0)$) {#2};
%     \draw [red,arrow]  ($(#1.east)+(0.8cm,0)$) -- +(-0.5cm,0);
% }

% \newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=2pt] (char) {#1};}}
\begin{tikzpicture}[remember picture,overlay,->]
    % the rectangle for message 1
    \node[draw=m1color,circle,inner sep=1pt] at ([xshift=1mm, yshift=1mm] ourVarEnd) {\tiny\bf\textcolor{m1color}{1}};
    \draw[m1color,line width=1.2pt] ([xshift=-3mm,yshift=3mm]milpVar.north west) rectangle ([yshift=-1mm,xshift=3mm]ourVarEnd.south);

    % the first rectangle for message 2
    \draw[m2color,line width=1.2pt] ([xshift=-6mm,yshift=4mm]mipAlg.north) rectangle ([yshift=-3mm,xshift=-7mm]milpOptEnd.south);
    \node[draw=m2color,circle,inner sep=1pt] at ([xshift=-5mm, yshift=7mm] milpOptEnd) {\tiny\bf\textcolor{m2color}{2}};

    % the second rectangle for message 2
    \draw[m2color,line width=1.2pt] ([xshift=-6mm,yshift=6mm]ourAlg.north) rectangle ([yshift=-3mm,xshift=-7mm]ourAlgEnd.south);
    \node[draw=m2color,circle,inner sep=1pt] at ([xshift=-5mm, yshift=1mm] ourAlgEnd) {\tiny\bf\textcolor{m2color}{2}};

    % \drawArrowTxt{milpVar}{Table legend} 
\end{tikzpicture}


==> arxivSource/tabs/notation.tex <==

\begin{table}[!tb]
    \centering
    % \resizebox{\linewidth}{!}{
    % } % end of resizebox
    \begin{tabularx}{\linewidth}{ll}
        \toprule
        Notation & Definition \\
        % & Coal & Natural gas & Petroleum & Renewable \\
        \midrule
        \midrule
        $\mathcal{G} $ & The original transportation graph \\
        $\mathcal{V}_c $ & The set of charging stations \\
        $\tilde{\mathcal{V}}_c $ & The set of charging stations and source and destination  \\
        $\mathcal{G}_s$ & The stage-expanded graph \\
        $\mathcal{G}_{ex}$ & The extended graph for solving the ILP~\eqref{prob:ilp} \\
        \midrule 
        \midrule 
        $s,d$ & The source and destination respectively \\
        $\beta_0$ & The initial SoC \\
        $T$  & The deadline constraint \\
        $B$ & The battery capacity \\
        $N$ & The maximum number of charging stops\\
        \midrule
        \midrule
        $c_e(t)$ & The energy consumption at road segment $e$  \\
        $\phi_v(t_c, \beta_v)$ & The SoC increment function \\
        $\pi_v(\tau)$ & The carbon intensity at node $v$ \\
        $F_v(\beta, t_c, \tau)$ & The carbon footprint objective \\
        \midrule
        \midrule
        $t_e^i$ & \multicellleft{The travel time at road segment $e$ at stage $i$} \\
        % \midrule
        $t_w^{i,v}$ & \multicellleft{The waiting time at charging station $v$ at stage $i$ } \\
        % \midrule
        $\beta_v^i$ & The arrival SoC at charing station $v$ at stage $i$  \\
        $\tau_v^i$ & The arrival time at charing station $v$ at stage $i$  \\
        \midrule
        $x_e^i$ & \multicellleft{The binary variable that selects  a road segment $e$ \\ at stage $i$} \\
        \midrule
        $y_v^i$ & \multicellleft{The binary variable that selects a charging station $v$ \\ at stage $i$} \\
        \bottomrule
    \end{tabularx}
    \caption{Key notations.}\label{tab:notation}
\end{table}

==> arxivSource/tabs/related-ev.tex <==

\newcommand{\cmark}{\ding{51}}% \usepackage{pifont}
\newcommand{\xmark}{\ding{55}}%
\newcommand{\multicell}[1]{\begin{tabular}[c]{@{}c@{}} #1 \end{tabular}}

%\begin{table*}[!tb]
\begin{tabular}{lccccccc}
    \toprule
Work & \multicell{Speed \\ Planning} & \multicell{Path \\ Planning} & \multicell{Deadline \\ Constraint} & \multicell{Partial \\ Recharge} & \multicell{Nonlinear \\ Recharge} & \multicell{Time\\ Varying Obj.} & Obj. \\ \midrule
\cite{eisnerOptimal2011,sachenbacherEfficient2011,baumEnergyoptimal2013} & \xmark & \cmark & \xmark & N/A & N/A & \xmark & energy \\
\cite{celaEnergy2014b,liuConstrained2017} & \xmark & \cmark & \cmark & N/A & N/A & \xmark & energy \\
\cite{storandtQuick2012} & \xmark & \cmark & \cmark & \xmark & \xmark & \xmark & energy \\
\cite{baumShortest2019} & \xmark & \cmark & \xmark & \cmark & \cmark & \xmark & time \\
\cite{wangContextAware2013} & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & time \\
\cite{goodrichTwophase2014,kobayashi2011route} & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & time/energy \\
\cite{sweda2017adaptive} & \xmark & \cmark & \xmark & \cmark & \cmark & \xmark & energy \\
\cite{liu2014joint} & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & monetary cost \\
\midrule %%%%%%%%%%%%%%%%%%% ----------------
\cite{dengEnergyefficient2017,liuEnergyEfficient2018,xuRide2019} & \cmark  & \cmark & \cmark & N/A  & N/A & \xmark & energy   \\ 
\cite{baumModeling2020, baumSpeedConsumption2014} & \cmark & \cmark & \cmark & N/A & N/A & \xmark & time/energy \\
\cite{floresOptimal2015} & \cmark & \xmark & \xmark & N/A & N/A & \xmark & energy \\
\cite{fontanaOptimal2013,hartmannEnergyEfficient2014} & \cmark & \cmark & \xmark & N/A & N/A & \xmark & energy \\
%\cite{hartmannEnergyEfficient2014} & \cmark & \cmark & \xmark & N/A & N/A & \xmark & energy \\
%\cite{lvSpeed2016} & \cmark & \xmark & \xmark & N/A & N/A & \xmark & time \\ % solar-powered, recharging during the route 
\cite{strehler2017energy} & \cmark & \cmark & \xmark & \cmark & \cmark & \xmark & time/energy \\
\textbf{This work} & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & carbon footprint \\
\bottomrule
\end{tabular}
%\end{table*}

==> arxivSource/tabs/related-method.tex <==



\newcommand{\multicell}[1]{\begin{tabular}[c]{@{}c@{}} #1 \end{tabular}}
\newcommand{\cmark}{\ding{51}}% \usepackage{pifont}
\newcommand{\xmark}{\ding{55}}%
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
Work & Approach & Formulated Problem & $\#$Variables & \multicell{$\#$Constraints} & Complexity & Optimality \\ \midrule
\cite{baumShortest2019} &Charging function propagating & Generalized RSP &  $|\mathcal{V}| + |\mathcal{E}|$ & - & Exponential & Exact \\
% Label setting + discrete decisions & \xmark & Exponential & - \\
\cite{strehler2017energy} & FPTAS & Generalized RSP &  $|\mathcal{V}| + |\mathcal{E}|$ & - & Polynomial & Pre-set $\epsilon$ \\
\cite{strehler2017energy} & Expanded graph & Shortest Path & $ \left( B/\epsilon \right) \left(|\mathcal{V}| + |\mathcal{E}| \right)^{\dagger} $ & - & Polynomial & Subject to $\epsilon$ \\
\cite{montoyaElectric2017} & Meta-heuristic & MILP & $ O \left(  K|\mathcal{V}| + |\mathcal{E}| \right)^{\dagger\dagger} $ & $ O\left( K|\mathcal{V}| + |\mathcal{E}| \right) $ & Exponential & - \\
\cite{fernandez2022arc} & Expanded graph &  ILP & $ \left( B/\epsilon \right) |\mathcal{E}| $ & $ \left( B/\epsilon \right) |\mathcal{E}| $  & Exponential & - \\
\textbf{This work} & Lagrangian relaxation  & Generalized RSP & $O\left( N |\mathcal{E}| + N |\mathcal{V}| \right)^\ddagger$ & $O\left( N   |\mathcal{E}| + N |\mathcal{V}|  \right)$ & Polynomial & Posterior bound \\ \bottomrule 
\end{tabular}
}
\footnotesize{$^\dagger$: $B$ is the value of capacity limit. $\epsilon$ is the tolerance of discretization. \quad $^{\dagger\dagger}$: $K$ is the number of breaking points in piece-wise linear approximation. \\ $^\ddagger$: $N$ is the number of charging stops during the trip. }



==> arxivSource/tabs/related-truck.tex <==

\newcommand{\cmark}{\ding{51}}% \usepackage{pifont}
\newcommand{\xmark}{\ding{55}}%
% \newcommand{\multicell}[1]{\begin{tabular}[c]{@{}c@{}} #1 \end{tabular}}

\begin{tabular}{lccccll}
    \toprule
    & \multicell{Speed Planning} & \multicell{Path Planning} & \multicell{Deadline Constraint} & \multicell{Charging Planning} & \multicell{Truck Type} & Objective  \\ \midrule
%     & \multicell{Speed \\ Planning} & \multicell{Path \\ Planning} & \multicell{Deadline \\ Constraint} & \multicell{Charging \\ Planning} & \multicell{Truck \\ Type} & Objective  \\ \midrule    
    RSP~\cite{hassin1992approximation,lorenz2001simple,juttner2001lagrange} & \xmark & \cmark & \cmark & N/A & ICE & Path cost \\
    E2T2~\cite{dengEnergyefficient2017,liuEnergyEfficient2018,xuRide2019,zhou2020minimizing} & \cmark & \cmark & \cmark & N/A & ICE & Energy/Emission \\
    %\cite{eisnerOptimal2011,sachenbacherEfficient2011,baumEnergyoptimal2013} & \xmark & \cmark & \xmark & N/A & energy \\
    %\cite{celaEnergy2014b,liuConstrained2017} & \xmark & \cmark & \cmark & N/A & & energy \\
    %\cite{storandtQuick2012} & \xmark & \cmark & \cmark & \xmark & & energy \\
    %\cite{baumShortest2019} & \xmark & \cmark & \xmark & \cmark & time \\
    %\cite{wangContextAware2013} & \xmark & \cmark & \xmark & \xmark & time \\
    %\cite{goodrichTwophase2014,kobayashi2011route} & \xmark & \cmark & \xmark & \xmark & time/energy \\
    % \cite{sweda2017adaptive} & \xmark & \cmark & \xmark & \cmark & energy \\
    %\cite{liu2014joint} & \xmark & \cmark & \xmark & \xmark & monetary cost \\ 
    % \cite{baumModeling2020, baumSpeedConsumption2014} & \cmark & \cmark & \cmark & N/A & Electric & Time/Energy \\
    % \cite{floresOptimal2015} & \cmark & \xmark & \xmark & N/A & energy \\
    % \cite{fontanaOptimal2013,hartmannEnergyEfficient2014} & \cmark & \cmark & \xmark & N/A & energy \\
    % \cite{baek2020battery} & \xmark & \cmark & \xmark &  \\
    many, e.g.,~\cite{hellstrom2009look} & \cmark & \xmark & \xmark & N/A & ICE & Energy \\
    many, e.g.,~\cite{strehler2017energy} & \cmark & \cmark & \xmark & \cmark & Electric/Hybrid & Time/Energy \\
    many, e.g.,~\cite{zhang2022optimal} & \cmark & \xmark & \cmark & \xmark & Electric & Energy \\
    \textbf{This work} & \cmark & \cmark & \cmark & \cmark  & Electric & Carbon footprint \\ \bottomrule
\end{tabular}

%\begin{tabular}{lcccccc}
%\toprule
%Work & \multicell{Speed \\ Planning} & \multicell{Path \\ Planning} & \multicell{Deadline \\ Constraint} & \multicell{Partial \\ Recharge} & \multicell{Nonlinear \\ Recharge} &  Obj. \\ \midrule
%\cite{eisnerOptimal2011,sachenbacherEfficient2011,baumEnergyoptimal2013} & \xmark & \cmark & \xmark & N/A & N/A & energy \\
%\cite{celaEnergy2014b,liuConstrained2017} & \xmark & \cmark & \cmark & N/A & N/A &  energy \\
%\cite{storandtQuick2012} & \xmark & \cmark & \cmark & \xmark & \xmark &   energy \\
%\cite{baumShortest2019} & \xmark & \cmark & \xmark & \cmark & \cmark &  time \\
%\cite{wangContextAware2013} & \xmark & \cmark & \xmark & \cmark & \xmark & time \\
%\cite{goodrichTwophase2014,kobayashi2011route} & \xmark & \cmark & \xmark & \xmark & \xmark &  time/energy \\
%\cite{sweda2017adaptive} & \xmark & \cmark & \xmark & \cmark & \cmark &  energy \\
%\cite{liu2014joint} & \xmark & \cmark & \xmark & \cmark & \xmark & monetary cost \\
%\midrule %%%%%%%%%%%%%%%%%%% ----------------
%\cite{dengEnergyefficient2017,liuEnergyEfficient2018,xuRide2019} & \cmark  & \cmark & \cmark & N/A  & N/A &  energy   \\ 
%\cite{baumModeling2020, baumSpeedConsumption2014} & \cmark & \cmark & \cmark & N/A & N/A  & time/energy \\
%\cite{floresOptimal2015} & \cmark & \xmark & \xmark & N/A & N/A &  energy \\
%\cite{fontanaOptimal2013,hartmannEnergyEfficient2014} & \cmark & \cmark & \xmark & N/A & N/A & energy \\
%%\cite{hartmannEnergyEfficient2014} & \cmark & \cmark & \xmark & N/A & N/A & \xmark & energy \\
%%\cite{lvSpeed2016} & \cmark & \xmark & \xmark & N/A & N/A & \xmark & time \\ % solar-powered, recharging during the route 
%\cite{strehler2017energy} & \cmark & \cmark & \xmark & \cmark & \cmark & time/energy \\
%\textbf{This work} & \cmark & \cmark & \cmark & \cmark & \cmark & carbon footprint \\
%\bottomrule
%\end{tabular}

==> arxivSource/tabs/result-cmp.tex <==

\begin{table}[!tb]
    \centering
    \begin{tabularx}{\linewidth}{lXXX}
        \toprule
        & FAST & IDA-E & IDA-C \\
        \midrule
    Carbon footprint (tons) & 1.763 & 1.346  & 1.281 \\
    Travel time (hours) & 34.51 & 48.70 & 45.43  \\
    Charge time (hours) & 10.00 & 4.25 & 4.43  \\
    Wait time (hours) & 1.25 & 1.41 & 3.58  \\
    \bottomrule
    \end{tabularx}
    \vspace{1mm}
    \caption{Average performance for different algorithms among 1,000 origin-destination pairs. }\label{tab:res-cmp}
\end{table}

==> arxivSource/tabs/src.des.tex <==
\begin{table}[tb]
    % \newcommand{\multicell}[1]{\begin{tabular}[c]{@{}c@{}} #1 \end{tabular}}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{llcc}
    %\begin{tabularx}{\linewidth}{llcc}
        \toprule
        Origin & Destination & \multicell{Distance \\ (miles)} & \multicell{Value \\ (billion USD)}  \\
        \midrule
        Los Angeles CA & Columbus OH & 1977 & 17.725 \\
        Los Angeles CA & Dallas-Fort Worth TX  & 1240 & 12.247 \\
        Los Angeles CA & Chicago IL & 1745 & 11.293 \\
        Los Angeles CA & Nashville TN & 1780 & 10.718 \\
        Los Angeles CA & Houston TX & 1373 & 7.837 \\
        % Los Angeles CA & Mississippi & 1644.644 & 7.417 \\
        % Los Angeles CA & New York & 2452.625 & 6.781 \\
        % Los Angeles CA & Atlanta GA & 1936.714 & 6.517 \\
        % Los Angeles CA & Detroit MI & 1982.850 & 6.491 \\
        % Los Angeles CA & Rest of TN & 2058.301 & 5.966 \\
       \bottomrule
    \end{tabular}
    }
    \vspace{1mm}
    \caption{Five popular origin-destination pairs from Los Angeles.}\label{tab:src-des}
    \vspace{-10mm}
\end{table}

==> figs/ex-subpath.tex <==

\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2cm,
thick,main node/.style={circle,draw,font=\sffamily\Large\bfseries}]

    \node[main node] (1) {s};
    \node[main node] (2) [right of=1] {$v_1$} ;
    \node[main node] (3) [right of=2] {$v_2$};
    \node[main node] (4) [right of=3] {d};
    % need to add library \usetikzlibrary{positioning}
    \node [below =0mm and 1.5mm of 1, ] {\footnotesize{$\substack{t_c^0=0, t_w^0=0, \\ \beta^0_{s}=\beta_0, \tau^0_{s}=0}$}};
    \node [below =0mm and 1.5mm of 2, ] {\footnotesize{$\substack{t_c^1, t_w^1, \\ \beta^1_{v_1}, \tau^1_{v_1},  y_{v_1}^1=1}$}};
    \node [below =0mm and 1.5mm of 3, ] {\footnotesize{$\substack{t_c^2, t_w^2, \\ \beta^2_{v_2}, \tau^2_{v_2},  y_{v_2}^2=1}$}};
    \node [below =0mm and 1.5mm of 4, ] {\footnotesize{$\beta^3, \tau^3=T$}};

    \path[every node/.style={font=\sffamily\small}]
    (1) edge [bend left] node [above] {$\vec{x}^1, \vec{t}^1$} (2) 
    (2) edge [bend left] node [above] {$\vec{x}^2, \vec{t}^2$} (3)
    (3) edge [bend left] node [above] {$\vec{x}^3, \vec{t}^3$} (4);
            
\end{tikzpicture}
    

==> tabs/graph-size.tex <==
\begin{table}[htb]
    \begin{tabular}{lll}
        \toprule
     & \#nodes & \#edges \\
     \midrule
    Original graph & 84,504 & 178,238 \\
    Charging station graph & 2,555 & 787,259 \\
    Expanded graph & ?? & ?? \\
    \bottomrule
    \end{tabular}
    \caption[]{Size of different graphs.}
\end{table}

==> tabs/method-novelty-old.tex <==

\newcommand\tikzmark[1]{%
    \tikz[remember picture]  \coordinate (#1){};%
}
% \newcommand{\multicell}[1]{\begin{tabular}[c]{@{}c@{}} #1 \end{tabular}}
% \newcommand{\multicellleft}[1]{\begin{tabular}[l]{@{}l@{}} #1 \end{tabular}}
\newcommand{\cmark}{\ding{51}}% \usepackage{pifont}
\newcommand{\xmark}{\ding{55}}%
\resizebox{\linewidth}{!}{
\begin{NiceTabular}{llll | lll}
\toprule
Graph Model in Formulation & Problem & $\#$Variables & \multicell{$\#$Constraints} & Algorithm & Complexity & Optimality \\ \midrule
% \cite{baumShortest2019} &Charging function propagating & Generalized RSP &  $|\mathcal{V}| + |\mathcal{E}|$ & - & Exponential & Exact \\
% Label setting + discrete decisions & \xmark & Exponential & - \\
% \cite{strehler2017energy} & FPTAS & Generalized RSP &  $|\mathcal{V}| + |\mathcal{E}|$ & - & Polynomial & Pre-set $\epsilon$ \\
% \multicellleft{Label-setting with \\ decision discretization} & Generalized RSP  & $ O\left( K^{|\mathcal{V}|} \right)^\dagger$ & - & Exponential & Subject to $K$ \\ \hline
Original graph  & MIP & $ O \left( |\mathcal{V}| + |\mathcal{E}| \right)$ & $ O\left( |\mathcal{V}| + |\mathcal{E}| \right) $ & Branch and bound  & Exponential & Optimal \\ \midrule
\multicellleft{Battery-expanded graph} & MILP$^\dagger$ & \tikzmark{milpVar} $ O \left( B / \epsilon \left( |\mathcal{V}| + |\mathcal{E}| \right)\right)$ & $ O \left( B / \epsilon \left( |\mathcal{V}| + |\mathcal{E}| \right)\right)$ & Branch and cut & Exponential & Optimal \\ \midrule
\multicellleft{Time-expanded and \\ battery-expanded graph} &  Shortest Path &  \tikzmark{spVar}  $  \left( (T \cdot B)/\epsilon^2 \right) \left(|\mathcal{V}| + |\mathcal{E}| \right)$ &  $ \left( (T \cdot B)/\epsilon^2 \right) \left(|\mathcal{V}| + |\mathcal{E}| \right)$ & Bellman-Ford  & Polynomial &  $O(\epsilon)$ to optimal \\ \midrule
% \multicellleft{Time-expanded and \\ battery-expanded \\ charging station graph} & Shortest Path & $ \left( (T \cdot B)/\epsilon^2 \right) |\mathcal{V}_c|^2 $ & - & Polynomial & Subject to $\epsilon$ \\ \hline
% \cite{fernandez2022arc} & Expanded graph &  ILP & $ \left( B/\epsilon \right) |\mathcal{E}| $ & $ \left( B/\epsilon \right) |\mathcal{E}| $  & Exponential & - \\
% \midrule
\textbf{Our stage-expanded graph} & Generalized RSP$^{\ddagger}$ & \tikzmark{ourVar} $O\left( N |\mathcal{E}| + N |\mathcal{V}| \right)$ & $O\left( N \left( |\mathcal{E}| + |\mathcal{V}| \right) \right)$ & \multicell{Dual subgradient}  & Polynomial & Posterior bound \\ \bottomrule 
\end{NiceTabular}
}
\footnotesize{$^{\dagger}$: Provided that the carbon intensity function is approximated by a piecewise linear function. \quad $^\ddagger$: RSP stands for restricted shortest path.}


\tikzset{arrow/.style ={draw, line width=1.5pt,dashed}}
% \newcommand{\drawArrowTxt}[2]{
%     \node[draw=none,red,anchor=west,text width=3cm] at ($(#1.east)+(0.8cm,0)$) {#2};
%     \draw [red,arrow]  ($(#1.east)+(0.8cm,0)$) -- +(-0.5cm,0);
% }
\begin{tikzpicture}[remember picture,overlay,->]
    \draw[red] (milpVar) -- (spVar);
    % \drawArrowTxt{milpVar}{Table legend} 
\end{tikzpicture}


==> tabs/related-ev.tex <==

\newcommand{\cmark}{\ding{51}}% \usepackage{pifont}
\newcommand{\xmark}{\ding{55}}%
\newcommand{\multicell}[1]{\begin{tabular}[c]{@{}c@{}} #1 \end{tabular}}

%\begin{table*}[!tb]
\begin{tabular}{lccccccc}
    \toprule
Work & \multicell{Speed \\ Planning} & \multicell{Path \\ Planning} & \multicell{Deadline \\ Constraint} & \multicell{Partial \\ Recharge} & \multicell{Nonlinear \\ Recharge} & \multicell{Time\\ Varying Obj.} & Obj. \\ \midrule
\cite{eisnerOptimal2011,sachenbacherEfficient2011,baumEnergyoptimal2013} & \xmark & \cmark & \xmark & N/A & N/A & \xmark & energy \\
\cite{celaEnergy2014b,liuConstrained2017} & \xmark & \cmark & \cmark & N/A & N/A & \xmark & energy \\
\cite{storandtQuick2012} & \xmark & \cmark & \cmark & \xmark & \xmark & \xmark & energy \\
\cite{baumShortest2019} & \xmark & \cmark & \xmark & \cmark & \cmark & \xmark & time \\
\cite{wangContextAware2013} & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & time \\
\cite{goodrichTwophase2014,kobayashi2011route} & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & time/energy \\
\cite{sweda2017adaptive} & \xmark & \cmark & \xmark & \cmark & \cmark & \xmark & energy \\
\cite{liu2014joint} & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & monetary cost \\
\midrule %%%%%%%%%%%%%%%%%%% ----------------
\cite{dengEnergyefficient2017,liuEnergyEfficient2018,xuRide2019} & \cmark  & \cmark & \cmark & N/A  & N/A & \xmark & energy   \\ 
\cite{baumModeling2020, baumSpeedConsumption2014} & \cmark & \cmark & \cmark & N/A & N/A & \xmark & time/energy \\
\cite{floresOptimal2015} & \cmark & \xmark & \xmark & N/A & N/A & \xmark & energy \\
\cite{fontanaOptimal2013,hartmannEnergyEfficient2014} & \cmark & \cmark & \xmark & N/A & N/A & \xmark & energy \\
%\cite{hartmannEnergyEfficient2014} & \cmark & \cmark & \xmark & N/A & N/A & \xmark & energy \\
%\cite{lvSpeed2016} & \cmark & \xmark & \xmark & N/A & N/A & \xmark & time \\ % solar-powered, recharging during the route 
\cite{strehler2017energy} & \cmark & \cmark & \xmark & \cmark & \cmark & \xmark & time/energy \\
\textbf{This work} & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & carbon footprint \\
\bottomrule
\end{tabular}
%\end{table*}

==> tabs/related-method.tex <==



\newcommand{\multicell}[1]{\begin{tabular}[c]{@{}c@{}} #1 \end{tabular}}
\newcommand{\cmark}{\ding{51}}% \usepackage{pifont}
\newcommand{\xmark}{\ding{55}}%
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
Work & Approach & Formulated Problem & $\#$Variables & \multicell{$\#$Constraints} & Complexity & Optimality \\ \midrule
\cite{baumShortest2019} &Charging function propagating & Generalized RSP &  $|\mathcal{V}| + |\mathcal{E}|$ & - & Exponential & Exact \\
% Label setting + discrete decisions & \xmark & Exponential & - \\
\cite{strehler2017energy} & FPTAS & Generalized RSP &  $|\mathcal{V}| + |\mathcal{E}|$ & - & Polynomial & Pre-set $\epsilon$ \\
\cite{strehler2017energy} & Expanded graph & Shortest Path & $ \left( B/\epsilon \right) \left(|\mathcal{V}| + |\mathcal{E}| \right)^{\dagger} $ & - & Polynomial & Subject to $\epsilon$ \\
\cite{montoyaElectric2017} & Meta-heuristic & MILP & $ O \left(  K|\mathcal{V}| + |\mathcal{E}| \right)^{\dagger\dagger} $ & $ O\left( K|\mathcal{V}| + |\mathcal{E}| \right) $ & Exponential & - \\
\cite{fernandez2022arc} & Expanded graph &  ILP & $ \left( B/\epsilon \right) |\mathcal{E}| $ & $ \left( B/\epsilon \right) |\mathcal{E}| $  & Exponential & - \\
\textbf{This work} & Lagrangian relaxation  & Generalized RSP & $O\left( N |\mathcal{E}| + N |\mathcal{V}| \right)^\ddagger$ & $O\left( N   |\mathcal{E}| + N |\mathcal{V}|  \right)$ & Polynomial & Posterior bound \\ \bottomrule 
\end{tabular}
}
\footnotesize{$^\dagger$: $B$ is the value of capacity limit. $\epsilon$ is the tolerance of discretization. \quad $^{\dagger\dagger}$: $K$ is the number of breaking points in piece-wise linear approximation. \\ $^\ddagger$: $N$ is the number of charging stops during the trip. }



==> tabs/result-cmp.tex <==

\begin{table}[!tb]
    \centering
    \begin{tabularx}{\linewidth}{lXXX}
        \toprule
        & FAST & IDA-E & IDA-C \\
        \midrule
    Carbon footprint (tons) & 1.763 & 1.346  & 1.281 \\
    Travel time (hours) & 34.51 & 48.70 & 45.43  \\
    Charge time (hours) & 10.00 & 4.25 & 4.43  \\
    Wait time (hours) & 1.25 & 1.41 & 3.58  \\
    \bottomrule
    \end{tabularx}
    \vspace{1mm}
    \caption{Average performance for different algorithms among 1,000 origin-destination pairs. }\label{tab:res-cmp}
\end{table}
